Stay in Touch! Shape and Shadow Influence Surface Contact in XR Displays

The information provided to a person's visual system by extended reality (XR) displays is not a veridical match to the information provided by the real world. Due in part to graphical limitations in XR head-mounted displays (HMDs), which vary by device, our perception of space may be altered. However, we do not yet know which properties of virtual objects rendered by HMDs -- particularly augmented reality displays -- influence our ability to understand space. In the current research, we evaluate how immersive graphics affect spatial perception across three unique XR displays: virtual reality (VR), video see-through augmented reality (VST AR), and optical see-through augmented reality (OST AR). We manipulated the geometry of the presented objects as well as the shading techniques for objects' cast shadows. Shape and shadow were selected for evaluation as they play an important role in determining where an object is in space by providing points of contact between an object and its environment -- be it real or virtual. Our results suggest that a non-photorealistic (NPR) shading technique, in this case for cast shadows, may be used to improve depth perception by enhancing perceived surface contact in XR. Further, the benefit of NPR graphics is more pronounced in AR than in VR displays. One's perception of ground contact is influenced by an object's shape, as well. However, the relationship between shape and surface contact perception is more complicated.

==> fig/EXP2_FittedCurves.tex <==



\begin{figure}[t]
    \centering
        \includegraphics[width=0.32\linewidth, keepaspectratio]{fig/Exp2_OST_SxS.png}
        \includegraphics[width=0.32\linewidth, keepaspectratio]{fig/Exp2_VST_SxS.png}
        \includegraphics[width=0.32\linewidth, keepaspectratio]{fig/Exp2_VR_SxS.png}
        \caption{Fitted curves for 2AFC Task in Experiment 2} 
        \label{fig:exp2_fitted_curves}
\end{figure}




% increase image height
% crop left side
% thicken lines

% remove key

==> sections/999_deleted.tex <==



\section{Related Work}

\subsection{Shadows \& Ground Contact Theory} %Cast Shadows \& Ground Contact
% Depth Perception and Shadows
% 2.1 Depth Perception Theory
% 2.2 Color Hue and Luminance as Depth Cues


In 1950, James J. Gibson introduced his ground theory of space perception in which he argues that there is "no such thing as the perception of space without the perception of continuous background surface" \cite{Gibson:1950:PVW}. In this document and many others that followed, he postulated that visual space is not defined by arrays of objects in empty air--but by the layout of surfaces, sets of adjoined surfaces, and entities that are arranged in relation to surfaces \cite{Gibson:1979:EAV, Gibson:1975:IEP}. 


As the field of computer science advanced, Gibson's theories were tested with computer generated graphics, as well. By evaluating egocentric distance perception, or the perceived distance relative to a viewer, researchers were able to manipulate intermediate platforms and surface discontinuities to measure how they affected one's perceived distance to a target in highly controlled, virtual environments \cite{Meng:2001:DPM, Bian:2005:GDE}.  Through these studies, it became clear that people's perception of distance to objects varied as the optical contact---the location at which the projected image of an object contacts the image of the ground beneath it---between a target and the surface beneath it varied \cite{ Meng:2002:DPA, Ni:2005:DPM, Ozkan:2010:BSH}. As Gibson had formulated, the perception of surface-layout was essential for an individual to determine absolute and relative information for an object's position in space \cite{Gibson:1950:PVW,Gibson:1979:EAV}. 

%Cast shadows, which signal the distance between an object and the surface on which its shadow falls
%shadows provide subtle information about the spatial structure of the world in "automatic" and unconscious ways through mechanisms of visual perception, as opposed to the "reflective" and conscious ways of cognition. 
%%Cast shadows, which create additional points of contact between an object and adjacent surfaces, play a particularly important role in our perception of space

Cast shadows---from which humans infer size \cite{Yonas:1978:DSI, Wanger:1992:ESQ, Casati:2016:SFS }, from which humans infer shape \cite{Cavanagh:1989:SFS, Knill:1997:GS}, and from which humans infer the distance between an object and adjacent surfaces\cite{Thompson:1998:VG, Hu:2000:VCI, Madison:2001:UIS}---play a particularly important role in our perception of space. In fact, one's perception of the position of an object can shift dramatically depending on the placement of its associated cast shadow \cite{Mamassian:1998:PCS, Ni:2004:PSL}.  Kersten et al.'s "ball-in-a-box" study provides perhaps one of the most poignant examples of this response \cite{Kersten:1997:MCS}. Kersten and colleagues  demonstrated that by changing the location of a shadow in space, even a stationary object may appear to move (See Figure \ref{fig:ball-in-box}). Furthermore, their research demonstrated that cast shadow shading could be manipulated to unnatural extents---in their case with light, photometrically incorrect shading---and yet still provide a powerful tool to determine spatial location. Should the reader desire a deeper understanding of the relationship between shadows and perception, the authors suggest "The Visual World of Shadows" by Casati and Cavanagh as a notable, recent review \cite{Casati:2019:VWS}.  


% prior to  in spite of 
% further beyond this nevertheless 

The corpus of this prior research in perception was conducted in either real world environments or in completely virtual ones via desktop monitor. However, it can be more difficult to determine where virtual objects are situated in head-mounted displays (HMDs) \cite{Harris:2019:VTS}.



 
 
 
 
 
 
  %Distance estimation and how it relates to the current project (indirectly) --- ground contact informs depth perception
%% And aspects like the quality of graphics produced by these displays may be less important \cite{Willemsen:2002:PED, Thompson:2004:DQC}. These findings have been used to inform the design of contemporary head-mounted displays as well as their applications. 


% augmented reality only has access to a subset of these cues. 
% Perhaps, because of this consistency, even when the quality of graphics is reduced to mere wireframe structures, people can correctly interpret depth information \cite{Thompson:2004:DQC}. 
% Ni:2005:DPM, Carlos --> y. Judged distance for a single cylinder floating above the ground was determined primarily by the location at which the object contacted the ground in the projected image (“optical contact”),



% pictorial depth cues --- account for some distance underestimation but only in comparison to "impoverished" virtual environment e.g., no textured ground plane
 

 
 
\subsection{Shape \& Shadows in XR } % Object Geometry \& Depth Perception


%%%Accordingly, we understand that the presence of a shadow benefits depth perception in augmented reality. But it is uncertain how they should be rendered---especially for augmented reality displays that rely on additive light for rendering. These displays cannot subtract light and therefore cannot render black over a realworld scene. Accordingly,  it is impossible to use traditional shading techniques to render shadows in these devices.  To this end, developers are investigating alternative rendering techniques for shadows in OST AR. For example, Manabe et al. \cite{Manabe:2018:CVS, Manabe:2019:SII} employed a simple rendering technique that employs simultaneous contrast illusion (what they call brightness induction) to give the illusion of a shadow. 

In traditional computer graphics, evidence shows that cast shadows function as "visual glue" to attach virtual objects to surfaces \cite{Thompson:1998:VG,Madison:2001:UIS}. Furthermore, people become more accurate when estimating egocentric distances when objects are clearly connected to the ground via shadow \cite{Ni:2004:PSL}. However, it is unclear how we can best create "visual glue" for augmented reality devices. Augmented reality introduces new complexities to the graphics pipeline, especially for optical see-through displays (OST), which rely on additive light for rendering. These displays cannot remove light, and thereby darken, virtual or real objects. Dark color values in these displays become progressively more transparent such that a pure black is completely invisible. As a result, depth from shading cues are less reliable and the visual position of rendered objects in space becomes ambiguous. 

The inability to produce dark color values with fidelity is especially problematic for rendering cast shadows. Groups such as Manabe et al. \cite{Manabe:2018:CVS, Manabe:2019:SII} have begun to develop alternatives to producing more perceptually valid shadow rendering techniques for optical see-through devices. For example, in their method described in Ikeda et al. \cite{Ikeda:2020:SIO}, they used simultaneous contrast to create the illusion of dark color values within the umbra of a shadow by applying brighter color values outside of the shadow's penumbra. However, research on shadow generation algorithms gives rise to another question: how much fidelity is needed for accurate perception in AR? Adams et al. \cite{Adams:2021:SLC} attempted to answer this question by evaluating both perceptually motivated methods, like a variant of the one used in Manabe et al. \cite{Manabe:2019:SII}, and a non-photorealistic rendering (NPR) method for shadows. They found that their NPR method, which produced a white shadow, generally outperformed perceptually motivated methods for ground contact judgements in OST and VST augmented reality. 


% In optical see-through (OST) augmented reality, Rosales et al. \cite{Rosales:2019:DJO} demonstrated that, in the absence of a cast shadow, people perceive an object that is raised above the ground as farther away. In other words, they relied on the object's point of optical contact, which causes them to overestimate the distance of an object from the viewer \cite{ Meng:2002:DPA, Ni:2005:DPM, Ozkan:2010:BSH}. \haa{Jump in logic. clarify optical contact}

%  Some research has also been conducted to understand how effective shadows are for benefiting depth perception in OST AR



% Kyto et al. \cite{Kyto:2014:SDP} % also need reference for shadows
% Ooi et al, too? See notes in lit review shadow doc


Researchers have known that shadows may play an important role in alleviating depth issues in augmented reality. As such, several evaluations of shadow position and shape have been conducted in both mobile AR \cite{ Berning:2014:SDP, Sugano:2003:ESR} and in optical see-through AR \cite{Ping:2020:ESM, Gao:2019:IVO, Diaz:2017:DDP, Singh:2017:EFD}. In perceptual matching tasks, in which a person must align a virtual object with a marked position in the real world, the presence of a cast shadow dramatically improves depth judgements \cite{Berning:2014:SDP, Diaz:2017:DDP, Gao:2019:IVO}. Interestingly, shadows that are rendered in incorrect positions that are not aligned with real world lighting, may have either beneficial or detrimental effects. Gao et al. \cite{Gao:2019:IVO} found that lighting misalignments adversely affected perceptual matching in their experiment. However, "drop shadows" in which shadows are rendered immediately below an object, regardless of the lighting in the environment around them, dramatically enhance perceptual matching judgments \cite{Berning:2014:SDP, Diaz:2017:DDP}. In addition, Gao et al. \cite{Gao:2019:IVO} revealed that shadow shape did not significantly affect performance in their perceptual matching task. 

However, these results taken in isolation may be somewhat misleading. All of these objects with shadows were presented floating above the ground \cite{Berning:2014:SDP, Diaz:2017:DDP, Gao:2019:IVO,Ping:2020:ESM, Gao:2019:IVO, Diaz:2017:DDP}. This is important because anchoring shadows--which are shadows formed when an object sits on a surface--and detached shadows--which are formed when a shadow does not touch the object that cast it--are perceived somewhat differently. For example, the shape of a shadow when detached need only be approximately conformal to its object's shape \cite{Mamassian:1998:PCS, Casati:2019:VWS}. Accordingly, it makes sense that Gao et al.'s experiment found no differences between their hard, soft and 'round' (incorrect shape) shadow conditions when the test object was a rotating cube. Much more dramatic changes in shadow shape would be required to evoke changes in perception.

In contrast, an anchoring shadow may be more sensitive to mismatches between the contours of a shadow and its associated object \cite{Mamassian:2004:ISS, Casati:2019:VWS}. However, as noted in Do et al. \cite{Do:2020:EOS}, AR depth perception experiments rarely incorporate multiple object shapes. Accordingly, in their mobile AR study they evaluated how color and luminance interacted to affect depth perception across four objects: a cube, a sphere, the Stanford bunny, and a low polygon version of the Stanford bunny. Although they predicted that simple shapes (i.e., the cube and sphere)  would be more affected by color and luminance as depth cues than complex shapes, this was only partially true. The sphere proved to be more affected by luminance than any other shape, but the cube was not susceptible to either color or luminance. Their results are reasonable considering that spheres have previously proven more challenging to perceive in depth, than more distinctly faceted shapes, like cubes or icosahedrons, in prior research in VR, as well \cite{Powell:2012:VPV}. %In fact, our current study corroborates their findings on shape perception.  

%Our results partially support H1 (Shape). We cannot conclude that the depth perception of the low-fidelity, simple shape (the cube) is affected by color and luminance. However, the high fidelity, simple shape (the sphere) was the only model that demonstrated classical effects of color on depth perception

%t. A possible reason is that the cube is less susceptible to color and luminance as depth cues due to the sharp edges and shadows. 
%Therefore, we cannot state that there is any difference in depth perception between color conditions for the cube.
%The perceived depth of the sphere is also more affected by luminance compared to the complex bunny shapes. None of the bright colors are in a perceptually similar grouping as its darker counterpart. The complex shapes have many groupings that include both dark and bright colors, unlike the sphere. H1 (Shape) is supported for the high-fidelity objects. The depth perception of complex shapes may not be affected by color and luminance as much as a simple shape due to the presence of other depth cues such as shadows and contours. The bunny has multiple grooves and curves in the mesh, which give the viewer more shadows and highlights, causing them to rely less on color and luminance




%properties of three-dimensional (3D) virtual objects interact with color and luminance to affect depth perception


 % surface contact cues (shadows) -- classic work
% If we look at prior work that evaluates shadows as a depth cue in traditional computer graphics, we can see that a paradigm shift may be needed for us to truely understand how shadows are influencing depth judgements in AR. 



% However, it is unclear how to best create visual glue for AR devices---esp those that rely on additive light displays, like in optical see-through devices. % dark color values are transparent.

 %\haley{You didn't discuss shape! Do, the icosahedron study, etc.}
 %\cite{Singh:2017:EFD} % shape = octahedron 
                       % brightness, focal distance, age 
 %\cite{Gao:2019:IVO}   % shape = cube 
                        % shadows , lighting coherence (OST AR)
                        % rotated object 
 %\cite{Ping:2020:ESM}   % shape = sphere 
                        % shading model/ color / opacity   (OST AR) 
                        % specular highlights could help improve depth perception in AR
 
 %\cite{Diaz:2017:DDP} % shapes = exp 1) 3d? cube with randomized rotation  exp2) 2d plane, 3d torus 
                        % shadows, texture, shading model, etc
 %\cite{Berning:2014:SDP} %shapes = cube, rectangular prism sphere (3d) & 2d. mobile ar. 
                         % shadows
 %\cite{Do:2020:EOS} % shapes = cube, sphere, stanford bunny (lo, hi poly) 
                    % shadows 
                    % color, luminance  
 %\cite{Sugano:2003:ESR}  % movile AR. shadow shape affects presence? depth eval not what you think

%% Similarly, Al-Kalbani et al. show that virtual object position can influence perceived depth and affect freehand grasping accuracy [2], although such effects might be mitigated with dual view visual feedback [3]. Finally, the rotation of an object may change viewers’ access to depth cues. For example, if the flat face of a three-dimensional cube faces a viewer, it obscures information about the physical depth of the cube and may also provide less information about surface shading.



%Add note on importance of monocular depth cues
%Individual depth cues are weighted differently against each other, so it may not be necessary for all depth cues to perfectly mimic the real world setting. Occlusion is one such powerful, monocular depth cue that affects perception, which is why AR developers are actively working on perfecting it. But it is uncertain what other depth cues are needed to ensure that objects are accurately positioned in space. It is likely that it is unnecessary to render all depth cues photorealistically for accurate perception, but it is uncertain which depth cues need to be rendered and how they should be rendered given AR display limitations. 



%%%% The need for the evaluation of shading techniques for cast shadows in optical see-through AR is clear. These devices cannot rely on traditional shading techniques as dark color values become increasingly transparent to the point where black is not rendered at all. We need to pursue alternative methods for rendering cast shadows.  However, VST AR and VR could also benefit from this investigation. In theory, VST displays benefit from the traditional graphics pipeline in a manner similar to VR displays. If this is true--then we should find similar results in evaluations of different shading techniques between these devices. However, if conflicting depth information between the real and virtual stimuli impact depth perception in VST AR displays, then shading techniques may differ in effectiveness. 


==> sections/999_deleted_results.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{OG Results for Experiment 1}


\subsubsection{Does shadow shading method matter?}
%Therefore, we can say that people in our experiment were 0.493 times as likely to correctly determine ground contact in OST AR when the shadow was light in comparison to when the shadow was dark. 

To test the influence of shadow shading method on surface contact judgments in XR  we evaluated the two shadow shading methods (dark and light) when collapsed across all other conditions  for each device. The resulting fixed effects estimates ($\beta$), standard errors (Std. Error), and significance values (\textit{p}) are displayed in Tables \ref{tab:exp1_ost}-\ref{tab:exp1_vr} for each XR display. The \textit{Shadow (dark vs. light)} variable provides insight into the current research question, where negative fixed effects indicate that people were more likely to correctly interpret surface contact for dark shadows, and positive effects indicate that people were more likely to correctly interpret surface contact for light shadows. No Bonferroni correction was applied to this analysis since only one comparison was made. Therefore, the significance value remained \textit{p}$<0.05$. 

\paragraph{OST AR: } Non-photorealistic, light shadows resulted in an increased likelihood of correct response in comparison to photorealistic, dark shadows in both the OST AR (Table \ref{tab:exp1_ost}) and the VST AR devices (Table \ref{tab:exp1_vst}). 

\paragraph {VR: }For VR, there was no significant difference in responses between light and dark shadows  (Table \ref{tab:exp1_vr}). These findings confirmed our first hypothesis (\textbf{H1}), in which we predicted that the light cast shadow methods would enhance ground contact perception in both AR devices. It was also promising that people performed similarly when presented with light and dark shadows in VR---an indication that there were no adverse effects to surface contact judgments from light rendering of cast shadow.  





%%Non-photorealistic, white shadows resulted in an increased likelihood of correct response in comparison against photorealistic, dark shadows over all devices when collapsed ($\beta = 0.450 , SE= 0.052, p<0.0001$).

%%This analysis was performed for each device, and the Bonferroni corrected significance level was set to $p<0.0167$.

\subsubsection{Does object shape matter?} \label{exp1_h2_results}
%\haley{Cube no longer outperforms sphere in OST AR for HoloLens after Bonferroni correction} \sarah{you do not need to do bonferroni correction here if you do planned orthogonal contrasts. I thought that is what you had done before. E.g., compare each of the other two shapes(ico and sphere) to cube. If you want to compare each shape to each other, then you do need to correct for multiple comparisons.} 

To understand whether object shape influenced surface contact judgments in XR, we evaluated the three object shapes (cube, icosahedron, and sphere) when collapsed across all other conditions. For each display the results of these analyses can be seen in Tables \ref{tab:exp1_ost}--\ref{tab:exp1_vr}, where \textit{Shape(cube vs. ico)}, \textit{Shape(cube vs. sphere)}, and \textit{Shape(ico vs. sphere)} are the relevant variables for our research question. Negative fixed effect estimates ($\beta$) indicate that the first object in the comparison is more likely to receive a correct surface contact judgment. Positive effects indicate that the second object in the comparison is more likely. The Bonferroni corrected significance value for these comparisons was $p<0.0167=0.05/3$.

We found support for \textbf{H2}, which predicted that an object's geometry would affect surface contact perception. We argued that specific shape properties, such as the presence of straight edges or curved lines along the bottom of an object, would be pertinent to judgments of surface contact. We found that participants were more accurate in determining surface contact with the cube than the sphere in both VST AR and VR and that they were more accurate with the icosahedron than the sphere in VST AR and OST AR (Tables \ref{tab:exp1_ost}-\ref{tab:exp1_vr}).  People's perception of surface contact with the icosahedron varied in effectiveness, which may have been expected since the icosahedron---an approximation for a sphere with similar rectilinear properties to a cube---presented an intermediate case for study. Specifically, people performed best when judging the icosahedron in comparison to all other shapes in OST AR (Table \ref{tab:exp1_ost}), and they were worst when judging the icosahedron in comparison to all other shapes in VR (Table \ref{tab:exp1_vr}). In VST AR, the icosahedron resulted in better performance than the sphere but worse than the cube (Table \ref{tab:exp1_vst}).

%\sarah{related to my comment above, you have not specified how the shape comparisons were coded (0,1) so it is difficult to determine the direction of the effects based on positive or negative betas. I noticed this especially when I was trying to interpret what your "median performance" ico really means. Is there are straightforward way to communicate this?}\bbc{Agree with Sarah here. There is no way to verify your interpretations without knowing this. For example, isn't it true that people were significantly more accurate with the sphere than the icosahedron in VR?} 


%In detail, within the OST display, the icosahedron outperformed both the cube ($\beta = 0.289 , SE= 0.111, p=0.009$)  and sphere ($\beta$ ~\textdblhyphen~ $ 0.510 , SE= 0.109, p<0.0001$), and the cube outperformed the sphere ($\beta = 0.221 , SE= 0.104, p=0.034$). In the VST display, the cube outperformed both the icosahedron ($\beta = 1.120 , SE= 0.136, p<0.0001$) and sphere ($\beta  = 1.527 , SE= 0.132, p<0.0001$), and the icosahedron outperformed the sphere ($\beta$ ~\textdblhyphen~ $ 0.406 , SE= 0.103, p<0.0001$). In VR, the cube outperformed the sphere ($\beta  = 1.821 , SE= 0.156, p<0.0001$) and the icosahedron ($\beta$ ~\textdblhyphen~ $ 2.144 , SE= 0.156, p<0.0001$), but the sphere outperformed the icosahedron ($\beta  = 0.323 , SE= 0.099, p=0.001$). 

%Instead, we argued that the number of points of contact an object had with the ground surface would have a more dramatic effect such that we could expect the sphere (with a single, occluded point of contact) to perform worse than the cube (with many points of contact). Furthermore, we expected this relationship to hold across all devices. 

%%Collapsing over all devices, we found a significant trend for the accuracy of ground contact perception where: cube > icosahedron > sphere. The cube resulted in the highest likelihood of correct response in comparison to the icosahedron ($\beta = 0.823 , SE= 0.070, p<0.0001$) and the sphere ($\beta = 0.995 , SE= 0.069, p<0.0001$). And the icosahedron outperformed the sphere ($\beta = 0.995 , SE= 0.069, p<0.0001$). 


\subsubsection{Is there an interaction between shape and shadow?}

\emph{A priori}, we anticipated that there would be interactions between shape and shadow; however, we were uncertain how these interactions would be expressed. We were most interested in whether the advantage for non-photorealistic (light) shadows was consistent across the different shapes. This led us to conduct 3 unique, paired comparisons for shape $\times$ shadow conditions for each device, where the relevant variables for our research question included: \textit{Shadow$\times$Shape (cube: dark vs. light)},  \textit{Shadow$\times$Shape (ico: dark vs. light)},  and \textit{Shadow$\times$Shape (sphere: dark vs. light)}.  In a similar manner to the previous analysis, negative fixed effects for $\beta$ indicated that the first object in the comparison was more likely to elicit a correct response, whereas positive effects indicated the second object. Because three comparisons were made, the Bonferroni corrected significance value for these comparisons was $p<0.0167$.   %\sarah{have you defined DS and LS? Sometimes you use Dark vs. Light and but more often photorealistic vs. non-photorealistic when you describe these levels, so think about what is the best way to abbreviate, but either way it should be defined} %I decided to just use "dark vs light" for simplicity, even in the table
%\sarah{this is not 6 comparisons, it is 3--dark vs. light shadow for each of 3 shapes} \haley{ahhhhhhhh don't look at me i'm ashamed}


For the OST display (Table \ref{tab:exp1_ost}), the analysis indicates that the fixed effects between light and dark shadow conditions did not significantly differ for the icosahedron, nor did they differ for the sphere. However people were more likely to make correct surface contact judgments with the light shadow than the dark shadow when presented with a cube. In contrast, for the VST display (Table \ref{tab:exp1_vst}) people's surface contact judgments were significantly better for all objects when the object was presented with a light cast shadow. In VR (Table \ref{tab:exp1_vr}), people were more accurate when presented with the light shadow when the object was a sphere, but differences in shadow shading did not significantly affect people's performance given the cube or the icosahedron. %\sarah{this is a good description of the effects--RE my comment above, you are using light and dark consistently here, and not non-photo and photorealistic} 
In sum, across all devices and all objects, the light shadow condition always performs similarly to or better than the dark shadow condition, but the degree of this benefit is contingent upon object shape. %\jeanine{I sort of like the light and dark distinction better than photorealistic vs. non, but up to you all. It just makes it easier to understand which shadow is which in real time as you're reading.}\bbc{I agree with this, but there is inconsistency in the paper on this point. It will have to be fixed.} \haley{Absolutely agreed}

%Furthermore, participants performed significantly better when given the cube with the light shadow than they performed for all other conditions. And they performed worse when given the cube with the dark shadow than they did for all other conditions.  
%For the Microsoft HoloLens, the dramatic difference in performance between light and dark shadows in the cube condition indicates that there is a strong interaction of shape and shadow when a rectilinear shape is viewed in OST AR. It also demonstrates why the icosahedron outperforms the cube when we collapse across shadow conditions. 

%\sarah{your text is clear for these interactions, but I think the tables are somewhat confusing. I think what we care most about are the comparisons that you describe--does light vs. dark differ for each shape? So, the other comparisons in the table are distracting and also not motivated clearly. If you want to leave these in, I think more is needed in the caption and/or text to help the reader interpret.}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\subsection{Results} \label{exp2_results}
% For Experiment 2, we additionally compared surface contact judgments between the same object presented at two different orientations to understand if an individual object's orientation would influence surface contact judgments. For this research question, we ran separate analyses for each object and collapsed across all other conditions for a given object. 

For the second study, we used the same  generalized linear model (GLM) approach that we employed in the first study (see Section \ref{exp1_results}) to answer our research questions. Separate GLMs were run for each of the three XR devices to understand how an object's cast shadow shading, geometric complexity, and orientation affected people's surface contact judgments in each device. All three variables were included as within-subject predictors. Specifically, we modeled binary outcomes (correct or incorrect) for our input variables (predictors), which included object shape (2 levels: cube and dragon), object orientation (2 levels: rotated by $0^{\circ}$ and by $45^{\circ}$), and shadow shading (2 levels:  dark and light). 

We tested three planned comparisons for each device. These comparisons were: 1) the difference in surface contact judgments between dark and light shadow shading across all other conditions (i.e., \textbf{H4} the main effect of shadow shading); 2) whether surface contact judgments differed for different object geometries (i.e., \textbf{H5} the main effect of object shape); and 3) whether an object's orientation influenced people's surface contact judgments for cubes and for dragons (i.e., \textbf{H6} the main effect of orientation for each object). We also evaluated interactions between object shape and shading to better understand the relationship between these variables. 

%\sarah{I haven't read further yet, but I don't think you tested orientation x shading, rather orientation x object (collapsed across light/dark) based on your table.} \haley{There were multiple typos here. Fixed}




\subsubsection{Does shadow shading method matter?} \label{exp2_results_shading}
 
For each device, we evaluated the two shadow shading conditions (dark and light) when collapsed across all other conditions and found that people's  likelihood of correct response for whether an object was off the ground or not was significantly higher when presented with the non-photorealistic, light shadow in all three XR displays. Tables \ref{tab:exp2_ost}-\ref{tab:exp2_vr} display the fixed effects for dark versus light shadows across all three devices with the \textit{Shadow (dark vs. light)} variable. No Bonferroni correction was applied to this analysis since only one comparison was made. Therefore, the significance value remained \textit{p}$<0.05$.


 These findings confirmed our first hypothesis (\textbf{H4}), in which we predicted that people's surface contact judgments would be more accurate when objects were presented with light cast shadows in both AR devices. However, it is interesting to note that people's judgments were also significantly better with non-photorealistic, light shadows in the VR condition in this experiment as well. 
 



\subsubsection{Does an object's complexity matter?} \label{exp2_results_complexity}
%We  anticipated that geometric complexity would not inherently improve depth perception. Given the results of our first study, in which the cube outperformed the sphere across all devices, we predicted that people's likelihood of correct response would be more affected by the shape of an object along the bottom edge than by geometric complexity---where complexity is defined by the number of polygons used to construct a given object's mesh.  Even though the complex object evaluated in this study (the Stanford dragon) provided more points of contact along the ground than either the icosahedron or the sphere that were previously evaluated, we believed that the straight, rectilinear edges of the cube would still prove more beneficial to ground contact judgments. 

To understand how object shape complexity influenced surface contact judgments in XR, we evaluated judgments for the cube and the dragon when collapsed across all other conditions. For each display the results of these analyses can be seen in Tables \ref{tab:exp2_ost}--\ref{tab:exp2_vr}, where \textit{Shape (cube vs. dragon)} is the relevant variable for our research question.  Because only one comparison was made, no Bonferroni correction was applied. 

When we compared surface contact judgments between the cube and the dragon we found that our hypothesis held true for both VST AR (Table \ref{tab:exp2_vst}) and VR (Table \ref{tab:exp2_vr}) with judgments for the cube being more accurate than those for the dragon. However, people had a higher likelihood of correct response for the dragon in OST AR (Table \ref{tab:exp2_vr}). As such, we were only partially able to confirm \textbf{H5}. Although our prediction that more complex objects would not inherently improve ground contact judgments is supported by our results in VST AR and VR---showing an advantage for the cube over the dragon---the opposite result found with the OST AR display is surprising. %a more complex interaction between shape and shadow is apparent in the OST AR display. 


\input{tables/_Exp2_Tables}



\subsubsection{Does the orientation of an object matter?} \label{exp2_results_orientation} 

To determine whether orientation had an effect on judgments, we ran separate GLMs for the cube and the dragon. We did not collapse across objects for this analysis, given that a meaningful comparison of change between two objects in orientation could not be conducted. The initial orientations for each object (which we describe as $0^\circ$ orientation) is relative to that individual object's original orientation and, as such, is a local value rather than a global one. The relevant variables for our analyses in Tables \ref{tab:exp2_ost}--\ref{tab:exp2_vr} were: \textit{Orien  cube  ($0^\circ$ vs. $45^\circ$)} and \textit{Orien  dragon  ($0^\circ$ vs. $45^\circ$)}. The Bonferroni corrected significance value for these comparisons was $p<0.025$ since two comparisons were made. 





% \sarah{I think I understand this, but this doesn't seem consistent with what you say the models were in 6.4 which seems to imply all one model, not separate for cube and dragon. I think we need to be more clearer on this.} \haley{Fixed?} \sarah{better, but now I think the orient x shape label is misleading. I think this is just a comparison between orientation for the cube or dragon separately, so should not be presented as an interaction in the table. I would just say something like, Orien (0 vs. 45) for cube, and Orien (0 vs. 45) for shape.} \haley{Fixed!}


People's likelihood of correct response for the cubes significantly differed between the two orientations in OST AR (Table \ref{tab:exp2_ost})  and VR  (Table \ref{tab:exp2_vr}). Judgments for the cube at $0^{\circ}$ were more accurate than judgments for the cube at $45^{\circ}$ in OST AR, but the opposite was true in VR. People's accuracy also differed between the two dragon orientations in OST AR  (Table \ref{tab:exp2_ost})  and VR (Table \ref{tab:exp2_vr}) such that judgments for the dragon at $0^{\circ}$ were more accurate than judgments for the dragon at $45^{\circ}$ in both devices. However, in the VST AR condition, there were no significant differences in surface contact judgments between orientations for either the cube or the dragon  (Table \ref{tab:exp2_vst}). Because changes in orientation had a significant effect for both objects in OST AR and VR, \textbf{H6} was partially confirmed. 



\subsubsection{Is there an interaction between shape and shadow?} \label{exp2_results_interactions}
% Looking at shape $\times$ shadow $\times$ orientation interactions across devices,
% \sarah{are these corrected for multiple comparisons? We should talk more about whether all of these should be done, or only comparisons that are motivated, similar question to exp 1}. \haley{I agree with Sarah's comment that we should only discuss motivated comparisons. Otherwise, the actual questions of our research may become lost. This section was a relic from the the original draft that I sent out a month ago, anyway. If anything, I can parse this down to just look at shadow x orientation interactions for each shape (which is something we discussed previously) }


Given our findings in Experiment 1, which showed interactions for surface contact judgments between shape and shadow, we anticipated interactions in Experiment 2. Understanding these interactions was especially important for determining if the advantage of non-photorealistic, light shadows that we found in the current study was consistent across different shapes. We also believed that this analysis would help us better understand why we found a significant effect for shadow shading conditions in Experiment 2 but not in Experiment 1 for the VR display.  For these reasons, we conducted two unique, paired comparisons for shape $\times$ shadow conditions for each device, where the relevant variables for our investigation included \textit{Shadow$\times$Shape (cube: dark vs. light)} and  \textit{Shadow$\times$Shape (dragon: dark vs. light)}. The Bonferroni corrected significance value for these comparisons was \textit{p}$<0.025$ since two comparisons were made. %\sarah{okay now I understand the interactions you tested but these are not in the tables at all. See comment above that I don't think Orien should be presented as an interaction} \haley{Agreed! Fixed}


Across all devices we found significant effects of cast shadow shading for the cube and for the Stanford dragon, where people's surface contact judgments were more accurate with the light shadow (Tables \ref{tab:exp2_ost}-\ref{tab:exp2_vr}). These findings are encouraging because they provide evidence that the significant main effects we found for shadow shading condition in Experiment 2 are generalizable across objects of different complexity. 


==> sections/99_conclusions-old.tex <==





\section{General Discussion} \label{conclusions}

%Given that people's surface contact judgments in Experiment 1 were not affected by shadow shading condition, our current results suggest that under certain conditions, surface contact judgments in virtual reality may also benefit from non-photorealistic shading approaches---but perhaps to a lesser extent than its augmented reality counterparts.  \bbc{This point needs to be brought up in the discussion, but isn't that I can see. The point is: what is different between this experiment and experiment 1 for VR? Orientation and shape complexity.}

 %Yet it is clear that an object's shape does impact these judgments. \jeanine{But the finding of shape is from Exp 1, right? Maybe not worth mentioning again here since it doesn't follow from current study.}
 
 %Our results on orientation also have implications for the study and development of XR applications. In the realm of research, it is apparent that the angle from which we view a 3D object may affect spatial perception judgments related to that object \cite{Ooi:2001:DDA, Messing:2005:DPV, Ahn:2019:SPA, Feldstein:2020:EDP}. Accordingly, researchers must be careful about which objects they use to evaluate depth perception and how they position target objects in space when evaluating depth perception in XR. One solution would be to progressively rotate a virtual target to minimize the influence of one orientation like in Peillard et al.  \cite{Peillard:2019:SED}. However, for the development of commercial and educational XR applications,  we recognize that people may need to view virtual images that are placed at a specific angle, for example, when interacting with a virtual desktop monitor in AR. For these kinds of applications, understanding how specific shapes and orientations of objects influence where people perceive them to be positioned in space may be more pertinent. 

% Over two experiments 

%\bbc{As you are revising this, it needs to be cut down as well. The paper is too long. I think about two paragraphs shorter are needed. This means that your recap needs to be very concise.}


Over two experiments we evaluated how the shape of a 3D object and the appearance of its cast shadow influenced one’s perception of surface contact in immersive displays. These experiments were motivated in part by the common complaint of augmented reality technology adopters that virtual objects in real world spaces appear to "float." Cast shadows provide an important depth cue that can alleviate this issue by perceptually attaching objects in space to the surfaces beneath them \cite{Thompson:1998:VG, Madison:2001:UIS}. Furthermore, cast shadows can improve depth perception in extended reality (XR) displays, which has been demonstrated by prior work in virtual desktop environments \cite{Ni:2004:PSL} as well as by prior work in augmented reality HMDs \cite{Diaz:2017:DDP,Gao:2019:IVO}. %\sarah{this last sentence is not clear about the distinction you are making between XR and VR and seems misleading to call the Braunstein work a virtual environment anyway--maybe instead graphical desktop displays?} \haley{very valid point}  

%To better understand how people perceive surface contact in XR displays, our first study looked at how virtual object geometry and cast shadow shading affected people's surface contact judgments across three different XR displays---each with their own unique rendering properties that may impact how monocular depth cues are utilized by a viewer: optical see-through augmented reality (OST AR), a video see-through augmented reality (VST AR), and virtual reality (VR). For our evaluation we asked volunteers to assess three object shapes (cube, icosahedron, and sphere) and two shadow shading conditions (dark and light). We found that people's judgments in both AR displays were more accurate when presented with the light shadow than the more realistic, dark shadow. In contrast, differences in shadow shading did not significantly affect people's surface contact judgments in VR. \sarah{I would add, except for with the sphere} \sarah{do you think there was a shadow effect for the sphere in VR because performance was overall worse, so there was room to improve? It is hard to know how much worse because we do not have figures of the likelihood curves.} Furthermore, we found effects of object shape and of object shape $\times$ shadow shading for all devices. \sarah{the previous sentence should not include an interaction--explain in words--what do you mean by this? Your next sentence doesn't say anything about shadow shading, only shape.} People's judgments were more accurate for the cube than the sphere for VST AR and VR, and their judgments were more accurate for the icosahedron than the sphere for VST AR and OST AR.

In both Experiment 1 and 2 we evaluated three extended reality (XR) displays with unique rendering properties: an optical see-through display, a video see-through display, and a virtual reality display. And we found different effects of object shape and shadow shading on surface contact judgments for each device. We believe this pattern showcases that the manner in which elements are rendered in XR affects our spatial perception, regardless of the device employed, and that these effects may not be the same between different displays. However, we are unable to conclude what aspects of these displays contributed to these differences in perception with this study alone.  

In regard to the effect of shadow shading on surface contact judgments in XR, in both Experiment 1 and Experiment 2 we found that people's surface contact judgments when presented with light, non-photorealistic shadows were either more accurate or as accurate as those presented with dark, realistic shadow shading in OST AR and VST AR. However, we only saw this effect in VR for our second experiment. Given that people's surface contact judgments in Experiment 1 were not affected by shadow shading condition, our current results suggest that under certain conditions, surface contact judgments in virtual reality may also benefit from non-photorealistic shading approaches---but perhaps to a lesser extent than its augmented reality counterparts. Our findings for object complexity and orientation for Experiment 2 may provide some insight into this finding. 

%Taken together, our first study provides evidence that people are as accurate when determining surface contact with the light shadow condition as the dark shadow condition across all of the displays tested, and they are even more accurate with the light shadow conditions in AR displays. Furthermore, we reveal that surface contact judgments are influenced by object geometry. Given the comparatively poor performance of the sphere across all devices, our findings caution against the use of spheres in tasks that require accurate surface contact perception. 
%  
%Overall---across both experiments, across all object shapes, and regardless of object orientation---we consistently found that people's surface contact judgments when presented with light, non-photorealistic shadows were either more accurate or as accurate as those presented with dark, realistic shadow shading. In addition, we found that object shape and orientation influence surface contact judgments across devices with one exception. Surprisingly, we did not see an effect of object orientation in the video see-through AR display, which warrants further investigation. 
% Given that people's surface contact judgments in Experiment 1 were not affected by shadow shading condition, our current results suggest that under certain conditions, surface contact judgments in virtual reality may also benefit from non-photorealistic shading approaches---but perhaps to a lesser extent than its augmented reality counterparts.  \bbc{This point needs to be brought up in the discussion, but isn't that I can see. The point is: what is different between this experiment and experiment 1 for VR? Orientation and shape complexity.}

 
%% exp 2 results   

%In our second study, we evaluated surface contact judgments across the same, three XR displays. We compared a complex shape (the Stanford dragon) against a simple, rectilinear shape (a cube) across the same two shadow shading conditions that were employed in our first study (light and dark). And we presented both target objects at multiple orientations.  We replicated the findings of our first study, finding that people's surface contact judgments were more accurate in both AR displays when objects were rendered with a light, non-photorealistic cast shadow. However, unlike in our first study, we also found the judgments in the VR display were significantly more accurate when objects were presented with a light shadow. 

 
%One of the reasons that creating accurate spatial perception in augmented reality (AR) devices is particularly challenging is that these displays  have unique graphical limitations. Optical see-through (OST) augmented reality devices provide a particularly poignant example of this, since their reliance on additive light displays makes it nigh impossible for them to render black---an important color for rendering realistic shading and shadow. Undeterred by the graphical limitations of additive light displays, fascinating prior work by researchers at Ritsumeikan University \cite{Manabe:2019:SII, Ikeda:2020:SIO} has investigated ways we may better render perceptually realistic shadows in OST AR. Their research leverages a person's visual system to create the illusion of dark color values using simultaneous contrast illusion to generate shadows.   \haley{They didn't invent the simultaneous contrast shadow rendering technique. We didn't invent this technique. It's been used in industry for years. But I might as well butter them up since they'll probably be reviewing our paper again.}

%Although it has been theorized that augmented reality displays need to render realistic graphics that match reality for veridical spatial perception  \cite{Adams:2020:RCC, Drascic:1996:PIA, Kruijff:2010:PIA}, there is little empirical evidence to support this claim. This paucity of evidence is driven by the inability of contemporary AR displays to render graphics that match reality---a technical limitation that makes such a theoretical claim difficult to verify. We may, nevertheless, evaluate non-photorealistic graphics that deliberately defy the demand for realistic graphics to better understand perception in AR displays. A similar approach has been used in virtual reality (VR) research to understand how the quality of graphics affects distance perception \cite{Thompson:2004:DQC}

 

The effects of object shape \& object complexity found in the current study provide evidence that AR designers and researchers may want to carefully consider the geometric shape of the objects used in their applications. In Experiment 1, we found only one case across all three XR devices where people's judgments were more accurate for the sphere than the other target shapes (where judgments where more accurate for the sphere than the icosahedron in VR). Our current study provides some evidence that spheres may be less effective than other shapes for establishing surface contact. Do et al. \cite{Do:2020:EOS}, in a similar line of research, discovered that people's depth judgments to spheres were more sensitive to changes in luminance than other shapes in mobile AR. Both our results and those of Do et al. \cite{Do:2020:EOS} provide a cautionary tale against the use of spheres for AR applications that require accurate spatial perception.  These findings may have implications for depth perception in XR studies, as spheres are a common target object used in distance perception research for these devices \cite{Armbruster:2008:DPV, Gao:2019:IVO, Peillard:2019:SED, Peillard:2020:CRP}.

In Experiment 2, in which we evaluated people's surface contact judgments between simple and a complex geometries, we found that people's surface contact judgments were better for the cube than the dragon (i.e, the more complex object) in both VST AR and VR. This finding suggests that object complexity does not inherently improve surface contact perception. However, judgments were more accurate for the dragon than the cube in the OST AR display.  Our findings on surface contact perception may have ramifications for depth perception in XR devices, but further research that includes a direct comparison of object shape and shadow shading on egocentric distance perception is needed to substantiate this claim. 

%In addition, we found that object shape influences surface contact judgments, where judgments were more accurate for the cube than the sphere in the VST AR and VR. And judgment for the icosahedron were more accurate than the sphere in VST AR and OST AR. Judgements for the sphere were only more accurate than one other shape condition (the icosahedron) in VR. Given that there was only one case across all three XR devices where people's judgments were more accurate for the sphere than the other target shapes, our current study provides some evidence that spheres may be less effective than other shapes for establishing surface contact.  This finding may have implications for depth perception in XR studies, as spheres are a common target object used in distance perception research for these devices \cite{Armbruster:2008:DPV, Gao:2019:IVO, Peillard:2019:SED, Peillard:2020:CRP}.  In addition, we found that there were interactions between shape and shadow for all three XR devices, but the shapes that showed interactions with shadows differed for each devices. 

%Both our results and those of Do et al. \cite{Do:2020:EOS} provide a cautionary tale against the use of spheres for AR applications that require accurate spatial perception. 

In addition, our results on orientation may have implications for the study and development of XR applications. In the realm of research, it is apparent that the angle from which we view a 3D object may affect spatial perception judgments related to that object \cite{Ooi:2001:DDA, Messing:2005:DPV, Ahn:2019:SPA, Feldstein:2020:EDP}. Accordingly, researchers must be careful about which objects they use to evaluate depth perception and how they position target objects in space when evaluating depth perception in XR. One solution would be to progressively rotate a virtual target to minimize the influence of one orientation like in Peillard et al.  \cite{Peillard:2019:SED}. However, for the development of commercial and educational XR applications,  we recognize that people may need to view virtual images that are placed at a specific angle, for example, when interacting with a virtual desktop monitor in AR. For these kinds of applications, understanding how specific shapes and orientations of objects influence where people perceive them to be positioned in space may be more pertinent. 

\subsection{Limitations}

% do not control for background 
% do not control for object shading 
% Current results only generalize to surface contact judgments. We can hypothesize that our results will transfer to egocentric depth perception based on prior research in VR. But we cannot know this for certain without actually evaluating our stimuli in an egocentric depth perception study 


There are clear limitations to the current research. For one, we did not manipulate object shading in our experiments because we were more interested in the effect of an object's shape on ground contact judgments. However, given the sensitive effects of shadow luminance values on surface contact judgments observed in our studies, it would be reasonable to claim that our results were influenced by the color of our target objects. Similar prior research on surface contact perception in XR has evaluated the effect of differences in object and shadow shading on people's surface contact judgments \cite{Adams:2021:SLC}.  Based on this prior research, we elected to use a median gray value to shade all of our test objects to mitigate effects of object shading, although we recognize that this is an imperfect solution.

Another limitation with both the current work and the prior work conducted by Anonymous et al. \cite{Adams:2021:SLC} is that neither of these experiments manipulate the color of the background surfaces on which target objects are displayed. Yet just as an object's shading may influence our spatial perception of that object in space \cite{Do:2020:EOS, Diaz:2017:DDP,Ping:2020:ESM,Ahn:2019:SPA}, so may the backdrop upon which it is presented \cite{Ozkan:2010:BSH}.   In our case, we used the same, median blue tablecloth throughout both experiments.  %Based on this prior research, we elected to use a median gray value to shade all of our test objects to mitigate effects of object shading, although we recognize that this is an imperfect solution.  


%Adams and colleagues assessed the effect of object and shadows shading methods on people’s surface contact judgments given light and dark shading conditions. Four object $\times$ shadow shading conditions were evaluated such that both object and shadow were evaluated with light and dark shading methods. Given a darkly shaded object, the light shadow condition performed better than all other conditions in VR, VST, and OST displays. But for VST AR and VR displays, the lightly shaded object with a light shadow performed similarly to both of the dark shadow shading conditions. This provides some evidence that object shading can indeed affect a shadow’s ability to provide surface contact information. However, even these findings encourage the use of non-photorealistic shading, since both light shadow conditions, regardless of target object shading, performed better than or equivalently to the dark shadow shading conditions. 
\section{Conclusions}

%The results of our current research and the results of Adams et al. \cite{Adams:2021:SLC} depict perception in OST AR as highly sensitive to changes in luminance, especially for surface contact judgments. This research is also in line with prior work conducted by Singh et al. \cite{Singh:2017:EFD} which demonstrated that the brightness of a target affected distance perception in optical see-through device. 

%It is also possible that differences in display resolution, which we do not directly measure due to the difficulty of comparison between traditional and optical see-through optics, may have influenced our results. However, we believe that this is unlikely given the incongruency between people’s ratings of each display’s quality of graphics and their actual performance. In addition, prior research conducted by Thompson et al. \cite{Thompson:2004:DQC} demonstrated that quality of graphics had no effect on distance judgments in virtual environments. 


%From our research findings, we may begin to extrapolate XR developer and design guidelines. 

Because the light  shadows in our current study enhanced people's accuracy in surface contact judgments---it may be worthwhile to evaluate whether more ambitious non-photorealistic rendering approaches facilitate spatial perception in AR. Evaluating colorful shadows, like those designed by Ooi et al. \cite{Ooi:2020:CCS}, for AR may be a desirable starting point. If more research findings are able to confirm the benefits for non-photorealistic rendering for spatial perception in AR, then we may be able to encourage the use of more stylized graphical elements for designers and developers of XR applications. However, for the moment, we must be cautious about arbitrarily applying non-photorealistic effects to XR simulations before evaluating them, especially given the results of  Cidota et al. \cite{Cidota:2016:UVE} which showed that blur and fade may have adverse effects on action-based depth judgments in augmented reality in personal space. 

%If non-photorealistic shading methods for shadows like the light shading method used here are not detrimental to surface contact judgments, then it may be worthwhile to investigate how other non-photorealistic shading techniques 


Although we suspect that our current findings have ramifications for egocentric depth judgments in XR displays given the findings of prior research \cite{Ni:2004:PSL}, for the current study we can only generalize our findings to surface contact judgments. In future research, it may be worthwhile to evaluate how object shape and cast shadow shading manipulations affect more direct measures of depth perception. Rosales et al. \cite{Rosales:2019:DJO} demonstrated that, in the absence of cast shadows, people perceive an object that is placed above the ground incorrectly as farther away. This may help explain some of the effects of overestimation found in prior AR depth perception research, especially given that many assessments use floating objects for assessment \cite{Peillard:2019:SED,Swan:2015:MRD,Singh:2012:DJR}. In future work, we intend to evaluate how photorealistic and non-photorealistic shadows affect egocentric depth judgments in XR displays. 





%Our findings have interesting implications for the design and development of XR displays and applications. On one hand, our results on shadow shading encourage the use of non-photorealistic rendering techniques in XR displays, since developers need not be restricted by the theoretical demand of consistent pictorial depth information \cite{}  for accurate depth judgments. Being able to employ non-photorealistic shading techniques in XR may also be beneficial for people with low vision who would benefit from high contrast imagery that non-photorealistic shading can provide. Moving forward, however, it will be important to evaluate the effect of more invasive non-photorealistic rendering techniques before adopting this strategy to improve depth perception. Furthermore, in the current research we solely evaluate surface contact judgments. Although providing surface contact information has been demonstrated to improve egocentric depth perception in prior research \cite{}, it will be important to directly evaluate how non-photorealistic graphics affect egocentric depth perception in these devices before adoption. 







%Several research groups have evaluated both the automatic and reflective processes by which humans seem to infer information from shadows. 

%However, humans infer a variety of information from shadows beyond position, which is a more automatic cognitive process. And the 

% Ni et al \cite{Ni:2004:PSL}
% Mention shadows effects are task specific (Cavanaugh, Bonfiglioli) 

%\haa{non photorealistic rendering and depth perception. mention vaziri, too}



%In addition, hardware solutions and different optical solutions Cite Peillard:SED:2019. retinal projections, etc also beneficial. 

%%%Ahn et al 2019 \cite{Ahn:2019:SPA} compared handheld AR, VST AR, and OST AR. Significant effects of display type, rendering style, and viewing angle. E.g., VST AR most accurate and fastest size perception. Mobile display cause serious over-estimation. OST AR caused significant underestimation. oh my. %%% Scale / Size manipulation


%It may also be beneficial for researchers to enlist multiple methods of evaluating depth perception, since the underlying mechanisms guiding judgments of depth differ between passive and action-based tasks. Bonfiglioli et al. \cite{Bonfiglioli:2004:DEC}, for example, found that shadow shape influenced grasping to a target object but not object identification. 

%"Their experiment suggests that there is a task-dependent influence on cast shadows on human performance. In the case, of object-oriented actions, cast shadows may represent further affordances of the object, and as such compete for the control of the action "




==> sections/99_deleted.tex <==
%\section{Introduction}
%XR displays have graphical limitations, which vary depending on the device. 

%\haley{Needs to be more broad!! provide context! Why do we care??? maybe talk takl about colored shadows, as well. Ease us into it a little smoother }


A common complaint by consumers of augmented reality (AR) applications is that virtual objects appear ``floaty'' in these displays. A Pok\'{e}mon in Pok\'{e}mon Go, the popular mobile AR game, may seem to float above the ground where it is placed. And a virtual hat in an AR face filter, like those used by Snapchat or Instagram, may appear detached from a person’s head. A detached---or ``floaty''---appearance is a strong indicator that the depth information presented by virtual stimuli and the information presented by the real world environment do not sufficiently match. In the current research, we evaluate how the way we render cast shadows for objects of different geometric shapes and orientations affects one’s perception of surface contact across different extended reality (XR) displays. 

Cast shadows are a powerful depth cue that may resolve the detached appearance problem. Though visually unassuming, shadows firmly ground objects in space by creating points of contact between objects and the surfaces beneath them \cite{Thompson:1998:VG, Hu:2000:VCI, Madison:2001:UIS}. Yet rendering realistic shadows can be complicated as well as computationally expensive in XR displays. For example, optical see-through (OST) AR devices cannot render dark color values due to their reliance on additive light displays. Instead, dark color values become increasingly transparent as they approach black. In addition, both video see-through (VST) and optical see-through (OST) AR displays must blend together both real and virtual inputs to create images. In contrast, virtual environments rendered by virtual reality (VR) displays benefit from consistent.  \bbc{This is not true.}.


%Shadows are an especially powerful cue for depth perception that function by creating points of contact between an object and the surface beneath it. However, additive light displays, like those employed by optical see-through (OST) augmented reality, cannot render black, which makes it nigh impossible to render shadows using the traditional graphics pipeline. Instead, dark shadows are rendered with increasing translucency as the color approaches black.  Translucent shadows may have poor salience and thus be a poor tool for creating ground contact in OST AR. A common complaint by people who use consumer AR is that virtual object appear "floaty"--indicating that objects rendered in AR are not adequately attached to the surfaces beneath them. In an attempt to design device-agnostic solutions, in the current research we probe into how object geometry, object orientation, and the visual representation of an object’s shadow affect spatial perception in XR. 





%A common complaint from users of augmented reality (AR) technology is that virtual objects appear to ``float'' within real world scenes. A detached---or ``floaty''---appearance is a strong indicator that the depth cues provided by virtual stimuli are insufficient to accurately locate the stimulus' position within a real world environment. Given that the human visual system integrates information from a variety of cues to interpret depth, the presence of unreliable depth cues can cause unstable depth perception when these cues are not combined in a consistent manner \cite{Landy:1995:MMD, Ernst:2004:MSR}. Drascic and Milgram \cite{Drascic:1996:PIA} as well as Adams \cite{Adams:2020:RCC} have pointed to cue conflicts as a potential factor contributing to inaccurate depth perception in augmented reality. 




% SHADOWS
%   traditional graphics pipeline and Renaissance art shadows
%   stylish shadows

%   but what about shadows in XR?
%   perceptually motivated shadows
%   but realistic shadows not always needed (diaz, adams)

%   if we dig into perception literature, we find
%   how shadows affect depth perception
%   how even non traditional shadows can improve depth perception

%   Traditionally, more consistent depth cues = better accuracy
%   but there is nascent research that suggests this may not always be necessary!

% This is promising, but there has been no robust study of this effect. In fact, the few XR research studies that have brought this point to the surface have done so almost as if by accident
% (good news for OST AR)
    % limits to rendering due to display
    %
%\input{fig/franklin.tex}




%\subsection{Depth Perception in XR}
% 2.2 Egocentric Distance Perception in AR 

Although the real world is filled with rich, consistent depth information \cite{Landy:1995:MMD,  Hillis:2002:CSI}, virtual information rendered by head-mounted displays (HMDs) can introduce distortions in depth perception caused by impoverished pictorial depth cues in sparse environments \cite{Renner:2013:PED, Harris:2019:VTS}, and caused by mechanical factors, such as added head weight \cite{Buck:2018:CDE, Willemsen:2009:EHM} and restricted field of view \cite{Knapp:2004:LFV, Li:2015:EMD, Willemsen:2009:EHM}. Fortunately, in VR displays depth perception distortions are relatively consistent. An extensive body of literature has uncovered the graphical and mechanical properties that account for the poorly understood yet consistent distance compression found in immersive VR HMDs \cite{Loomis:2003:VPE, Creem-Regehr:2015:EDP, Creem-Regehr:2015:PAS, Renner:2013:PED}\bbc{This paragraph needs work.}.  

%%For a more in-depth review of distance estimation literature in virtual reality, see Creem-Regehr et al. \cite{Creem-Regehr:2015:PAS} and Renner et al. \cite{Renner:2013:PED}

Considering that much of the distance compression seen in virtual reality (VR) HMDs has been attributed to mechanical factors \cite{Buck:2018:CDE, Willemsen:2009:EHM, Renner:2013:PED}, one might predict that AR head-mounted displays would suffer from the same fate. Nevertheless, research evaluating depth perception in AR has thus far been inconclusive. Some prior research has found that immersive AR displays elicit similarly compressed responses as seen in VR \cite{Swan:2007:EDJ,Berning:2014:SDP,Kyto:2014:SDP, Jones:2011:PVI, Vaziri:2017:IVE,Rosales:2019:DJO,  Diaz:2017:DDP}, while other research has shown accurate distance estimation and even distance overestimation \cite{Swan:2006:PMT,Jones:2008:EVR,Pointon:2018:JAC, Peillard:2019:SED, Peillard:2020:CRP, Gruenefeld:2020:BTS}. Worse yet, these inconsistencies are found across both video see-through  \cite{Kyto:2014:SDP,Vaziri:2017:IVE} and optical see-through \cite{Swan:2006:PMT,Swan:2007:EDJ,Creem-Regehr:2015:EDP,Jones:2008:EVR, Pointon:2018:JAC,Rosales:2019:DJO} AR displays. 

Direct comparisons of depth perception across different types of AR devices can be difficult. And thus far no singular display type has proven itself superior to others for accurate depth perception, which may be expected given there are technological and perceptual trade-offs between video see-through and optical see-through devices \cite{Rolland:1995:COV}. A contemporary example of this challenge can be seen in the egocentric depth perception studies conducted by Ballestin et al. \cite{Ballestin:2018:PAP} and Medeiros et al. \cite{Medeiros:2016:PDO}. Both studies evaluated optical see-through and video see-through HMDs in action-based reaching tasks. Ballestin et al. \cite{Ballestin:2018:PAP} found that an optical see-through device (the Meta 2) outperformed their custom video see-through display in terms of accuracy. Yet Medeiros et al. \cite{Medeiros:2016:PDO} found the opposite to be true when evaluating the Meta 1 against an Oculus Rift with attached stereoscopic video cameras.\bbc{I'm not really seeing how the prior three paragraphs advance an argument relevant to this paper. It seems to me what you want to talk about is how shadows provide important cues for depth perception, shadow rendering is different among different technologies (which you have done), and move on to motivate the importance of understanding how shadows are perceived using the different technologies and what the degrees of freedom a designer has are, and how that affects depth perception. A tour of egocentric distance estimation and so on isn't helpful here. Moreover, some of the stuff you've said isn't quite accurate, so that's a problem, too. In general, I think the intro needs to be more focused.} 



%% REMOVED PARAGRAPH BECAUSE BG SECTION IS TOO LONG
%%Within personal space, reaching paradigms have also been used to compare OST AR against VR displays. The results of this research are similarly difficult to interpret. Batmaz et al. \cite{Batmaz:2019:DHM} boldly asserted that any differences in depth perception between OST AR and VR displays did not adversely affect interaction after finding no significant differences in reaching behaviors between the Meta 2 and HTC Vive Pro in their study. Cidota et al. \cite{Cidota:2016:UVE} similarly found no significance in reaching behaviors when comparing OST AR and VR conditions with the AIRO II HMD, which supported both display modalities. However, Swan et al. \cite{Swan:2015:MRD} found that people overestimated the distance of virtual target objects in the nVisor ST60 OST AR display within personal space--a pattern that is typically not found in VR since VR HMDs induce distance compression. Even looking at depth perception studies in action space, which extends between 2 and 30 meters, we find irregular patterns in spatial perception. Using a blind walking paradigm, Jones et al. \cite{Jones:2011:PVI} found underestimation in OST AR (the nVisor ST)---but to a lesser extent than what had been found in VR. Pointon et al. \cite{Pointon:2018:JAC} found evidence of both over- and underestimation in their assessment of depth perception via affordance judgements in OST AR (the HoloLens 1), which they reported was likely due to the different spatial characteristics of the virtual objects.



%\haley{MERGE WITH FIRST PARAGRAPH}
%This volatility of this prior research reflects a common complaint by users of AR technology that virtual objects appear to 'float' within real world scenes. A detached---or 'floaty'---appearance is a strong indicator that the depth information presented by virtual stimuli and the information presented by the real world environment do not sufficiently match. 

The presence of unreliable depth cues can cause unstable depth perception when these cues are not combined in a consistent manner \cite{Landy:1995:MMD, Ernst:2004:MSR}, which may explain the volatility of this prior XR research. The challenge of presenting consistent depth information is especially difficult in augmented reality since AR displays must additionally match depth information between both real and virtual stimuli  \cite{Adams:2020:RCC, Drascic:1996:PIA, Kruijff:2010:PIA}. Perhaps because of this difficulty, consistent patterns of depth perception distortions elude the field of immersive augmented reality. 


To better match graphics in AR with real world depth information, researchers have tried to create increasingly, perceptually realistic graphics to match real world environments \cite{Manabe:2019:SII, Ikeda:2020:SIO}. However, preliminary evidence suggests that non-photorealistic shadow shading techniques in AR may be beneficial for attaching virtual objects to the surfaces beneath them \cite{Adams:2021:SLC}. This finding is surprising given that  researchers have previously theorized that consistent depth cue information between real and virtual objects is necessary to improve depth perception in augmented reality \cite{Adams:2020:RCC, Kruijff:2010:PIA, Drascic:1996:PIA}. Still, Adams et al. \cite{Adams:2021:SLC} only evaluated a single, rectilinear shape across their experiments.  In the current work, we directly investigate how photorealistic and non-photorealistic shadow shading techniques affect surface contact judgements in XR. Furthermore, we conduct our analyses using objects of different shapes and orientations. Should our results show that a non-photorealistic (NPR) shading technique can benefit perceived ground contact in XR, then our research will open up an avenue for both researchers and developers to explore how NPR graphics can be employed to improve our spatial perception in these devices.

%Should our results coincide with those of Adams et al. \cite{Adams:2021:SLC}, then our findings would encourage the use of non-photorealistic shading to improve perceived ground contact in XR. 




%% For the current project, we want to know how the manner in which we render virtual objects affects one’s spatial perception in extended reality (XR) displays. Therefore, we conduct a series of perceptual studies across three unique types of XR display: virtual reality (VR), video see-through augmented reality (VST AR), and optical see-through augmented reality (OST AR). 




%However, given the results of \haley{Adams et al. [InReview]}, it is worth investigating how nontraditional shading approaches affect depth perception in XR. Furthermore, for these shading effects to be understood, multiple geometries need be assessed. 



%%Preliminary evidence suggests that non-photorealistic shadow shading techniques in AR may be beneficial for attaching objects to the surfaces beneath \haley{(Adams et al. [InReview])}. This finding is surprising given what we know about depth perception. In real world environments conflicting depth cue information causes perceptual uncertainty, which indicates that an individual lacks confidence about their assessment of where objects are positioned in space \cite{Drascic:1996:PIA}.  It has been demonstrated that perceptual uncertainty decreases as the number of consistent depth cues increases to the limits of the perceptual system \cite{Jacobs:2002:WDV}, and it has been theorized that consistent depth cue information between real and virtual objects will improve depth perception in augmented reality, accordingly \cite{Adams:2020:RCC, Kruijff:2010:PIA, Drascic:1996:PIA}.


















\section{Introduction}
To better match graphics in AR with real world depth information, researchers have tried to create increasingly, perceptually realistic graphics to match real world environments \cite{Manabe:2019:SII, Ikeda:2020:SIO}. However, preliminary evidence suggests that non-photorealistic shadow shading techniques in AR may be beneficial for attaching virtual objects to the surfaces beneath them \cite{Adams:2021:SLC}. This finding is surprising given what we know about depth perception in real world environments. \sarah{what do we know? That realistic shadows matter?} Still, Adams et al. \cite{Adams:2021:SLC} only evaluated a single, rectilinear shape across their experiments.  In the current work, we directly investigate how photorealistic and non-photorealistic shadow shading techniques affect surface contact judgements in XR. Furthermore, we conduct our analyses using objects of different shapes and orientations. Should our results coincide with those of Adams et al. \cite{Adams:2021:SLC}, then our findings would encourage the use of non-photorealistic shading to improve perceived ground contact in XR. 



\section{Overview}
%We conduct two evaluations to understand how the way we render graphics in extended reality (XR) displays affects spatial perception . In these studies, we pay particular attention to virtual object geometry and shadow shading technique since they both play important roles in depth perception. Shadows, in particular, are essential for creating a sense of contact between an object and the surface beneath it, thus integrating an object--be it virtual or real--within space. We hope to better understand performance trade-offs across devices when photorealistic and non-photorealistic rendering techniques are employed.

%We also posit that it is imperative for researchers to study how different types of immersive display affect one's perception of space, as poor spatial perception may render the displays useless for many training and education applications. We , therefore, conduct our studies across three, unique types of head-mounted displays: virtual reality (VR), video see-through augmented reality (VST AR), and optical see-through augmented reality (OST AR). %By evaluating multiple displays, we hope to better understand performance trade-offs across devices when photorealistic and non-photorealistic rendering techniques are employed.

We evaluate a viewer's sense of perceived surface contact over two studies. In both, shadows are manipulated to either have dark (photorealistic) or light (non-photorealistic) color values. In the first experiment, we manipulate both object geometry and shadow shading technique to understand what components of object geometry benefit surface contact perception. 
In our second experiment, we use one of the simple geometries from our first study and compare ground contact perception between the object and the object when rotated. We also compare this simple geometry to a far more complex model (the Stanford dragon) and the complex model when rotated.

%Preliminary evidence has shown that photorealistic renderings may not inherently benefit depth perception in augmented reality. The current research will rigorously test that finding. 


%Finally, in our third study we evaluate the extent to which object geometry and shadow shading affect depth judgments. In this final evaluation, we will analyze the best and worst stimuli for creating a sense of surface contact with an egocentric distance estimation protocol.


%In our second experiment, we use one of the simple geometries from our first study and compare ground contact perception between the object and the object when rotated. We also compare this simple geometry to a far more complex model (the Stanford dragon) and the complex model when rotated. %We hope to demonstrate that more complex 3D models are not necessarily easier to discern than basic primitives and that the effects observed in our first study are not due to the use of a single orientation. 

%Taken together, the first two studies should create a set of guidelines for how to create virtual objects to improve ground contact perception in XR. In our final study, we evaluate the best and worst conditions in an egocentric depth estimation task to understand the extent to which these factors affect depth perception. 





%  clearly, shadows are important
% we need to know what how the way we render graphics in XR affects our perception of space
% so in our current work we conduct a series of three perceptual studies

% Our first two studies take a psychophysical approach to evaluating one's perception of ground contact
% Explain psychophysics
% In the first study we look at object shape and shadow color. 

% In the second study we look at object orientation between a simple and a complex geometry. 

% Finally, in the third study we comiple the results of our prior research and evaluate the best and worst rendering solutions for creating a sense of ground contact. And we assess the extent to which they affect egocentric distance judgments 





% Below are a few questions that the experiments seek to answer:  

% Experiment 1 - Object Geometry -  Do non-photorealistic shadows benefit ground contact judgments in AR across different 3D geometries? Is it more difficult to discern ground contact for certain shapes? 

% Experiment 2 - Object Orientation -  Does the orientation of an object alter one’s perception of ground contact? Furthermore, is it easier for people to discern depth and ground contact for more complex shapes due to the presence of additional depth information (e.g., shading, self-occlusions)?
%
%Experiment 3 - Distance Perception - Does the manner in which a shadow is rendered affect egocentric distance estimates? How might shape affect distance perception in augmented reality? [[TBA]] 




\section{background on distance perception}
Within personal space, reaching paradigms have also been used to compare OST AR against VR displays. The results of this research are similarly difficult to interpret. Batmaz et al. \cite{Batmaz:2019:DHM} boldly asserted that any differences in depth perception between OST AR and VR displays did not adversely affect interaction after finding no significant differences in reaching behaviors between the Meta 2 and HTC Vive Pro in their study. Cidota et al. \cite{Cidota:2016:UVE} similarly found no significance in reaching behaviors when comparing OST AR and VR conditions with the AIRO II HMD, which supported both display modalities. However, Swan et al. \cite{Swan:2015:MRD} found that people overestimated the distance of virtual target objects in the nVisor ST60 OST AR display within personal space--a pattern that is typically not found in VR since VR HMDs induce distance compression. 

Even looking at depth perception studies in action space, which extends between 2 and 30 meters, we find irregular patterns in spatial perception. Using a blind walking paradigm, Jones et al. \cite{Jones:2011:PVI} found underestimation in OST AR (the nVisor ST)---but to a lesser extent than what had been found in VR. Pointon et al. \cite{Pointon:2018:JAC} found evidence of both over- and underestimation in their assessment of depth perception via affordance judgements in OST AR (the HoloLens 1), which they reported was likely due to the different spatial characteristics of the virtual objects. In their evaluation of video see-through displays via a pointer-matching (perceptual matching) protocol, Kyto et al. \cite{Kyto:2014:SDP} found evidence of distance underestimation. However, we must be cautious when extending the results of perceptual matching assessments to statements about egocentric depth perception. As Kyto et al. \cite{Kyto:2014:SDP} and Klein et al. \cite{Klein:2009:MPM} note, perceptual matching measures do not provide absolute measures of distance perception since they rely on relative, exocentric distance judgments to align two disparate targets in space. This judgement does not inherently require that egocentric distance be coded. 
 
Rosales et al. \cite{Rosales:2019:DJO} demonstrated that, in the absence of cast shadows, people perceive an object that is placed above the ground incorrectly as farther away,  \haley{which may account for some of the distance overestimation found in AR studies, since many AR distance estimation studies use floating objects? Food for thought.. }


  %It is interesting to note that many of the research studies that evaluate the effect of shadows in AR rely on visual matching paradigms and they evaluated geometries that float above ground. Both of these decisions have important ramifications for their experimental results. % Both Gao et al. \cite{Gao:2019:IVO} and  %Gao looks at off round hard edge and soft edge 
  
  %%% The Effects of Cast Shadows and Stereopsis on Performing Computer-Generated Spatial Task
  
  %%% Correlation between perception of color, shadows, and surface textures and the realism of a scene in virtual reality


%\haa{Remove. Save your rants for later, Haley! }
%The second factor to consider is that the majority of these studies utilize similar perceptual matching paradigms \cite{Berning:2014:SDP, Sugano:2003:ESR, Singh:2017:EFD, Diaz:2017:DDP, Gao:2019:IVO}. Because these protocols require people to align a virtual and real object that is, for convenience, typically placed on the ground---"drop shadows" allow participants to evaluate the distance between the real object and the virtual shadow (as opposed to the real object and the virtual object). This concern is also mentioned by Gao et al. \cite{Gao:2019:IVO}. Furthermore, many of these studies claim to evaluate egocentric depth perception, but because people are asked to align to objects in space---this paradigm is actually a measure of exocentric depth perception. 

  % Detached shadows are more forgiving --> Shadow shape has been demonstrated to make a difference for motor tasks \cite{Bonfiglioli:2004:DEC}
 
 %%Many depth perception studies in augmented reality utilize visual matching paradigms in which participants are asked to align virtual targets with markers in the real world---a paradigm which reflects exocentric distance judgments by evaluating the viewer's perceived distance between two objects: one real and one virtual.  Diaz et al. \cite{Diaz:2017:DDP} found that the presence of shadows improved visual matching performance, and even improved performance as much as 90\% in their drop shadow condition. 
 
 %%Gao et al. \cite{Gao:2019:IVO} similarly found that the presence of shadows improved visual matching judgements in OST AR, and they noted that shadow shape did not  



%%Distance perception in VR literature has benefited from many iterations of depth perception studies that use minor manipulations to equipment and that use agreed-upon egocentric distance estimation paradigms (e.g., verbal estimate, blind walking, and triangular blind walking). Distance perception studies in augmented reality are highly variable by comparison. In fact, one of the most popular 'egocentric distance' paradigms used in AR depth perception studies, perceptual matching, does not measure egocentric distance perception at all. Perceptual matching measures exocentric distance judgments, because viewers are required to align two disparate targets in space. This judgement does not inherently require that egocentric distance be coded. 







\section{Conclusions and Future Work} \label{conclusions}
\haa{This section is a little rough. Will revise when I have time.}
% Lights shadows did better
Over both experiments, we found that light shadows enhanced surface contact judgments in both AR devices. In VR, light shadows performed either similarly to or better than dark shadow conditions. When coupled with the findings of prior research by Adams et al. \haley{Adams:2021:SLC}, our current research provides strong evidence that non-photorealistic shading can enhance surface contact perception in XR. However, we found differences in shadow performance across displays. Stimuli in the OST AR display elicited distinctly different response patterns that indicate more sensitivity to color value intensity. This may be considered a reasonable outcome, given prior research by Singh et al. \cite{Singh:2017:EFD} which demonstrated that the brightness of a target affects distance perception in optical see-through device such that brighter virtual objects were perceived as closer to the viewer.


% Effects of shape & shadow shading
Given prior research by Thompson et al. \cite{Thompson:2004:DQC}, which demonstrated that quality of graphics had no effect on distance estimation in virtual environments, and the results of Adams et al. \haley{Adams:2021:SLC} \& Singh et al. \cite{Singh:2017:EFD}, we believe that our results were influenced more by object shading information than by resolution. Previously, Adams et al. \haley{Adams:2021:SLC} found that their non-photorealistic shadow shading condition, which also used light color values, improved surface contact perception across VST AR and VR devices when the target object was darkly shaded. And they found that light shadows improved ground contact perception in OST AR, regardless of the shading condition of the target object. Based on the findings of this research, we elected to use a medium gray color value to shade target object. However, despite differences in shading and object shape between the two studies, the trends of our current findings bear an uncanny resemblance to the findings of this prior research. 

% We did not change object shading
Because we were interested in cast shadow shading methods, we made a deliberate choice to only manipulate cast shadow shading. However, this may be considered a limitation since the object shading was not manipulated to be non-photorealistic to match the cast shadows. As a result, the light shadow naturally had more contrast against the target objects than the dark cast shadow. Now that the current research has established that surface contact perception is flexible enough to allow for non-photorealistic rendering techniques, it may be worthwhile to pursue more ambitious non-photorealistic 3D object shading techniques in future XR application development and research. 

% Shapes (Exp 1)
We found differences in surface contact judgments across all devices for object shape, which indicates that AR designers and researchers may want to carefully consider the shape of the objects used in their applications. In a similar line of research, Do et al. \cite{Do:2020:EOS} discovered that people's depth judgements to spheres were more sensitive to changes in luminance than other shapes. In Experiment 1, we found that the sphere consistently resulted in a lower likelihood of correct surface contact judgment in comparison to the rectilinear object across all devices. When taken together, both our results and Do et al. \cite{Do:2020:EOS}'s results provide a cautionary tale against the use of spheres for improving depth perception in XR.

% Shapes (Exp 2)
In our second experiment, we found shape $\times$ shadow interactions in which performance was dictated by object then by shadow shading condition for both VST AR and VR. In contrast, in OST AR performance was dictated by shadow shading condition then by object type. Our current findings indicate that OST AR is more sensitive to shading than either of the other XR displays---a finding that reflects a similar trend found in Adams et al. \haley{Adams:2021:CLS}. 


%\haa{orientation discussion}
Our results on orientation also have ramifications for the study and development of XR applications. Although motion parallax as a depth cue was provided in the current research, since head movements were not restrained, people were seated in a chair throughout the study and thus relatively still. It is likely that the effects of orientation would matter less if participants were allowed to maneuver around to object. However, we recognize that many applications for AR may rely on virtual images from which a person views from a limited perspective, for example, a virtual desktop. Although, we may progressively rotate a target object in XR to minimize the influence of orientation for a given depth perception study like in Peillard et al. \cite{Peillard:2019:SED}, we should also consider how to best anchor object in space without inducing additional movements since moving objects are not always desirable. 

%\haa{colorful shadows section}


From the findings of our two studies, we may begin to extrapolate XR developer and design guidelines. Bright color values are easier to see for people with low vision. If non photorealistic shading methods for shadows like those used here are not detrimental to depth perception, then they may provide a useful tool for enhancing visibility in AR for both normally-sighted and low vision users.  Even more colorful shadows, like those designed by Ooi et al. \cite{Ooi:2020:CCS} for AR, may also be a viable option. This opens up the realm for more stylized and more accessibility-driven graphics approaches in AR, since we need not be restrained by the need for consistent depth information between real and virtual environment in our AR displays. 


%Several research groups have evaluated both the automatic and reflective processes by which humans seem to infer information from shadows. 

%However, humans infer a variety of information from shadows beyond position, which is a more automatic cognitive process. And the 

% Ni et al \cite{Ni:2004:PSL}
% Mention shadows effects are task specific (Cavanaugh, Bonfiglioli) 

%\haa{non photorealistic rendering and depth perception. mention vaziri, too}

Pictorial cues may be especially beneficial for improving depth perception in AR, since they are somewhat device agnostic. Although the manner in which they are rendered may differ across all devices, they are nonetheless available across all devices.  However, we should note that not all non-photorealistic effects may not generally benefit depth perception in augmented reality, especially given the results of Cidota et al. \cite{Cidota:2016:UVE} which demonstrate that blur and fade may have adverse effects on action-based depth judgements in augmented reality in personal space. Pictorial cues are desirable to study as they provide a device agnostic solution for benefiting spatial perception across XR devices. Yet there are also other, binocular depth cues that need be improved for these devices to provide veridical perception. 


%In addition, hardware solutions and different optical solutions Cite Peillard:SED:2019. retinal projections, etc also beneficial. 

%%%Ahn et al 2019 \cite{Ahn:2019:SPA} compared handheld AR, VST AR, and OST AR. Significant effects of display type, rendering style, and viewing angle. E.g., VST AR most accurate and fastest size perception. Mobile display cause serious over-estimation. OST AR caused significant underestimation. oh my. %%% Scale / Size manipulation

In future research, it would be worthwhile to evaluate how non-photorealistic manipulations effect more direct measures of depth perception. Rosales et al. \cite{Rosales:2019:DJO} demonstrated that, in the absence of cast shadows, people perceive an object that is placed above the ground incorrectly as farther away. This may help explain some of the effects of overestimation found in prior AR depth perception research, especially given that most assessments use floating objects for assessment. In future work, we intend to evaluate how photorealistic and non-photorealistic shadows affect egocentric depth judgments in XR displays. 

%It may also be beneficial for researchers to enlist multiple methods of evaluating depth perception, since the underlying mechanisms guiding judgements of depth differ between passive and action-based tasks. Bonfiglioli et al. \cite{Bonfiglioli:2004:DEC}, for example, found that shadow shape influenced grasping to a target object but not object identification. 

%"Their experiment suggests that there is a task-dependent influence on cast shadows on human performance. In the case, of object-oriented actions, cast shadows may represent further affordances of the object, and as such compete for the control of the action "







\begin{table*}[htpb!]
\scriptsize
\centering 
\renewcommand{\arraystretch}{1.0} \setlength{\tabcolsep}{5pt}
\begin{tabularx}{\textwidth}{ l *{7}{l}}
    %\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} \\
         {\textbf{}} &Icosa LS &Icosa DS &Sph DS &Sph LS &Cube DS \\
        \toprule \\
         Cube LS    &$\beta=0.404$, $SE=0.185$	&$\beta=0.714$, $SE=0.178$ &$\beta=1.010$, $SE=0.174$	&$\beta=1.144$, $SE=0.172$	 &$\beta=1.446$, $SE=0.169$	\\ 
                    &$p=0.029*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\
         
         Icosa LS   &	 &$\beta=0.309$, $SE=0.165$	 &$\beta=0.606$, $SE=0.159$	 &$\beta=0.740$, $SE=0.158$ &$\beta=1.042$, $SE=0.154$	\\
                    &   &$p=0.060$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\
         
         Icosa DS   &	&	 &$\beta=0.297$, $SE=0.151$	 &$\beta=0.430$, $SE=0.149$ &$\beta=0.732$, $SE=0.146$	\\ 
                    &   &   &$p=0.050$ &$p=0.004*$ &$p<0.001^*$ \\
         
         Sphere DS  &	&	&	 &$\beta=0.134$, $SE=0.143$	 &$\beta=0.436$, $SE=0.140$	\\
                    &   &   &   &$p=0.351$ &$p=0.002^*$ \\
                        
         Sphere LS  &	&	&	&	 &$\beta=0.302$, $SE=0.138$	\\
                    &   &   &   &    &$p=0.028^*$ \\
         \hline \\
         
\end{tabularx}
\caption{Fixed effects of linear mixed model from first experiment}\label{tab:1}
\end{table*}








\begin{table}[htpb!]
\scriptsize
\centering 
\renewcommand{\arraystretch}{1.0} \setlength{\tabcolsep}{2pt}
\begin{tabularx}{\linewidth}{ l *{7}{l}}
         {\textbf{}} &Icosa LS &Icosa DS &Sph DS &Sph LS &Cube DS \\
        \toprule 
         Cube LS    &$\beta=0.404$	&$\beta=0.714$ &$\beta=1.010$ 	&$\beta=1.144$  &$\beta=1.446$	\\ 
                    &$p=0.029*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\ \\
         
         Icosa LS   &	 &$\beta=0.309$	 &$\beta=0.606$ &$\beta=0.740$ &$\beta=1.042$	\\
                    &   &$p=0.060$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\ \\
         
         Icosa DS   &	&	 &$\beta=0.297$ &$\beta=0.430$ &$\beta=0.732$ 	\\ 
                    &   &   &$p=0.050$ &$p=0.004*$ &$p<0.001^*$ \\ \\
         
         Sphere DS  &	&	&	 &$\beta=0.134$ 	 &$\beta=0.436$,  	\\
                    &   &   &   &$p=0.351$ &$p=0.002^*$ \\ \\
                        
         Sphere LS  &	&	&	&	 &$\beta=0.302$ 	\\
                    &   &   &   &    &$p=0.028^*$ \\ 
         \hline \\
         
\end{tabularx}
\caption{Fixed effects of linear mixed model from first experiment}\label{tab:2}
\end{table}















\begin{table*}[htpb!]
\centering 
\renewcommand{\arraystretch}{1.0} \setlength{\tabcolsep}{5pt}
\begin{tabularx}{\textwidth}{ l *{7}{l}}
    %\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} \\
         {\textbf{}} &Icosa LS &Icosa DS &Sph DS &Sph LS &Cube DS \\
        \toprule \\
         Cube LS    &$\beta=0.404$, $SE=0.185$	&$\beta=0.714$, $SE=0.178$ &$\beta=1.010$, $SE=0.174$	&$\beta=1.144$, $SE=0.172$	 &$\beta=1.446$, $SE=0.169$	\\ 
                    &$p=0.029*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\
         
         Icosa LS   &	 &$\beta=0.309$, $SE=0.165$	 &$\beta=0.606$, $SE=0.159$	 &$\beta=0.740$, $SE=0.158$ &$\beta=1.042$, $SE=0.154$	\\
                    &   &$p=0.060$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\
         
         Icosa DS   &	&	 &$\beta=0.297$, $SE=0.151$	 &$\beta=0.430$, $SE=0.149$ &$\beta=0.732$, $SE=0.146$	\\ 
                    &   &   &$p=0.050$ &$p=0.004*$ &$p<0.001^*$ \\
         
         Sphere DS  &	&	&	 &$\beta=0.134$, $SE=0.143$	 &$\beta=0.436$, $SE=0.140$	\\
                    &   &   &   &$p=0.351$ &$p=0.002^*$ \\
                        
         Sphere LS  &	&	&	&	 &$\beta=0.302$, $SE=0.138$	\\
                    &   &   &   &    &$p=0.028^*$ \\
         \hline \\
         
                  {\textbf{}} &Icosa LS &Icosa DS &Sph DS &Sph LS &Cube DS \\
        \toprule \\
         Cube LS    &$\beta=0.404$, $SE=0.185$	&$\beta=0.714$, $SE=0.178$ &$\beta=1.010$, $SE=0.174$	&$\beta=1.144$, $SE=0.172$	 &$\beta=1.446$, $SE=0.169$	\\ 
                    &$p=0.029*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\
         
         Icosa LS   &	 &$\beta=0.309$, $SE=0.165$	 &$\beta=0.606$, $SE=0.159$	 &$\beta=0.740$, $SE=0.158$ &$\beta=1.042$, $SE=0.154$	\\
                    &   &$p=0.060$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\
         
         Icosa DS   &	&	 &$\beta=0.297$, $SE=0.151$	 &$\beta=0.430$, $SE=0.149$ &$\beta=0.732$, $SE=0.146$	\\ 
                    &   &   &$p=0.050$ &$p=0.004*$ &$p<0.001^*$ \\
         
         Sphere DS  &	&	&	 &$\beta=0.134$, $SE=0.143$	 &$\beta=0.436$, $SE=0.140$	\\
                    &   &   &   &$p=0.351$ &$p=0.002^*$ \\
                        
         Sphere LS  &	&	&	&	 &$\beta=0.302$, $SE=0.138$	\\
                    &   &   &   &    &$p=0.028^*$ \\
         \hline \\
         
                  {\textbf{}} &Icosa LS &Icosa DS &Sph DS &Sph LS &Cube DS \\
        \toprule \\
         Cube LS    &$\beta=0.404$, $SE=0.185$	&$\beta=0.714$, $SE=0.178$ &$\beta=1.010$, $SE=0.174$	&$\beta=1.144$, $SE=0.172$	 &$\beta=1.446$, $SE=0.169$	\\ 
                    &$p=0.029*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\
         
         Icosa LS   &	 &$\beta=0.309$, $SE=0.165$	 &$\beta=0.606$, $SE=0.159$	 &$\beta=0.740$, $SE=0.158$ &$\beta=1.042$, $SE=0.154$	\\
                    &   &$p=0.060$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\
         
         Icosa DS   &	&	 &$\beta=0.297$, $SE=0.151$	 &$\beta=0.430$, $SE=0.149$ &$\beta=0.732$, $SE=0.146$	\\ 
                    &   &   &$p=0.050$ &$p=0.004*$ &$p<0.001^*$ \\
         
         Sphere DS  &	&	&	 &$\beta=0.134$, $SE=0.143$	 &$\beta=0.436$, $SE=0.140$	\\
                    &   &   &   &$p=0.351$ &$p=0.002^*$ \\
                        
         Sphere LS  &	&	&	&	 &$\beta=0.302$, $SE=0.138$	\\
                    &   &   &   &    &$p=0.028^*$ \\
         \hline \\
         
\end{tabularx}
\caption{Fixed effects of linear mixed model from first experiment}\label{tab:3}
\end{table*}








\begin{figure}[t]
    \centering
        \includegraphics[width=\linewidth, keepaspectratio]{fig/Rplot.png} 
        \caption{Experiment 1 OST AR Psychometric Curves}
        \label{fig:ostex}
\end{figure}

\begin{table}[t]
\scriptsize
\centering 
\renewcommand{\arraystretch}{1.0} \setlength{\tabcolsep}{2pt} 
\begin{tabularx}{\linewidth}{ l *{7}{l}}
         {\textbf{}} &\fcolorbox{yellow}{yellow}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Icosa LS &\fcolorbox{green}{green}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Icosa DS &\fcolorbox{red}{red}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Sph DS &\fcolorbox{magenta}{magenta}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Sph LS & \fcolorbox{blue}{blue}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Cube DS \\
        \toprule 
        
        \fcolorbox{orange}{orange}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Cube LS    &$\beta=0.404$	&$\beta=0.714$ &$\beta=1.010$ 	&$\beta=1.144$  &$\beta=1.446$	\\ 
         &$SE=0.029$ &$SE=0.001$ &$p=0.001$ &$SE=0.001$ &$SE=0.001$ \\
                    &$p=0.029*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\ \\
         
        \fcolorbox{yellow}{yellow}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Icosa LS   &	 &$\beta=0.309$	 &$\beta=0.606$ &$\beta=0.740$ &$\beta=1.042$	\\
                  &  &$SE=0.001$ &$p=0.001$ &$SE=0.001$ &$SE=0.001$ \\
                    &   &$p=0.060$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\ \\
         
        \fcolorbox{green}{green}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Icosa DS   &	&	 &$\beta=0.297$ &$\beta=0.430$ &$\beta=0.732$ 	\\ 
                  & & &$p=0.001$ &$SE=0.001$ &$SE=0.001$ \\
                    &   &   &$p=0.050$ &$p=0.004*$ &$p<0.001^*$ \\ \\
         
        \fcolorbox{red}{red}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Sphere DS  &	&	&	 &$\beta=0.134$ 	 &$\beta=0.436$,  	\\
                           & & &  &$SE=0.001$ &$SE=0.001$ \\
                    &   &   &   &$p=0.351$ &$p=0.002^*$ \\ \\
                        
        \fcolorbox{magenta}{magenta}{\rule{0pt}{6pt}\rule{6pt}{0pt}}\quad Sphere LS  &	&	&	&	 &$\beta=0.302$ 	\\
                         & & & &  &$SE=0.001$ \\
                    &   &   &   &    &$p=0.028^*$ \\ 
         \hline \\
         
\end{tabularx}
\caption{Fixed effects of linear mixed model from first experiment}\label{tab:2b}
\end{table}



\begin{table*}[ht]
\tiny
\centering 
\renewcommand{\arraystretch}{1.0} \setlength{\tabcolsep}{2pt} 
\begin{tabularx}{\linewidth}{ l *{9}{l}}
         {\multirow{1}{*}{\includegraphics[scale = 0.3]{fig/Rplot.png}}}  &&\fcolorbox{orange}{orange}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Cube LS &\fcolorbox{yellow}{yellow}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Icosa LS &\fcolorbox{green}{green}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Icosa DS &\fcolorbox{red}{red}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Sph DS &\fcolorbox{magenta}{magenta}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Sph LS & \fcolorbox{blue}{blue}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Cube DS    \\
        \toprule 
    
        
        &\fcolorbox{orange}{orange}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Cube LS    &&$\beta=0.404$	&$\beta=0.714$ &$\beta=1.010$ 	&$\beta=1.144$  &$\beta=1.446$	\\ 
         &&&$SE=0.029$ &$SE=0.001$ &$SE=0.001$ &$SE=0.001$ &$SE=0.001$ \\
                   &&&$p=0.029*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\ \\
         
        &\fcolorbox{yellow}{yellow}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Icosa LS   &&	 &$\beta=0.309$	 &$\beta=0.606$ &$\beta=0.740$ &$\beta=1.042$	\\
                  &&  &&$SE=0.001$ &$p=0.001$ &$SE=0.001$ &$SE=0.001$ \\
                    && &  &$p=0.060$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\ \\
         
        &\fcolorbox{green}{green}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Icosa DS   &&&	 &$\beta=0.297$ &$\beta=0.430$ &$\beta=0.732$ 	\\ 
                  &&&& &$p=0.001$ &$SE=0.001$ &$SE=0.001$ \\
                    &&&  &   &$p=0.050$ &$p=0.004*$ &$p<0.001^*$ \\ \\
         
        &\fcolorbox{red}{red}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Sphere DS  &&&	&	 &$\beta=0.134$ 	 &$\beta=0.436$  	\\
                           &&&& &  &$SE=0.001$ &$SE=0.001$ \\
                    &&&  &   &   &$p=0.351$ &$p=0.002^*$ \\ \\
                        
        &\fcolorbox{magenta}{magenta}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Sphere LS  &&&	&	&	 &$\beta=0.302$ 	\\
                         &&&& & &  &$SE=0.001$ \\
                    &&&&   &   &    &$p=0.028^*$ \\ 
                    
        & \fcolorbox{blue}{blue}{\rule{0pt}{3pt}\rule{3pt}{0pt}}\quad Cube DS    \\           \\         
         \hline \\
\end{tabularx}
\caption{Fixed effects of linear mixed model from first experiment}\label{tab:2b}
\end{table*}







\fboxsep=1mm 

\begin{table*}[ht]
\small
\centering 

\renewcommand{\arraystretch}{1.0} \setlength{\tabcolsep}{1pt} 
\begin{tabularx}{\linewidth}{ ll| *{8}{l}}
         {\multirow{1}{*}{\includegraphics[scale = 0.3]{fig/Rplot.png}}}  &&\fcolorbox{orange}{orange}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Cube LS &\fcolorbox{yellow}{yellow}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Icosa LS &\fcolorbox{green}{green}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Icosa DS &\fcolorbox{red}{red}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Sph DS &\fcolorbox{magenta}{magenta}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Sph LS & \fcolorbox{blue}{blue}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Cube DS    \\
         
        \cmidrule{3-8}
    
        &\fcolorbox{orange}{orange}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Cube LS   &&$\beta=0.404$	&$\beta=0.714$ &$\beta=1.010$ 	&$\beta=1.144$  &$\beta=1.446$	\\ 
                   &&&$p=0.029^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\ 
         
        &\fcolorbox{yellow}{yellow}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Icosa  LS  &$\beta=0.404$	 &&$\beta=0.309$	 &$\beta=0.606$ &$\beta=0.740$ &$\beta=1.042$	\\
                    &&$p=0.029^*$  &&$p=0.060$ &$p<0.001^*$ &$p<0.001^*$ &$p<0.001^*$ \\ 
         
        &\fcolorbox{green}{green}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Icosa  DS &$\beta=0.714$ &$\beta=0.309$	 &&$\beta=0.297$ &$\beta=0.430$ &$\beta=0.732$ 	\\
                    &&$p<0.001^*$ &$p=0.060$  &   &$p=0.050$ &$p=0.004^*$ &$p<0.001^*$ \\ 
         
        &\fcolorbox{red}{red}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Sphere DS   
        &$\beta=1.010$ &$\beta=0.606$ &$\beta=0.297$	&	 &$\beta=0.134$  &$\beta=0.436$ 	\\
                    & &$p<0.001^*$ &$p<0.001^*$  &$p=0.050$   &   &$p=0.351$ &$p=0.002^*$ \\ 
                        
        &\fcolorbox{magenta}{magenta}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Sphere LS &$\beta=1.144$ &$\beta=0.740$  &$\beta=0.430$	&$\beta=0.134$	&	 &$\beta=0.302$ 	\\
                    &&$p<0.001^*$ &$p<0.001^*$  &$p=0.004^*$   &$p=0.351$   &    &$p=0.028^*$ \\ 
                    
        & \fcolorbox{blue}{blue}{\rule{0pt}{1pt}\rule{1pt}{0pt}} Cube DS   
        &$\beta=1.446$ &$\beta=1.042$ &$\beta=0.732$ &$\beta=0.436$ &$\beta=0.302$ \\ 
        &&$p<0.001^*$ &$p<0.001^*$  &$p<0.001^*$ &$p=0.002^*$ &$p=0.028^*$  \\         
        \cmidrule{3-8} \\
         
\end{tabularx}
\caption{Fixed effects of linear mixed model from first experiment}\label{tab:2b}

\end{table*}


==> sections/9_deleted.tex <==




For illustration, Equation \ref{eq:3} represents the model used for each device in Experiment 1, where i represents a single observation. This means that any predictor with the subscript i indicates a variable that varies within participants. For each model, the regression finds coefficients ($\gamma_{ij}$) and an intercept $\mu$ that best fit the data for this binary outcome. The andom intercept ($\mu$) for each participant accounted for individual variability in surface contact judgments (i.e., the variability associated with repeated measures within each participant).


\begin{equation}
\begin{aligned}
    \mbox{ContactJudgment}_{i} &= \gamma_{00}  + \\
      & \gamma_{01}\times\mbox{Shadow}_{i} + \\ 
      & \gamma_{10}\times\mbox{Shape}(\textit{cube vs. ico})_{i} + \\ 
      & \gamma_{20}\times\mbox{Shape}(\textit{cube vs. sphere})_{i} + \\ 
      & \gamma_{30}\times\mbox{Shape}(\textit{ico vs. sphere})_{i} + \\ 
      & \gamma_{11}\times\mbox{Shadow}_i\times\mbox{Shape}(\textit{cube vs. cube})_{i} +\\
      & \gamma_{21}\times\mbox{Shadow}_i\times\mbox{Shape}(\textit{ico vs. ico})_{i} + \\
      & \gamma_{31}\times\mbox{Shadow}_i\times\mbox{Shape}(\textit{sphere vs. sphere})_{i} +\\
      & + \mu \\
\label{eq:3}
\end{aligned}
\end{equation}


Each variable was entered as a categorical factor with 2 or 3 levels. For Experiment 1 shape had 3 levels (cube,  icosahedron,  sphere), and shadow had 2 levels (dark \& light). We also specified interactions between shape and shadow  ($\gamma_{11}$, $\gamma_{21}$, $\gamma_{31}$).  Finally, contrast coding was used to allow for the planned comparisons.


==> sections/A1_psychophysics.tex <==









\section{Experiment 1: Shape and Shadow} \label{exp1}


In our first experiment, we evaluated how traditional (dark) and non-photorealistic (light) shading techniques for cast shadows affect one’s ability to perceive surface contact for a cube, an icosahedron, or a sphere (Figure \ref{fig:exp1_all}). These three objects were selected for their distinctive geometric properties.  In particular, the shape, shading, and shadows of the cube and sphere are recognizable and different. The icosahedron represents an in-between case, with its indistinct shape, but shading closer to that of the sphere and shadow closer to that of the cube. Our hypotheses for this experiment are as follows:
%However, the resulting shapes and defined edges of the three objects differ dramatically. The sphere consists of 400 surfaces to give a viewer the perception of curved lines. In contrast, the cube is a simple, rectilinear shape with only six surfaces. The icosahedron presents an in-between case, as it holds properties of both objects and consists of 20 surfaces.

\textbf{H1}: We predicted that people’s ability to correctly perceive ground contact would be affected by an object's geometry, especially along the bottom edge that would be in contact with a surface. Specifically, we anticipated that people's likelihood of correct response would be lower for the sphere across all devices.  A perfect sphere has only a single point of contact with a ground surface and that singular point is occluded when viewed from above. In contrast, both the icosahedron and the cube were flat along the edge and benefited from many points of contact with the surface beneath them, although the surface area of the bottom of the icosahedron was smaller than that of the cube.  

\textbf{H2}: We anticipated that people would be more likely to correctly perceive surface contact when presented with the light shadow shading method, in comparison to the traditional dark shading method in both AR devices. Although, our prediction may seem counterintuitive, some prior research has shown that non-photorealistic shadows may function as well as photorealistic shadows as a depth cue for spatial perception \cite{Kersten:1997:MCS,Adams:2021:SLC}. 

\textbf{H3}: We also anticipated that there would be interactions between shape and shadow shading methods. However, \emph{a priori} we were uncertain how these interactions would be expressed. 

% Because the spheres used in the current study were not textured, they appeared the same from different vantage points, which we anticipated would make it more difficult for viewers to leverage motion parallax as a depth cue \cite{DeLaMalla:2016:HVA, Powell:2012:VPV}. BB - I thought we explained this yesterday. This part of the hypothesis cannot possibly be correct as it misunderstands what motion parallax is. Motion parallax is the 2D optic flow generated by objects at different relative depths. This 2D flow is used by the visual system to reconstruct 3D structure. You will have a hard time explaining how 3D structure of an object influenced 2D optic flow.


\subsection{Participants}


Six individuals in total (3M, 3F) aged 23--30 volunteered to participate in our first experiment, which used a well-founded psychophysical paradigm. Psychophysics is a class of psychological methods that quantitatively measures perceptual responses to changes in physical stimuli \cite{Farell:1999:VRP}. These methods can use a small number of participants to make a large number of simple, behavioral responses that reveal underlying perceptual processes, gaining experimental power from a large number of observations. Psychophysical paradigms have proven highly replicable and robust since they employ judgments or adjustments with low individual variance \cite{Epstein:1980:SOB,Smith:2018:SIB}.   Psychophysics methods have previously been employed successfully by other XR research groups \cite{Bulthoff:2001:VAV,Schuetz:2019:EFL,Frankenstein:2020:APA}. 

All participants had normal or corrected to normal vision. Our experimental methods were approved by the local institutional review board, written consent was obtained from all subjects prior to participation, and each participant was paid 20 USD for 2-3 hours of their time.  


\begin{figure}[b]
    \centering
        \includegraphics[width=0.85\linewidth, keepaspectratio]{fig/WebsterA2.png} 
        \includegraphics[width=0.85\linewidth, keepaspectratio]{fig/VR_Geo12_Environment_Cropped.png}
        \caption{A participant views the experiment in the VST AR condition (top). An image of the virtual environment used for the VR condition (bottom). }
        \label{fig:participant}
\end{figure} 

\subsection{Design}

To address our hypotheses, we utilized a 3 (XR display) $\times$ 3 (target shape) $\times$ 2 (shadow shading)  $\times$ 6 (target height) within-subjects design to evaluate the effects of object shape and shadow shading on surface contact judgments for objects at different vertical displacements. Although we conducted our experiment with three different XR displays, we did not make any direct statistical comparisons across displays due to the high variance in optical and graphical properties across devices. However, we evaluated the same experimental conditions for each XR display. As such, this section describes the experimental design that was used for each XR device. 


%During the experiment, people were asked to make surface contact judgments for three different target object shapes (a cube, an icosahedron, and a sphere) that were rendered with either dark or light cast shadow shading. Dark shadows were rendered with a realistic, dark gray color value and light shadows were rendered with a non-photorealistic, off-white color value. In contrast, the target objects were rendered with a middle gray color value. Figure \ref{fig:exp1_all} displays all of the target shape and shadow shading conditions.   

Each participant evaluated 3  object shapes with 2 different shadow shading conditions,which resulted in 6 unique combinations of experimental stimuli. The target shapes evaluated were a cube, an icosahedron, and a sphere. The shadows were shaded with either dark or light color values. Figure \ref{fig:exp1_all} displays all of the target shape and shadow shading conditions. All targets were rendered on a table 1 meter in front of the viewer (Figure \ref{fig:participant}). The size of the targets was adjusted to be 11.2 cm wide. Accordingly, the cube had a length, width, and height of 11.2 cm, the sphere's diameter was 11.2 cm, and he icosahedron was scaled so that its width was approximately 11.2 cm. 

%After viewing each stimulus pair, the participant was asked which object was closer to the ground. The participant was forced to choose one of the targets as the target positioned closer to the surface beneath it.

We employed a temporal two-alternative forced choice paradigm with method of constant stimuli---a classic psychophysical method \cite{Farell:1999:VRP,Bogacz:2006:POD}---to evaluate people's perception of surface contact. Two-alternative forced choice, or 2AFC, is a method for assessing someone's sensitivity to a change in stimuli. It involves a \emph{forced choice}, because participants must chose between one of two options.  A temporal 2AFC paradigm may also be referred to as a two-interval forced choice (2IFC) paradigm. After viewing both stimuli in a sequence, participants in our experiment are then asked "Which object is closer to the ground?". Compared targets were always of the same shape and shadow condition for each trial. 

%It involves a \emph{forced choice}, because participants in a 2AFC experiment must chose between one of two options. They are not allowed to not answer. In a \emph{temporal} 2AFC design each option is presented in sequence. In the  current study, participants are shown two targets with different vertical displacements in a sequence. They are then asked "Which object is closer to the ground?". In our procedure, the two targets presented in a sequence were always of the same shape and shadow condition for each trial. 

How the six levels of vertical displacement were presented was dictated by \emph{method of constant stimuli}. As such, at least one of the target stimuli was always placed in contact with the surface beneath it. The other object was then displaced vertically by one of six heights between 0 and 6mm at regular intervals of $.06^{\circ}$ changes in viewing angle. When displacement was 0, both the first and second targets were positioned in contact with the surface. %The order in which vertically displaced targets was presented was random. 
%For method of constant stimuli, the order in which vertically displaced targets was presented was random. ---as opposed to in an ascending or descending order.


Changes in vertical displacement were subtle. All six height displacements are displayed in Figure \ref{fig:exp1_all}, and the calculations for vertical displacement are described in detail in Section \ref{method_vertical}. Each height comparison was presented 20 times each, except for when both the first and second object heights were equal (at 0). In this case, the height conditions were only presented 10 times each. Stimulus pairs were presented pseudo-randomly such that there were no repetitions of shape $\times$ shadow $\times$ height combinations before all combinations were presented once. In addition, the order of presented stimuli was balanced so that the number of trials in which the target was presented in contact with the ground first and the number of times it was presented second were equivalent for each condition.


Trials for the task were blocked by device and order of device was counterbalanced across subjects. For each XR device, a participant completed 660 2AFC trials. Each participant thus completed 1,980 trials total, and 11,880 data points were collected across all subjects. We collected data over a large number of trials, which is common practice in psychophysical paradigms, to increase accuracy and ensure low variance in our study \cite{Prins:2016:PPI}. By evaluating a large number of simple behavioral responses on a small number of participants, this family of paradigms is better able to evaluate perceptual behaviors that have little variance between individuals \cite{Epstein:1980:SOB,Smith:2018:SIB}.

We further confirmed that variance in our collected data was not due to between participant variance by calculating the intraclass correlation coefficient (ICC). The ICC measures the amount of variance accounted for by a grouping variable. For our analysis, individual participants was selected as the grouping variable, where an ICC value of 1 indicates  that  any  variance  in  the  data  is  between  participants  while  a  value  of  0  indicates  that  no  variance  in  the data is due to between participant factors. We found that $\tau_{ost}$ = .009 for data collected with the OST AR display, which indicated negligible variance was caused by between subjects factors. Similarly low ICC values were found for the VST AR  and VR display data with ICCs of $\tau_{vst}$ = .012 and $\tau_{vr}$ = .042, respectively. 

% HoloLens: [1] 0.009106272
% Zed:      [1] 0.01225212
% VR:       [1] 0.04157362







\subsection{Procedure}
%Before the participant entered the room, table surfaces and equipment were wiped down with disinfectant. If the participant arrived without a face mask, then they were given one upon arrival. The experimenter was also required to wear a mask and to maintain a 2 m distance from the volunteer. 

Before the experiment began, each individual was informed about the study and filled out a consent form. They were told that they may stop the experiment at any time and that they were allowed to take breaks during the experiment if needed. Both the experimenter and the volunteer wore face masks while maintaining 2 m of separation between each other during the experiment. 

Because the experiment was blocked by device, participants picked up one of the three designated XR HMDs and started up the system. They were then verbally instructed on how to interact with the system and they performed 10-20 practice trials that were randomly selected trials from the experiment. After the volunteer expressed that they were comfortable with the system and experimental paradigm, the experiment began. 

For the temporal 2AFC paradigm with method of constant stimuli, each  stimulus was presented for 600 ms. In between each stimulus pair, there was an interval of 800 ms in which a random pattern was presented at the position of the object to avoid visual aftereffects. After the presentation of each stimulus pair, the participant was asked ``Which stimulus is closer to the ground?''. They were told that at least one of the objects was positioned on the ground. They then responded using the left mouse button to indicate the first stimulus and the right button for the second stimulus.  The experiment was self-paced, and both the user’s response as well as their response time were recorded for each trial. The next trial began 1000 ms after the participant responded to the previous trial---unless the experiment was paused. After every 66 trials, participants were presented with a visual prompt that asked if they needed to take a break. 

Between devices, participants were also required to take a break to prevent fatigue. During the break, they filled out a brief survey that asked them to describe any strategies that they used to determine ground contact. After finishing the experiment in its entirety, they were asked to fill out a final survey. Although we did not directly compare peoples' performance across XR devices in this study, due to the high variance in display properties, in the final survey we asked participants about their experiences in each device. We believed this information would be informative for interpreting our results. Therefore, in the post experiment survey, they were asked to rank the difficulty of the experimental task for each device and to rank the displays' quality of graphics. They were also asked if their strategy for determining ground contact differed across devices.

%Between devices, participants were required to take a short break.  and they were asked to fill out a brief post survey which asked them to rate the difficulty of each condition and to describe what strategy they used to determine ground contact. \haa{For difficulty ratings, participants were asked, "How hard was it to determine which object was closer to the ground?" for each condition. They rated difficulty by assigning a Likert type number value between 1 and 5, where 1 indicated "very easy" and 5 indicated "very difficult".} After finishing the experiment in its entirety, they were also asked to fill out a final survey. In this survey, they were asked to rate the difficulty of the experimental task for each device and to rate the display's quality of graphics. They were also asked if their strategy for determining ground contact differed across devices. 


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth, keepaspectratio]{fig/study2_exp1_plotsC.png}
        \caption{
        Experiment 1 --- Response data from the 2AFC task was fit with cumulative logistic distributions using maximum likelihood to estimate parameters. The figure shows the psychometric curves for response data for the OST AR display (left), the VST AR display (middle), and the VR display (right) conditions. The psychometric curves display the probability of correct response for a given shape and shadow condition at each level of vertical displacement. Detection thresholds, also called points of subjective equality (PSE), equal the level of vertical displacement at which participants were able to discern that an object was placed above the ground. In a 2AFC experiment, detection thresholds correspond to 75\% probability of correct response. Detection thresholds are marked along the psychometric curve and their values are reported in Table \ref{tab:exp1_pse}. See Section \ref{exp1_results} for more details about the calculations behind the psychometric function and parameters.}
       \label{fig:exp1_pse_curves}
\end{figure*}


\subsection{Results} \label{exp1_results}


%Our analyses used the binomial mixed model approach described in Section \ref{method_analysis} in which we ran separate models for each of the three devices. 

%\haley{ We used a generalized linear model (GLM) to analyze participants' judgments. GLMs are a form of generalized regression that is appropriate for non-normally distributed outcomes and repeated-measures designs. In addition, generalized linear models provide the added advantage of model specification, which allowed us to include only the interactions that were hypothesized \emph{a priori}, thereby increasing our power to detect differences  \cite{Raudenbush:2002:HLM}. } 
%\holly{will need to update the above text to be consistent with binomial logistic regression (the current reference and explanation is for hierarchical (MLM) regression).}

%% \haley{Viola! Below is a more detailed description of the fitting process behind the psychometric curve and how the PSE was calculated from this. Typically, when people report PSEs they also include visualizations of the actual psychometric function used to calculate the PSE since it's where the value comes from. The PSE is basically a parameter estimated from the distribution. This is one of the big reasons that I think it is important to include figures with the distributions. }

\paragraph{Descriptive Statistics} 
\sarah{I think I get what you are trying to do here with the psychometric functions but I do not think they add anything to clarify the take home message because your analyses with the logit model are *much* easier to interpret. I think this descriptive statistics section (with figure 7 and table of PSEs is going to confuse the reader. If the curves are included, then you are going to need to interpret/explain why some conditions are so much flatter than others--less precision or more uncertainty--and we do not have a good answer for this. Also, currently you have not included any height interactions in the logit model and this would be the way to statistically make any claims that the slopes are different for the different conditions. I don't think we want to go there.)}
For each XR display, we also report the psychometric function and detection thresholds of our experimental conditions \cite{Knoblauch:2012:MPD,Kingdom:2016:PPI}. Psychometric data and thresholds were calculated by fitting cumulative logistic psychometric functions to participants' forced-choice judgements using the quickpsy package in R by Linares \& Lopez-Moliner~\cite{Linares:2016:QRP}. The parametric model and the estimation of its parameters used maximum likelihood, according to the following form: 

%\cite{Knoblauch:2012:MPD}

\begin{equation} \label{eq:psy}
\psi(x) = \gamma + (1 - \gamma - \lambda) * fun\left( x \right)  
\end{equation}


\begin{equation} \label{eq:psy_log}
fun(x)= \frac{1}{1+ e^{-\beta ( x-\alpha)}} 
\end{equation}

% alpha and beta are part of the vector of parameters
%mean and std deviation

% Prins 2012
% https://jov.arvojournals.org/article.aspx?articleid=2192299

% Good ExampleL
%https://www.frontiersin.org/articles/10.3389/fpsyg.2018.01250/full
%Finally, all models assume that the probability that an observer responds independently of the stimulus on any given trial (the lapse rate) equals 0.02. While this assumption is certain to be not exactly correct, data obtained in an experiment like this generally contain very little information regarding the value of the lapse parameter and for that reason, freeing it is problematic (Prins, 2012; Linares and López-Moliner, 2016). Note that in a task such as this, the rate at which an observer lapses determines both the lower and upper asymptote of the function. Thus, all models in Figure 1B assume that γ = λ = 0.02.

% Good theoretical explanation for lapse rate
% https://link.springer.com/article/10.3758/s13414-019-01706-7
% One should not free a parameter simply because one can. As noted, this is especially a concern with the lapse rate because of its redundancy with the PF's other parameters. Moreover, as has been shown before (Linares & López-Moliner, 2016; Prins, 2012), unless the design supports the estimation of a lapse rate (i.e., contains sufficient information regarding the value of the lapse rate), allowing the lapse rate to vary does little to improve bias in the parameters of interest.
% It should be stressed, however, that failing to allow at all for the occasional lapse in attention or finger error by utilizing a model that assumes a lapse rate of zero may lead to severe bias in location and slope parameters if a lapse does in fact occur

In Equation \ref{eq:psy},  $\gamma$ is the guess rate, $\lambda$ is the lapse rate and  $ fun\left( x \right) $ is a sigmoidal-shape, logarithmic function with asymptotes at 0 and 1. Because we employ a 2AFC paradigm, to fit the model we set $\gamma$ to chance level (guess = .5). \haley{To account for any lapse in attention or finger error from participants, we include the lapse rate, which is the probability that an observer responds independently of the stimulus on any given trial. Failing to allow for the lapse rate can lead to severe bias in location and slope parameters \cite{Prins:2012:PFL,Linares:2016:QRP}. A $\lambda$ of 0.02 was selected as a reasonable estimation of participants' lapse rate for the current experiments.} %since studies like the one  presented present very little information regarding the value of the lapse parameter}. 
%To account for any response lapses from participants, we do not fix $\lambda$, which corresponds to (1-$\gamma$) times the lapse rate~\cite{Kingdom:2016:PPI}, but estimate it as a parameter. 
Equation \ref{eq:psy_log} represents the logarithmic function where $\alpha$ is the scale parameter, also called the detection threshold or point of subjective equality (PSE). $\beta$ is the shape parameter, which corresponds to the standard deviation. 
%The scale parameter $\alpha$ corresponds to the point of subjective equality (PSE), which is the median of the distribution. Another name for $\alpha$ is the absolute detection threshold. It corresponds to the median of the distribution and corresponds to the vertical displacement measured by visual angle. 


%The parameter {\displaystyle \alpha >0}\alpha >0 is a scale parameter and is also the median of the distribution. The parameter {\displaystyle \beta >0}\beta >0 is a shape parameter.


The absolute detection threshold ($\alpha$) is the level of stimulus intensity at which someone is able to detect the stimulus. For 2AFC paradigms, this corresponds to the 75\% point on the psychometric curve, which is the median of the distribution. In our experiment, stimulus intensity corresponds to vertical displacement or height as measured by visual angle.  In Figure \ref{fig:exp1_pse_curves} this threshold is marked by a single point for each condition. The height values at the 75\% thresholds are also reported in Table~\ref{tab:exp1_pse}. Confidence intervals for thresholds were calculated via parametric bootstrapping with 1000 iterations.


Because the detection threshold is the height at which participants are able to reliably detect which target was placed on the ground, lower detection threshold values indicate better performance. 



\paragraph{Statistical Analyses} 
Participants were asked to make binary decisions about which object was positioned closer to the ground (first or second object) in a 2AFC task. Therefore, for our statistical analyses we used binary logistic regression models, which are appropriate for dichotomous outcome variables, to analyze participants' judgments. We used the glm function from the stats package in R \cite{Ihaka:1996:R} to conduct logistic regressions by specifying binomial errors and a logit link function. Because we wanted to analyze people's perception in each device, we ran separate models for each of the XR displays. For each display, we modeled binary outcomes (accuracy: correct (1) or incorrect (0)) for our predictors: object shape, shadow shading, and height. Height was recorded in millimeters then centered at zero and treated as continuous. Object shape (3 levels: cube, icosahedron, sphere) and shadow shading (2 levels: dark, light) were treated as categorical factors. Interactions between shape and shadow were included in the models.

We used these models to test three planned comparisons for each device to understand how object shape and shadow influenced people's surface contact judgments. These comparisons were: 1) whether surface contact judgments differed for different object geometries (i.e., \textbf{H1}~the main effect of object shape); 2) the difference in surface contact judgments between dark and light shadow shading across all other conditions (i.e., \textbf{H2} the main effect of shadow shading); and 3) interactions between object shape and shading (i.e., \textbf{H3}).



%\haley{We then tested three planned comparisons for each of these devices to understand how object shape and shadow shading influenced people's surface contact judgments.}
%\holly{We used these models \haley{this effect coded model?} to test three planned comparisons for each device to understand how object shape and shadow influenced people's surface contact judgments.} These comparisons were: 1) the difference in surface contact judgments between dark and light shadow shading across all other conditions (i.e., \textbf{H1} the main effect of shadow shading); 2) whether surface contact judgments differed for different object geometries (i.e., \textbf{H2} the main effect of object shape); and 3) interactions between object shape and shading (i.e., \textbf{H3}).


In order to examine whether there were main effects, we coded shadow and shape factors using deviation coding (also known as effect or sum coding). For the shape factor, the sphere was set as the reference group (i.e., coded as -1). For the shadow factor, the light shadow condition was coded as .5 and dark shadow was coded as -.5. Using this deviation coding also allowed us to observe whether there was a main effect of height. The general logistic regression equation is depicted in Equation \ref{eq:glm_model} below.

\begin{equation}
   \begin{split}
    \log\left(\frac{p}{1-p}\right) = B_0 & + B_1(\mbox{shadow}) + B_2(\mbox{cube}) \\ & + B_3(\mbox{icosahedron}) + B_4(\mbox{height}) \\
    & + B_5(\mbox{shadow} \times \mbox{cube}) \\
     & + B_6(\mbox{shadow} \times \mbox{icosahedron})
   \end{split} \label{eq:glm_model}
\end{equation}

For the shape variable (\textbf{H1}), we were interested in whether the sphere lead to lower accuracy than the other two shapes, collapsed across shadow and height. In order to answer this question, we conducted planned contrasts on the aforementioned model comparing each shape to one another, using the Bonferroni correction to account for multiple comparisons. 

In order to examine whether there was a main effect of shadow shading (\textbf{H2}), the shadow regression coefficient represents the difference between dark and light shadows averaging over shape and height. We were also interested in a potential interaction between shape and shadow (\textbf{H3}). Specifically, was each shape affected by the shadow shading? In order to answer this question, we calculated the shadow simple slopes for each shape. %\holly{We don't have to account for multiple comparisons here because we aren't comparing the slopes to one another - we're just comparing each one individually to 0.} 



%For the shape variable (\textbf{H2}), we were interested in whether the sphere lead to lower accuracy than the other two shapes, collapsed across shadow and height. In order to answer this question, we re-ran the logistic regression with shadow deviation coded (as in the full deviation coded model described above), but shape was dummy coded with sphere as the reference group (i.e., coded as 0 for both shape contrasts). Consequently, the coefficient for cube in this deviation-dummy coded model is the difference between the cube and sphere, collapsed across shadow and height. The coefficient for icosahedron is the difference between the icosahedron and sphere.

%We were also interested in a potential interaction between shape and shadow (\textbf{H3}). Specifically, was each shape affected by the shadow shading? In the deviation-dummy coded model, the coefficient for the shadow x cube interaction represents the difference between the effect of shadow on the cube and the effect of shadow on the sphere (i.e., whether the shadow slope for cube differs from the shadow slope for sphere). However, we were interested in the effect of shadow for each shape individually, rather than comparing the effect of shadow between shapes. As a result, we calculated the simple slopes from the deviation-dummy coded model, which compare the effect of shadow for each shape against 0.




For the sake of simplicity, we discuss the implications of our findings as well as which factors are significant in text, and we report the full details of the effects of factors in our analyses in Table \ref{tab:exp1_results}.






%\begin{equation} \label{eq:2}
%d_v = \left( \frac{ \tan(\sigma) \; {h_e} - d_{t}} {\tan(\sigma)} \right) 
%\end{equation} 


%$$\psi(x) = \gamma + (1 - \gamma - \lambda) * fun(x)$$
%$$fun(x) = 1 + exp(-p[2] * x-p[1])))^{-1}$$ 



%\haley{
%For each XR display, we report the detection thresholds, or points of subjective quality (PSEs) of our experimental conditions,  which were calculated via the psychometric function. We then present the results of our logistic regression and how these results answer our hypotheses. } 
%\holly{I think the PSE needs more explanation, but I saw your figure 8 comment, so I'm assuming that's still being worked out.}


%The results of the logistic regression for the OST AR display data are presented below, while the the psychometric curves and detection thresholds, or point of subjective equality (PSE)


%Object shape was dummy coded with sphere as the reference level since we predicted that perception of ground contact would be impaired by the lack of a flat edge. Shadow was dummy coded with dark as the reference level.



%\holly{For ease of interpretation, we report the unstandardized regression coefficients as odds ratios. Since we coded cube as the reference level for shape and dark as the reference level for shadow, and centered height, the regression coefficients have the following interpretations. B0, the model intercept, is the odds ratio for cubes with dark shadows presented at average height. B1 is the change in the odds between dark and light shadows for cubes presented at average height. B2 is the difference in the odds between the cube and icosahedron when they are presented with dark shadows at average height. B3 is the difference in the odds between the cube and sphere when they are presented with dark shadows at average height. B4 is the change in the odds for every 1mm increase in height, for cubes with dark shadows. B5 is the difference in shadow slopes between the cube and icosahedron, and B6 is the difference in shadow slopes between the cube and sphere. Although the regression coefficients of this model are based on the cube presented with dark shadows at average height, we can derive the odds for the other conditions by substituting values for the model predictors and doing simple arithmetic. The regression coefficients for each XR display are presented as odds ratios in Tables.... As exemplified by the above descriptions, due to the inclusion of the interaction, the main effects in our models are conditional effects. For example, the effect of shadow is conditional upon the level of shape (e.g., in our model, the shadow effect is conditional on using cube as the reference level for shape). As a result, we focus on the interpretations of the interactions in our results.} \holly{Need to format the betas with subscripts, but I'll wait to do that until we decide if we like this description or not.}


%We ran separate models for each of the three XR devices to understand how shadow shading and shape influenced people's surface contact judgments in each device. We then tested three planned comparisons for each device. These comparisons were: 1) the difference in surface contact judgments between dark and light shadow shading across all other conditions (i.e., \textbf{H1} the main effect of shadow shading); 2) whether surface contact judgments differed for different object geometries (i.e., \textbf{H2} the main effect of object shape); and 3) interactions between object shape and shading.

%Because participants in our study were asked to make binary decisions about which object was positioned closer to the ground (first or second object) in a 2AFC task, \haley{our GLMs were fitted by specifying binomial errors and a logit link function using the glm function in the lme4 library \cite{Bates:2010:LME4} in R \cite{Ihaka:1996:R}.} To be more specific, we modeled binary outcomes (correct or incorrect) for our input variables (predictors), which included object shape (3 levels: cube, icosahedron, sphere) and shadow shading (2 levels: dark, light). %All analyses were estimated with restricted maximum likelihood. %% <- Not needed for glm. only needed for glmm. 
 
%Our experimental variables (or predictors) were included at the within-subject level. Because all of our predictors were categorical, fixed effect estimates ($\beta$) represent the expected difference between each level of a variable. For our models, the expected difference was in the likelihood of correct response between variables. Because each of our analyses compared between levels of predictors, a negative fixed effect for $\beta$ indicated that the first level was more likely to result in a correct surface contact judgment in our 2AFC task. Positive effects effects for $\beta$ indicated that the second level was more likely to results in correct surface contact judgment.  % \sarah{I'm not sure you want to say it this way, because in the specific sections, you say for example, positive is more likely correct response for non-photorealistic and negative is photorealistic. So the pos/neg depends on the way that you code the variable. I'm suggesting take out this previous sentence altogether and just define the positive/negative direction in the subsections, but open to other ideas.} \haley{Took another stab at it. But I also agree that I need to remind readers what positive and negative effects mean in the next sections}
%\sarah{changed predictor to level in your description of the directions--does this make sense?} \haley{Yes!}
%Standard errors (\textit{SE}) represent the variance that surrounds each estimate, and \textit{p} indicates the probability of obtaining a difference in our sample if the null hypothesis is true. 

%To more accurately represent the statistical significance of our findings, we applied Bonferroni correction to our level of significance criterion (\textit{p}). Bonferroni correction is recommended for evaluations with multiple comparisons to compensate for an increased chance of Type I error. The significance level used for each analysis is included within the statistical reporting for each experimental finding. 
% For example, in our evaluation of the three object shapes when collapsed across all other conditions, the significance level was set at $p< \frac{0.05}{3} = 0.0167$.

\begin{comment}
\jeanine{I'm unclear as to why we are giving an example here for only one display type? Put all results in at same time. There's now maybe too much time spent discussing the analyses...} \haley{Failed attempt to make Results sound more 'tutorial'. Example removed}

 \sarah{this is not the degree to which estimates are different than 0--p values say nothing about the size or degree of the effect, but rather the probability of obtaining a difference in your sample if the null hypothesis is true (can you tell I am teaching research methods right now?).\haley{The things I would do to audit your class!} But I don't think you need to define this here at all--you already describe the bonferoni correction earlier.}  \haley{ Definition of p updated. Bonferroni content removed }. 




%Cohen’s \textit{d} is also reported, which indicates the size of the effects we observed. 
\haley{OKAY. Bobby, after looking into Cohen's D, Odds Ratios, and SIMR analysis I don't actually think we should report a post hoc power analysis. Post hoc power analyses are apparently misleading and inaccurate, especially for mixed models. That may also explain why none of the papers with GLMMs that I've read include post hoc power analyses. But I'll keep the reported Odds ratios for now..} \bbc{You should not report a post-hoc power analysis. However, when you designed these experiments, didn't you do a power analysis at all? How did you determine that 6 subjects, etc., was going to be enough? I recall us going over this several times in the design of the studies.} \haley{Oh my. That was so long ago. I vaguely recall running some analyses with G Power back then, but I'm not confident that I could replicate that test exactly now. Also, if I had a saved output from that, then it's probably gone. I reinstalled the OS on my laptop a couple months ago.  On the other hand, I remember (and have notes) from prior research studies and their N. The bigger issue was not the number of people (N=6 was standard if not slightly above average in the psychophysics studies I surveyed) but the number of repetitions. That's where I got 20 repetitions. 20 was as low as you could go to get reliable results---If I recall correctly. I have papers that I could cite for that claim, if desired.}

 \sarah{I'm now thinking that you don't need equation 3. I think it is confusing and I'm not sure totally correct--what does cube vs. cube mean?). I looked back at our other VR conference papers and sometimes we just explain the predictors in words, which I think is what we want to do here.} \haley{Oh thank goodness. The equation just makes it more confusing imo. EQ 3 and its discussion have been removed}
\end{comment}


\begin{comment}
For illustration, Equation \ref{eq:3} represents the model used for each device in Experiment 1, where i represents a single observation. This means that any predictor with the subscript i indicates a variable that varies within participants. For each model, the regression finds coefficients ($\gamma_{ij}$) and an intercept $\mu$ that best fit the data for this binary outcome. The andom intercept ($\mu$) for each participant accounted for individual variability in surface contact judgments (i.e., the variability associated with repeated measures within each participant).


\begin{equation}
\begin{aligned}
    \mbox{ContactJudgment}_{i} &= \gamma_{00}  + \\
      & \gamma_{01}\times\mbox{Shadow}_{i} + \\ 
      & \gamma_{10}\times\mbox{Shape}(\textit{cube vs. ico})_{i} + \\ 
      & \gamma_{20}\times\mbox{Shape}(\textit{cube vs. sphere})_{i} + \\ 
      & \gamma_{30}\times\mbox{Shape}(\textit{ico vs. sphere})_{i} + \\ 
      & \gamma_{11}\times\mbox{Shadow}_i\times\mbox{Shape}(\textit{cube vs. cube})_{i} +\\
      & \gamma_{21}\times\mbox{Shadow}_i\times\mbox{Shape}(\textit{ico vs. ico})_{i} + \\
      & \gamma_{31}\times\mbox{Shadow}_i\times\mbox{Shape}(\textit{sphere vs. sphere})_{i} +\\
      & + \mu \\
\label{eq:3}
\end{aligned}
\end{equation}


Each variable was entered as a categorical factor with 2 or 3 levels. For Experiment 1 shape had 3 levels (cube,  icosahedron,  sphere), and shadow had 2 levels (dark \& light). We also specified interactions between shape and shadow  ($\gamma_{11}$, $\gamma_{21}$, $\gamma_{31}$).  Finally, contrast coding was used to allow for the planned comparisons. 
\end{comment}





%The absolute detection thresholds, or points of subjective equality (PSE), for the dark and light shadow conditions for each shape (cube, dragon). In our experiment, thresholds equal the level of vertical displacement at which participants were able to discern that an object was placed above the ground. 

\begin{comment}
\begin{figure*}[ht] 
        \centering 
        \includegraphics[width=\linewidth,keepaspectratio]{fig/study2_exp1_bars_lapses.png}  
        \caption{ Experiment 1 --- Detection thresholds, also called points of subjective equality (PSE), are shown for the OST AR display (left), the VST AR display (middle), and the VR display (right) conditions. In our experiment, thresholds equal the level of vertical displacement at which participants were able to discern that an object was placed above the ground. 
        PSE thresholds correspond to 75\% probability of correct response as specified by the psychometric functions displayed in Figure \ref{fig:exp1_pse_curves}. 
        Error bars show  95 \% confidence intervals.
        For each display, we report the absolute detection thresholds for every shape and shadow condition. 
        For visual reference, the statistical significance for our evaluations of H3 (interactions between shape and shadow) at p $<$ .05 are noted by (*). }       
        \label{fig:exp1_bars}
\end{figure*}
\end{comment}









\subsubsection{Optical See-through AR}


The psychometric curves and detection thresholds for each shape and shadow condition tested are reported in Figure \ref{fig:exp1_pse_curves} (left) and Table \ref{tab:exp1_pse}, respectively. The results of our statistical analyses are reported in Table \ref{tab:exp1_results}. In our experiment, we expected participants to be more likely to correctly indicate which object was on the ground as the height of target objects increased. This trend can be seen in the positive slope of the psychometric functions in Figure \ref{fig:exp1_pse_curves}. The improvement of participants' performance as height increased is further demonstrated statistically by a main effect of height in our logistic regression model ($OR = 1.09$, $p < .001$). An odds ratio ($OR$) of 1.09 indicates that for every 1mm increase in height, the odds of correctly stating which object was closer to the ground increased by a factor of 1.09. \sarah{the beginning of this paragraph is confusing because it is not clear what the psychometric curves and PSE are giving us and the discussion is interleaved with the statistical analyses that were not done on the PSEs. My suggestion is to delete the descriptive curves and revise to the following:}

The results of our statistical analyses are reported in Table \ref{tab:exp1_results}. We expected participants to be more likely to correctly indicate which object was on the ground as the height of target objects increased. The improvement of participants' performance as height increased is demonstrated statistically by a main effect of height in our logistic regression model ($OR = 1.09$, $p < .001$). Collapsed across all shape and shadow conditions, the odds ratio ($OR$) of 1.09 indicates that for every 1mm increase in height, the odds of correctly stating which object was closer to the ground increased by a factor of 1.09.



\paragraph{H1: Does object shape matter?}

The sphere was the least likely shape to elicit correct responses. In our paired comparisons of people's accuracy for each target shape, when collapsed across shadow and height, we found that people's accuracy when they were shown the sphere was significantly worse than when their accuracy when shown shown the cube ($OR = 1.42$, $p < .01$) or the icosahedron ($OR = 1.67$, $p < .001$). \sarah{In other words, participants were 1.42 times or 1.67 times more likely to choose the correct object with the cube or icosahedron, respectively, than with the sphere.} There was not a significant difference in response accuracy between the cube and icosahedron ($OR = .85$, $p = .50$).

\paragraph{H2: Does shadow shading method matter?} 
The main effect for shadow ($OR = 1.71$, $p < .001$) indicates that a correct response was 1.71 times more likely when the object was presented with a light shadow compared to a dark shadow. 


\paragraph{H3: Is there an interaction between shape and shadow?} 
Analysis of the shadow by shape simple slopes indicated that the effect of shadow was only significant for the cube ($OR = 4.21$, $p < .001$). 


\input{tables/_Exp1_PSE_Table}


\subsubsection{Video See-through AR}


The detection thresholds for our experimental conditions are reported in Table~\ref{tab:exp1_pse} while the complete psychometric curves are shown in Figure~\ref{fig:exp1_pse_curves} (middle). The results of our statistical analyses are reported in Table~\ref{tab:exp1_results}. For VST AR we again found a main effect of height ($OR = 1.07$, $p < .001$), which is also illustrated by the positive slopes of the psychometric curves in Figure~~\ref{fig:exp1_pse_curves}. Accordingly, as the height of the vertically displaced object increased, participants were more likely to correctly indicate which object was on the ground. 

\paragraph{H1: Does object shape matter?}
People were most likely to produce a correct response when presented with the cube, and they were least likely to make a correct response when presented with a sphere. Planned contrasts for the shape variable indicated that the odds of providing a correct response significantly differed between all shape comparisons. The cube was more likely to yield a correct response than either the sphere ($OR = 4.90$, $p < .001$) or the icosahedron  ($OR = 2.93$, $p < .001$). And the odds of providing a correct response for the icosahedron was higher than the odds for the sphere ($OR = 1.67$, $p < .001$). 

\paragraph{H2: Does shadow shading method matter?} 
The main effect for shadow ($OR = 2.28$, $p < .001$) indicates that a correct response was 2.28 times more likely when the object was presented with a light shadow compared to a dark shadow.



\paragraph{H3: Is there an interaction between shape and shadow?} 
Analysis of the shadow by shape simple slopes indicated that the effect of shadow was significant for all three shapes. That is, the probability of providing a correct response was higher when a light shadow was presented regardless of whether the object presented was a sphere ($OR = 1.38$, $p < .05$), a cube ($OR = 2.40$, $p < .001$), or an icosahedron ($OR = 3.58$, $p < .001$). \sarah{I think you need a reference to figure 8 here and at the other H3 sections} 

%\haley{The detection thresholds for the sphere were PSE = 0.14, CI = $[0.09, 0.18]$ and PSE = 0.19, CI = $[0.14, 0.24]$ for the light and dark shadow, respectively. For the icosahedron the light and dark shadow detection thresholds were PSE = 0.06, CI = $[0.04, 0.08]$ and PSE = 0.16, CI = $[0.12, 0.20]$. For the cube the light and dark shadow thresholds were PSE = 0.05, CI = $[0.01, 0.05]$ and PSE = 0.08, CI = $[0.06, 0.09]$.}



\input{tables/_Exp1_Tables}


\begin{figure*}[b]
    \centering
    \includegraphics[width=\linewidth, keepaspectratio]{fig/_Simple_Slopes_Geo1d.png}
        \caption{
        Experiment 1 --- Predicted probability of correct response for shape (cube, icosahedron, sphere) and shadow (dark, light) interactions  with 95\% confidence }
       \label{fig:exp1_slopes}
\end{figure*}



\subsubsection{Virtual Reality}


The psychometric curves for our experimental conditions are shown in Figure~\ref{fig:exp1_pse_curves} (right) and the corresponding detection thresholds are reported in Table~\ref{tab:exp1_pse}. The results of our statistical analyses are reported in Table~\ref{tab:exp1_results}. For VR we found a main effect of height ($OR = 1.06$, $p < .001$) such that for every 1mm increase in height, the odds of correctly stating which object was closer to the ground increased by a factor of 1.06.The psychometric curves in Figure~\ref{fig:exp1_pse_curves} also illustrate that participants became more likely to correctly indicate which object was placed on the ground as the height of the vertically displaced objects increased. 

\paragraph{H1: Does object shape matter?} 
People were most likely to make a correct response when presented with the cube, and they were least likely to make a correct response when presented with the icosahedron. The probability of providing a correct response significantly differed for all shape comparisons. Specifically, planned contrasts, when collapsed across shadow and height, showed that participants were more likely to make a correct response when presented with the cube than the icosahedron ($OR = 8.20$, $p < .001$) or sphere ($OR = 5.95$, $p < .001$). They were then more likely to make a correct response given the sphere over the icosahedron ($OR = .73$, $p < .01$). 

\paragraph{H2: Does shadow shading method matter?} 
The main effect for shadow was not significant ($OR = 1.23$, $p = .07$), suggesting that, averaged across shape and height, shadow shading did not have a significant effect on judgments of ground contact in virtual reality.


%Collapsed across shadow and height, the odds of providing a correct response increased by a factor of 5.95 when the cube was presented compared to the sphere (\textit{B} = 1.78, \textit{SE} = 0.16, odds ratio = 5.95, $p <$ 0.001). The odds of providing a correct response decreased by a factor of 0.73 when the icosahedron was presented compared to the sphere (\textit{B} = -0.32, \textit{SE} = 0.10, odds ratio = 0.73, $p <$ 0.01). Additionally, the cube was more likely to yield a correct response compared to the icosahedron (\textit{B} = 2.10, \textit{SE} = 0.16, odds ratio = 8.20, $p <$ 0.001). \haley{Overall, the icosahedron was the least likely to produce a correct response (PSE = 0.17, CI = $[0.14, 0.21]$), followed by the sphere (PSE = 0.13, CI = $[0.11, 0.16]$), then the cube (PSE = 0.05, CI = $[0.03], 0.06$).}  

%Overall, the icosahedron was the least likely to produce a correct response (\textit{M}\textsubscript{probability} = 0.74, \textit{SE} = 0.01), followed by the sphere (\textit{M}\textsubscript{probability} = 0.80, \textit{SE} = 0.01), then the cube (\textit{M}\textsubscript{probability} = 0.96, \textit{SE} = 0.01).

%cube   0.05 [0.03, 0.05]
% ico   0.17 [0.14, 0.21]    
% sph   0.13 [0.11, 0.16]

\paragraph{H3: Is there an interaction between shape and shadow?} 
Analysis of the shadow by shape simple slopes indicated that the effect of shadow was only significant for the sphere ($OR = 1.43$, $p < .05$). 

%0.154	0.12	0.189
%0.117	0.088	0.143


%%%\subsubsection{Does shadow shading method matter?}
%%%Therefore, we can say that people in our experiment were 0.493 times as likely to correctly determine ground contact in OST AR when the shadow was light in comparison to when the shadow was dark. 

%%%To test the influence of shadow shading method on surface contact judgments in XR  we evaluated the two shadow shading methods (dark and light) when collapsed across all other conditions  for each device. The resulting fixed effects estimates ($\beta$), standard errors (Std. Error), and significance values (\textit{p}) are displayed in Tables \ref{tab:exp1_ost}-\ref{tab:exp1_vr} for each XR display. The \textit{Shadow (dark vs. light)} variable provides insight into the current research question, where negative fixed effects indicate that people were more likely to correctly interpret surface contact for dark shadows, and positive effects indicate that people were more likely to correctly interpret surface contact for light shadows. No Bonferroni correction was applied to this analysis since only one comparison was made. Therefore, the significance value remained \textit{p}$<0.05$. 

%%%\paragraph{OST AR: } Non-photorealistic, light shadows resulted in an increased likelihood of correct response in comparison to photorealistic, dark shadows in both the OST AR (Table \ref{tab:exp1_ost}) and the VST AR devices (Table \ref{tab:exp1_vst}). 

%%%\paragraph {VR: }For VR, there was no significant difference in responses between light and dark shadows  (Table \ref{tab:exp1_vr}). These findings confirmed our first hypothesis (\textbf{H1}), in which we predicted that the light cast shadow methods would enhance ground contact perception in both AR devices. It was also promising that people performed similarly when presented with light and dark shadows in VR---an indication that there were no adverse effects to surface contact judgments from light rendering of cast shadow.  





%%Non-photorealistic, white shadows resulted in an increased likelihood of correct response in comparison against photorealistic, dark shadows over all devices when collapsed ($\beta = 0.450 , SE= 0.052, p<0.0001$).

%%This analysis was performed for each device, and the Bonferroni corrected significance level was set to $p<0.0167$.

%%%\subsubsection{Does object shape matter?} \label{exp1_h2_results}
%\haley{Cube no longer outperforms sphere in OST AR for HoloLens after Bonferroni correction} \sarah{you do not need to do bonferroni correction here if you do planned orthogonal contrasts. I thought that is what you had done before. E.g., compare each of the other two shapes(ico and sphere) to cube. If you want to compare each shape to each other, then you do need to correct for multiple comparisons.} 

%%%To understand whether object shape influenced surface contact judgments in XR, we evaluated the three object shapes (cube, icosahedron, and sphere) when collapsed across all other conditions. For each display the results of these analyses can be seen in Tables \ref{tab:exp1_ost}--\ref{tab:exp1_vr}, where \textit{Shape(cube vs. ico)}, \textit{Shape(cube vs. sphere)}, and \textit{Shape(ico vs. sphere)} are the relevant variables for our research question. Negative fixed effect estimates ($\beta$) indicate that the first object in the comparison is more likely to receive a correct surface contact judgment. Positive effects indicate that the second object in the comparison is more likely. The Bonferroni corrected significance value for these comparisons was $p<0.0167=0.05/3$.

%%%We found support for \textbf{H2}, which predicted that an object's geometry would affect surface contact perception. We argued that specific shape properties, such as the presence of straight edges or curved lines along the bottom of an object, would be pertinent to judgments of surface contact. We found that participants were more accurate in determining surface contact with the cube than the sphere in both VST AR and VR and that they were more accurate with the icosahedron than the sphere in VST AR and OST AR (Tables \ref{tab:exp1_ost}-\ref{tab:exp1_vr}).  People's perception of surface contact with the icosahedron varied in effectiveness, which may have been expected since the icosahedron---an approximation for a sphere with similar rectilinear properties to a cube---presented an intermediate case for study. Specifically, people performed best when judging the icosahedron in comparison to all other shapes in OST AR (Table \ref{tab:exp1_ost}), and they were worst when judging the icosahedron in comparison to all other shapes in VR (Table \ref{tab:exp1_vr}). In VST AR, the icosahedron resulted in better performance than the sphere but worse than the cube (Table \ref{tab:exp1_vst}).

%\sarah{related to my comment above, you have not specified how the shape comparisons were coded (0,1) so it is difficult to determine the direction of the effects based on positive or negative betas. I noticed this especially when I was trying to interpret what your "median performance" ico really means. Is there are straightforward way to communicate this?}\bbc{Agree with Sarah here. There is no way to verify your interpretations without knowing this. For example, isn't it true that people were significantly more accurate with the sphere than the icosahedron in VR?} 


%In detail, within the OST display, the icosahedron outperformed both the cube ($\beta = 0.289 , SE= 0.111, p=0.009$)  and sphere ($\beta$ ~\textdblhyphen~ $ 0.510 , SE= 0.109, p<0.0001$), and the cube outperformed the sphere ($\beta = 0.221 , SE= 0.104, p=0.034$). In the VST display, the cube outperformed both the icosahedron ($\beta = 1.120 , SE= 0.136, p<0.0001$) and sphere ($\beta  = 1.527 , SE= 0.132, p<0.0001$), and the icosahedron outperformed the sphere ($\beta$ ~\textdblhyphen~ $ 0.406 , SE= 0.103, p<0.0001$). In VR, the cube outperformed the sphere ($\beta  = 1.821 , SE= 0.156, p<0.0001$) and the icosahedron ($\beta$ ~\textdblhyphen~ $ 2.144 , SE= 0.156, p<0.0001$), but the sphere outperformed the icosahedron ($\beta  = 0.323 , SE= 0.099, p=0.001$). 

%Instead, we argued that the number of points of contact an object had with the ground surface would have a more dramatic effect such that we could expect the sphere (with a single, occluded point of contact) to perform worse than the cube (with many points of contact). Furthermore, we expected this relationship to hold across all devices. 

%%Collapsing over all devices, we found a significant trend for the accuracy of ground contact perception where: cube > icosahedron > sphere. The cube resulted in the highest likelihood of correct response in comparison to the icosahedron ($\beta = 0.823 , SE= 0.070, p<0.0001$) and the sphere ($\beta = 0.995 , SE= 0.069, p<0.0001$). And the icosahedron outperformed the sphere ($\beta = 0.995 , SE= 0.069, p<0.0001$). 


%%%\subsubsection{Is there an interaction between shape and shadow?}

%%%\emph{A priori}, we anticipated that there would be interactions between shape and shadow; however, we were uncertain how these interactions would be expressed. We were most interested in whether the advantage for non-photorealistic (light) shadows was consistent across the different shapes. This led us to conduct 3 unique, paired comparisons for shape $\times$ shadow conditions for each device, where the relevant variables for our research question included: \textit{Shadow$\times$Shape (cube: dark vs. light)},  \textit{Shadow$\times$Shape (ico: dark vs. light)},  and \textit{Shadow$\times$Shape (sphere: dark vs. light)}.  In a similar manner to the previous analysis, negative fixed effects for $\beta$ indicated that the first object in the comparison was more likely to elicit a correct response, whereas positive effects indicated the second object. Because three comparisons were made, the Bonferroni corrected significance value for these comparisons was $p<0.0167$.   %\sarah{have you defined DS and LS? Sometimes you use Dark vs. Light and but more often photorealistic vs. non-photorealistic when you describe these levels, so think about what is the best way to abbreviate, but either way it should be defined} %I decided to just use "dark vs light" for simplicity, even in the table
%\sarah{this is not 6 comparisons, it is 3--dark vs. light shadow for each of 3 shapes} \haley{ahhhhhhhh don't look at me i'm ashamed}


%%%For the OST display (Table \ref{tab:exp1_ost}), the analysis indicates that the fixed effects between light and dark shadow conditions did not significantly differ for the icosahedron, nor did they differ for the sphere. However people were more likely to make correct surface contact judgments with the light shadow than the dark shadow when presented with a cube. In contrast, for the VST display (Table \ref{tab:exp1_vst}) people's surface contact judgments were significantly better for all objects when the object was presented with a light cast shadow. In VR (Table \ref{tab:exp1_vr}), people were more accurate when presented with the light shadow when the object was a sphere, but differences in shadow shading did not significantly affect people's performance given the cube or the icosahedron. %\sarah{this is a good description of the effects--RE my comment above, you are using light and dark consistently here, and not non-photo and photorealistic} 
%%%In sum, across all devices and all objects, the light shadow condition always performs similarly to or better than the dark shadow condition, but the degree of this benefit is contingent upon object shape. %\jeanine{I sort of like the light and dark distinction better than photorealistic vs. non, but up to you all. It just makes it easier to understand which shadow is which in real time as you're reading.}\bbc{I agree with this, but there is inconsistency in the paper on this point. It will have to be fixed.} \haley{Absolutely agreed}

%Furthermore, participants performed significantly better when given the cube with the light shadow than they performed for all other conditions. And they performed worse when given the cube with the dark shadow than they did for all other conditions.  
%For the Microsoft HoloLens, the dramatic difference in performance between light and dark shadows in the cube condition indicates that there is a strong interaction of shape and shadow when a rectilinear shape is viewed in OST AR. It also demonstrates why the icosahedron outperforms the cube when we collapse across shadow conditions. 

%\sarah{your text is clear for these interactions, but I think the tables are somewhat confusing. I think what we care most about are the comparisons that you describe--does light vs. dark differ for each shape? So, the other comparisons in the table are distracting and also not motivated clearly. If you want to leave these in, I think more is needed in the caption and/or text to help the reader interpret.}




\subsubsection{How difficult was each condition?}
%To better understand how participants interpreted each experimental stimuli, they were asked both multiple choice and open-ended questions about the experiment. 
%For each device, they assigned a rank of easiest, middle, or hardest for difficulty; and they assigned a rank of best, middle, or worst for graphics quality.
 
We examined post-experiment survey responses to better understand how participants interpreted our experimental stimuli.  Participants were asked to rank the devices from easiest to hardest for determining ground contact, and they were asked to rank devices on graphics quality from lowest to highest. For difficulty rankings, they assigned each XR display to one of three categories: easiest, middle, or hardest. For quality of graphics rankings, they assigned each display to best, middle, or worst. 

There was no clear easiest display, given that all three XR devices were rated as the easiest display by two out of six (2/6) participants. However, the AR devices were seen as more difficult than the VR condition, with both the OST AR display (4/6) and the VST AR display (2/6) receiving ratings for being the most difficult display. Participants also stated that the video see-through display had the lowest perceived quality of graphics with three out of six (3/6) worst votes and 3/6 median votes,  and that the optical see-through display had the highest quality graphics (5/6). %\bbc{Make a note: For your proposal and dissertation, a bar chart with color for each of the rankings would elucidate these findings really well. Here, I think it makes more of them than we probably want to, given the space limitations.} \haley{Hopefully, I'll do something even better than a bar chart for the proposal! You know how I feel about bar charts haha}

%\haley{Hopefully, it's more clear now}\sarah{not totally clear what these numeric values mean--is it 5 out of 6 rated as highest quality?. What was the actual measurement on the survey?}

Peoples' reported strategies in the post-experiment survey support the idea that the curved lines of the sphere and its shadow increased the difficulty of discerning surface contact. For discussion, we will refer to each participant with an acronym (e.g., P1 for the first participant).  P1, P3, and P4 reported looking at shadows ``\textit{beneath}" the objects or ``\textit{beneath the front side}" of objects. P3 also commented that they tried to remember the point of optical contact for a given object. P2 and P5 explicitly stated that they looked for the ``\textit{edges}" of shadows to make judgments. A reliance on shadow edges would also explain why people's responses for the sphere were generally less accurate, regardless of XR display. Participants reported that they employed the same strategies for discerning ground contact across devices. 




\subsection{Discussion}


In our first experiment, we found that light shadows improved ground contact judgments compared to dark shadows for both AR devices and that they performed comparably to dark shadows in VR. These results encourage the use of non-photorealistic rendering solutions for improving surface contact judgments across XR displays. Perceived surface contact plays an important role in depth perception and improving it may help alleviate the disconnected appearance between virtual objects and real surfaces in AR.

%\holly{This will need to be updated. In all XR displays, the cube had higher accuracy than the sphere. In VST AR and VR, the cube had the highest accuracy (i.e., it was higher than the sphere and higher than the icosahedron). In OST AR, there was no difference between the cube and icosahedron. So, generally, the cube had the highest accuracy. And generally, the sphere had the lowest accuracy (sig lower than cube and ico for OST and VST), although the ico had the lowest accuracy for VR (sphere was still lower than cube).} 
In addition, we found that object shape influences surface contact judgments, where judgments were more accurate for the cube than the sphere in all three XR devices. Judgments for the icosahedron were more accurate than the sphere in VST AR and OST AR. Given that there was only case where people's judgements were more accurate for the sphere than another target shape, our current study provides some evidence that spheres may be less effective than other shapes in establishing surface contact. This finding may have implications for depth perception in XR studies, as spheres are a common target object used in distance perception research for these devices \cite{Armbruster:2008:DPV, Gao:2019:IVO, Peillard:2019:SED, Peillard:2020:CRP}. In addition, while our results for the main effect suggest an overall advantage for light shadows for AR, there were some differences in these effects for specific shapes and devices. The benefit of light shadows was largely driven by the cube in OST AR. But in VST AR all shapes were significantly influenced by the presence of a shadow. 

%\holly{In OST, only the cube was affected by shadow. In VST, all shapes were affected by the shadow. In VR, only the sphere was affected by the shadow.}

%In addition, we found that object shape may affect these judgments. In our first study, we found that a rectilinear object with multiple points of contact with the surface beneath it (i.e., the cube) generally outperformed an object with curved contours and a single point of contact with the surface beneath it (i.e., the sphere) across all devices\bbc{This is not true. It was significantly different in 2 of 3 devices. See comment above. Make precise points.}. This finding may have implications for depth perception in XR studies, as spheres are a common target object used in distance perception research for these devices \cite{Armbruster:2008:DPV, Gao:2019:IVO, Peillard:2019:SED, Peillard:2020:CRP}. \sarah{do you want to also comment on what the interactions showed?}

There are limitations to the present experiment. All objects were viewed from a single vantage point, which may affect how generalizable our results are to other geometric shapes and perspectives in XR. This concern is supported by prior research, which has demonstrated that spatial perception is influenced by viewing angle \cite{Lawson:2008:UMF,Ahn:2019:SPA}. Some prior behavioral studies in AR have made conscious efforts to display objects at multiple orientations to subvert any possible effects of orientation \cite{Gao:2019:IVO}. Others have displayed objects at varying heights and distances \cite{Adams:2021:SLC}. Thus, to understand better how the placement of an object may affect people's ability to determine surface contact, we will evaluate target objects at different orientations in the next experiment. %(Section~\ref{exp2}).

A second limitation is that we do not evaluate any 3D objects that have a comparable complexity to those that might be used in typical AR and VR applications. All three objects that we evaluated were simple geometric shapes. As highlighted by Powell et al. \cite{Powell:2012:VPV}, an object's geometry has the ability to influence one's perception of space. In Powell and colleagues' study, researchers evaluated people's ability to reach and grasp virtual spheres, icosahedrons, and apples in VR. They found that the richer geometry cues provided by the icosahedron and apple positively influenced reaching and grasping behaviors. In a similar manner, Do et al. \cite{Do:2020:EOS} evaluated the effect of object color and luminance on objects of different shapes for depth judgments in mobile AR. They found interactions with color and luminance on depth perception. The findings of both of these studies motivate us to evaluate a more complex geometric shape in our next experiment.








%surface contact paradigm to ensure that our results are generalizable. 

%In addition, should we find differences in surface contact judgments for object complexity or orientation, then our results may have ramifications for the design of XR applications. 




%In our second experiment, we wanted to investigate if a more complex 3D object---like the Stanford dragon---would be similarly affected by changes in shadow shading. Prior research by Bailey et al . \cite{Bailey:2006:REW} and Do et al. \cite{Do:2020:EOS} has shown evidence that model dimension or shape may interact with shading as a depth cue. Do et al. \cite{Do:2020:EOS} demonstrated that depth judgments for a complex object, the Stanford bunny in their experiment, was less senstive to changes in shading . We believe that these findings warrant the investigation of our shadow shading conditions for more complex objects.  In addition, we wanted to determine if people’s judgments of ground contact were sensitive to an object’s orientation.


%In addition, we should note that surface contact judgments in OST AR may be more sensitive to changes in shading, as evidenced by the dramatic difference in performance between the cube condition with the light shadow shading method, which outperformed all other conditions, and the cube condition with the dark shadow shading method, which performed worse than all other conditions. 

















==> sections/A2_psychophysics.tex <==







% Revision notes
% H5: update
%%%% cube clearly easier if pointy face points towards you
%%%% cite: Mike Tars (?) canonical orientation
%%%% Also, shape of shadow changes with change in object orientation

%%% Ahhh actually, may want to look at shadow x orientation for each shape? ...




\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth, keepaspectratio]{fig/EXP2_Cubes_Vert_Label2.png}
        \caption{The cube from Experiment 1 is rotated by 45$^{\circ}$ and evaluated under the same shadow shading methods and vertical displacements in Experiment 2.  Here both cubes are shown for visual comparison.}
       \label{fig:exp2_cubes}
\end{figure}

\section{Experiment 2: Complexity and Orientation} \label{exp2}

%\haley{This is rough, but it's done}

%In our second experiment, we wanted to investigate if a more complex 3D object---like the Stanford dragon---would be affected by changes in shadow shading. 
%Prior research by Bailey et al. \cite{Bailey:2006:REW} and Do et al. \cite{Do:2020:EOS} has shown evidence that model dimension or shape may interact with shading as a depth cue. Do et al. \cite{Do:2020:EOS} demonstrated that depth judgments for a complex object, the Stanford bunny in their experiment, was less sensitive to changes in shading. 
%To better understand how object shape complexity influences surface contact judgments for photorealistic and non-photorealistic shadows, we chose to evaluate a more complex shape, the Stanford dragon, with 113,000 polygons.  In addition, because we use a single vantage point to view stimuli in our current paradigm, we wanted to determine if people’s judgments of ground contact were sensitive to an object’s orientation. We believe that evaluating surface contact judgments to objects at multiple orientations will allow us to better ensure that our results are generalizable, especially since prior research has shown that viewing angle can influence spatial perception \cite{Ooi:2001:DDA, Messing:2005:DPV, Ahn:2019:SPA, Feldstein:2020:EDP}. It was also possible that surface contact judgments to objects would be altered by changes in a target object's orientation since the shape of a cast shadow changes along with any changes to its associated object. As such, changes in orientation also cause the shape of a shadow to change.  Figures  \ref{fig:exp2_cubes} and \ref{fig:exp2_dragons}, which display the experimental stimuli used in Experiment 2, present a strong visual argument for investigating orientation since we can observe changes in shape and shading between an object and its cast shadows in these images with rotation. To address these concerns, we evaluate two target objects, a cube and the Stanford dragon, at two orientations, rotated by $0^{\circ}$ and rotated by $45^{\circ}$, in our second study. 

% In our second experiment, we argued once again that people's likelihood of correct response would be more affected by the bottom edge of an object's geometry than its inherent complexity. In addition, we wanted to know if the orientation of an object could adversely affect one’s ability to utilize a shadow to determine surface contact. Figure \ref{fig:exp2_cubes} displays the cube at both orientations and Figure \ref{fig:exp2_dragons} displays the dragon at both orientations. 

%Specifically, we chose to look at how a more complex object would perform under the same shading conditions, and we chose to look at objects with two different orientations.

% \jeanine{I think we need to say more here. What is left open about the findings from Exp 1 that motivated this one? Why would a different shape or orientation matter?}

In this experiment we investigated if shape complexity and orientation influenced the perception of surface contact when dark and light shadows were present.  Figures~\ref{fig:exp2_cubes} and~\ref{fig:exp2_dragons}, which display the experimental stimuli used in Experiment 2, present a strong visual argument for investigating orientation given we can observe changes in shape and shading between an object and its cast shadows in these images with rotation. To address these concerns, we evaluate two target objects, a cube and the Stanford dragon, at two orientations, rotated by $0^{\circ}$ and rotated by $45^{\circ}$, in our second study. Our hypotheses for these experiments were as follows:

\textbf{H4}: We anticipated that people would be worse at discerning the Stanford dragon’s surface contact because it has fewer points in contact with the ground and the 3D model does not have a straight edge along the bottom---unlike the cube primitive. In essence, we argued that the likelihood of correct response would be more affected by the bottom edge of an object's geometry than its inherent complexity. This finding would provide evidence against the idea that more complex geometries are inherently better for depth perception \cite{Do:2020:EOS,Powell:2012:VPV,Bailey:2006:REW}. 

\textbf{H5}: Based on the results from our first study, we predicted that people's surface contact judgments would be more accurate for the light shadow condition than the dark shadow condition across both AR devices. %\sarah{do you mean *both* AR devices or are you including VR in this prediction and mean to say XR?} \haley{definitely just both AR conditions. Fixed} 


\textbf{H6}: We predicted that, overall, a change in object orientation would affect participants' surface contact judgments since changes in orientation can alter both the perceived shape of the surface contact and its associated cast shadow for the viewer. Because the starting position ($0^{\circ}$) was different for the cube and the dragon, it's possible that the $45^{\circ}$ rotation might have deferentially affected the perception of the shapes. Therefore, we also include an interaction between shape and orientation in our analysis.

%We predicted that an object’s orientation would affect people's surface contact judgments since changes in orientation can alter both the perceived shape of the surface contact and its associated cast shadow for the viewer. %\sarah{orientation doesn't really alter the actual shape, right? Do you mean projected or perceived shape?}\bbc{I have reformulated this hypothesis to state what I thought. See if it makes sense.} \sarah{yes, looks good.}

%\jeanine{Is there evidence to suggest that complex objects are better for perceiving depth accurately??} Finally, we predicted that \textbf{H5}: an object’s orientation would not matter since viewers' head movements were not restricted during our experiments and motion parallax was therefore available as a depth cue. \jeanine{I went back to the Intro and Background and there is no mention of motion parallax, so why are we introducing here? What does it add?}

%  Even though the Stanford dragon provides more points of contact along the ground than the prior evaluated objects, I anticipate that the straight, rectilinear edges of the cube will prove more beneficial to ground contact judgments. 




\begin{figure}[t]
    \centering
       \includegraphics[width=\linewidth, keepaspectratio]{fig/EXP2_Dragons_Vert_Label2.png}
        \caption{In Experiment 2, the Stanford dragon was also rendered in each display and shown at two orientations. All other shading and displacement factors were the same as in Experiment 1.}
        \label{fig:exp2_dragons}
\end{figure}



\subsection{Participants}
The same six individuals (3M, 3F) aged 23--30 volunteered to participate in our second experiment. Our experimental methods were approved by the local institutional review board, written consent was obtained from all subjects prior to participation, and each participant was paid 20 USD for 2-3 hours of their time. 

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth, keepaspectratio]{fig/study2_exp2_plotsC.png}
        \caption{
        Experiment 2 ---   Detection thresholds are shown for the OST AR display (left), the VST AR display (middle), and the VR display (right) conditions. In our experiment, thresholds equal the level of vertical displacement at which participants were able to discern that an object was placed above the ground.
        PSE thresholds correspond to 75\% probability of correct response as specified by the psychometric functions displayed in Figure \ref{fig:exp2_pse_curves}. 
        Error bars show  95 \% confidence intervals.
        For each display, we report the absolute detection thresholds for every shape and shadow condition. 
        For visual reference, the statistical significance for our evaluations of H5 (interactions between shape and shadow) at p $<$ 0.05 are noted by (*). }
        %Each point within the figures corresponds to the average probability of correct response in Experiment 1 for a given shape and shadow condition at each level of vertical displacement (except for the case when displacement of both targets was 0mm since there was no incorrect response for this condition). In addition, the psychometric curves for response data are shown, which were calculated by fitting the data with cumulative normal curves via generalized linear model.}
        %%% Response data from the 2AFC task in Experiment 2 has been fitted with a cumulative logistic distribution using maximum likelihood. The figure shows the psychometric curves for response data for the OST AR display (left), the VST AR display (middle), and the VR display (right) conditions.}
        %        Experiment 1 --- The psychometric functions were calculated by fitting response data to cumulative logarithmic distributions. The psychometric curve displays the probability of correct response for a given shape and shadow condition at each level of vertical displacement. PSE thresholds are marked along the curve for each condition.
       \label{fig:exp2_pse_curves}
\end{figure*}

\subsection{Design}

Our experimental design for the second evaluation mirrored the one employed by our first, in which a temporal two-alternative forced choice (2AFC) paradigm with a method of constant stimuli was employed. All experimental details were the same, except for the independent variables. We used the same testing environment, height displacement values (between 0 and 6mm), the same number of comparisons, and the same number of trials. We employed two models, the cube from Experiment~1, and the Stanford Dragon,\footnote{http://graphics.stanford.edu/data/3Dscanrep/} tesselated to have 113,000 polygons. %\bbc{The default dragon has something like 871K or 1.13M triangles depending on which model you get - you got a low-res model somewhere, I assume?}. \haley{I decimated the original 3D model in Blender so it wouldn't cause any performance issue in the Zed or HoloLens :) }

Each participant evaluated two cast shadow conditions (dark and light) over three different object + orientation conditions: the cube rotated by $45^{\circ}$, the Stanford dragon rotated by $0^{\circ}$, and the Stanford dragon rotated by $45^{\circ}$. This resulted in 6 unique combinations of experimental stimuli. However, our analysis evaluated 8 combinations of stimuli, as we included the non-rotated cube condition (at the two shadow conditions) from Experiment 1. This was done to prevent participant fatigue from an increased number of trials. In the second experiment, 1,980 points of data were collected from each volunteer for a total of 11,880 datapoints. When combined with the cube data from the first experiment, each participant completed 2,640 trials for a total of 15,840 trials across all subjects. 

%\sarah{I think the previous description of how you get 8 combinations can be simplified. Something like: However, our analysis evaluated 8 combinations of stimuli, as we included the non-rotated cube condition (at the two shadow conditions) from experiment 1.} \haley{Fixed} 

Using the same approach that we employed for Experiment 1, we evaluated the extent to which participant variance accounted for variance in our collected data by calculating the intraclass correlation coefficient (ICC) for Experiment 2. For the OST AR display condition we found $\tau_{ost}$ = 0.006 and for the VST AR display we found $\tau_{vst}$ = 0.028. For the VR display condition $\tau_{vr}$ = 0.023. Because our ICC values were near zero, we determined that our experimental findings were not significantly influenced by between participant variation. 


\subsection{Procedure}
The procedure for the second experiment followed the same protocol used in Experiment 1. However, this time volunteers did not undergo training for the devices and experimental paradigm since they had already performed the experimental task before.




\input{tables/_Exp2_PSE_Table}




\subsection{Results} \label{exp2_results}
% For Experiment 2, we additionally compared surface contact judgments between the same object presented at two different orientations to understand if an individual object's orientation would influence surface contact judgments. For this research question, we ran separate analyses for each object and collapsed across all other conditions for a given object. 

\paragraph{Descriptive Statistics} For our second study, we used the same approach for analysis as described in Experiment 1. We first report the psychometric functions and detection thresholds of our experimental conditions by fitting response data to the cumulative logistic distribution in the same manner as described in Experiment 1 (Section \ref{exp1_results}). We calculated the psychometric functions using the quickpsy package in R \cite{Linares:2016:QRP}. The resulting psychometric curves can be seen in Figure \ref{fig:exp2_pse_curves}, and detection thresholds are reported in Table \ref{tab:exp2_pse}.


\paragraph{Statistical Analyses} 

For our analyses, we used the binary logistic regression model approach that we employed in the first study (See Section \ref{exp1_results}) to analyze participants' 2AFC judgements for each of the three XR devices.  Separate GLMs with logit link functions were run for each device to understand how an object's cast shadow shading, geometric complexity, and orientation affected people's surface contact judgments in each device. Specifically, we modeled binary outcomes (correct or incorrect) for our predictors: object shape, object orientation, shadow shading, and height. Height was recorded in millimeters then centered at zero and treated as continuous. Object shape (2 levels: cube and dragon), orientation (2 levels: rotated by $0^{\circ}$ and by $45^{\circ}$), and shadow shading (2 levels:  dark and light) were treated as categorical factors. These factors were deviation coded. For shadow shading, dark was coded as -.5 and light was .5; for shape, cube was -.5 and dragon was .5; for orientation, $0^{\circ}$ was -.5 and $45^{\circ}$ was .5. %Specifically, we modeled binary outcomes (correct or incorrect) for our predictors, which included object shape (2 levels: cube and dragon), object orientation (2 levels: rotated by $0^{\circ}$ and by $45^{\circ}$), and shadow shading (2 levels:  dark and light).

We tested three planned comparisons for each device. These comparisons were:
 1) whether surface contact judgments differed for different object geometries (i.e., \textbf{H4} the main effect of object shape); 2) the difference in surface contact judgments between dark and light shadow shading across all other conditions (i.e., \textbf{H5} the main effect of shadow shading); and 3) whether an object's orientation influenced people's surface contact judgments (i.e., \textbf{H6} the main effect of orientation). We also included an interaction between object shape and shading and an interaction between object shape and orientation to better understand the relationship between these variables.  %whether an object's orientation influenced people's surface contact judgments for cubes and for dragons (i.e., \textbf{H6}). We also included an interaction between object shape and shading to better understand the relationship between these variables. 

% original orientation versus rotated 
%To determine whether orientation had an effect on judgments, we ran separate simple slopes for the cube and the dragon. We did not collapse across shape for this analysis, given that a meaningful comparison of change between two objects in orientation could not be conducted. The initial orientations for each object (which we describe as $0^\circ$ orientation) is relative to that individual object's original orientation and, as such, is a local value rather than a global one. \holly{reminder to myself to revisit this paragraph}

\input{tables/_Exp2_Tables}


\begin{figure*}[b]
    \centering
    \includegraphics[width=\linewidth, keepaspectratio]{fig/_Simple_Slopes_Geo2.png}
        \caption{
        Experiment 2 --- Predicted probability of correct response for shape (cube, dragon) and shadow (dark, light) interactions  with 95\% confidence }
       \label{fig:exp2_slopes}
\end{figure*}


\subsubsection{Optical See-through AR} \label{exp2:res:ost}
%The results of the logistic regression for the OST AR display data are presented in Table \ref{tab:exp1_ost}.

The psychometric curves and detection thresholds for each shape and shadow condition tested are reported in Figure \ref{fig:exp2_pse_curves} (left) and Table \ref{tab:exp2_pse}, respectively. The results of our statistical analyses are reported in Table \ref{tab:exp2_results}. In our experiment, we expected participants to be more likely to correctly indicate which object was on the ground as the height of target objects increased. This trend can be seen in the positive slope of the psychometric functions in Figure \ref{fig:exp2_pse_curves}. The improvement of participants' performance as height increased is further demonstrated statistically by a main effect of height in our logistic regression model ($OR = 1.13$, $p < .001$). An odds ratio ($OR$) of 1.13 indicates that for every 1mm increase in height, the odds of correctly stating which object was closer to the ground increased by a factor of 1.13.

%\holly{This would mess with the hypothesis numbers, but I'm tempted to order the results as follows: 1) Does an object's complexity matter?; 2) Does shadow shading matter? (and within this section, describe the interaction between shape and shadow); and 3) Does orientation matter? (and within this section, describe the interaction between shape and orientation). If you wanted to be consistent with Exp 1, you could also switch the order shading and shape. I like this ordering because it keeps the interactions with their associated main effects, which I think is important for Exp 2 since you didn't have specified predictions about the interactions. } \haley{YES. I see where you're coming from. Reordering sounds like a good idea. I've updated Exp 1 and Exp 2 accordingly}


\paragraph{H4: Does an object's complexity matter?} 
The dragon shape was more likely to elicit correct responses than the cube ($OR = 1.38$, $p < .01$), when averaged across shadow shading, orientation, and height. This result differs from what we observed in both the VST AR and VR conditions as reported in Sections \ref{exp2:res:vst} and \ref{exp2:res:vr}. 

\paragraph{H5: Does shadow shading method matter?} 
The main effect for shadow ($OR = 3.70$, $p < .001$) indicates that a correct response was 3.70 times more likely when the object was presented with a light shadow compared to a dark shadow, when collapsed across shape, orientation, and height. There was also a significant interaction between shape and shadow ($OR = .41$, $p < .001$). Analysis of the shadow simple slopes by shape indicated that, for both shapes, a light shadow was more likely to yield a correct judgment of ground contact than a dark shadow (supporting the main effect of shadow). However, this effect was stronger for the cube ($OR = 5.79$, $p < .001$) than the dragon ($OR = 2.37$, $p < .001$).

\paragraph{H6: Does object orientation matter?}
There was a significant main effect of orientation ($OR = 1.96$, $p < .001$) indicating that, overall, participants were more likely to make a correct judgment when the object was rotated $45^\circ$ from its starting position. This main effect was qualified by an interaction between object shape and orientation ($OR = .60$, $p < .01$). In order to interpret the interaction, we calculated the orientation simple slopes for each shape. For both shapes, the likelihood of correctly judging ground contact was higher for the $45^\circ$ orientation than the $0^\circ$ orientation (supporting the main effect of orientation). However, this effect was stronger for the cube ($OR = 2.53$, $p < .001$) than for the dragon ($OR = 1.52$, $p < .01$).
%To determine whether orientation had an effect on judgments, we ran separate simple slopes for the cube and the dragon. We did not collapse across shape for this analysis, given that a meaningful comparison of change between two objects in orientation could not be conducted. The initial orientations for each object (which we describe as $0^\circ$ orientation) is relative to that individual object's original orientation and, as such, is a local value rather than a global one. \holly{reminder to myself to revisit this paragraph}

%Our analysis of orientation by shape simple slopes indicated that the effect of orientation was significant for both objects. That is, the probability of providing a correct response was higher when an object was rotated by 45$^\circ$ regardless of whether the object presented was a cube ($OR = 2.53$, $p < .001$) or a dragon ($OR = 1.52$, $p < .01$).

%\paragraph{Is there an interaction between shape and shadow?}

%Analysis of the shadow by shape simple slopes indicated that the effect of shadow was significant for both shapes. That is, the probability of correct response was higher when a light shadow was presented regardless of whether the object presented was a cube ($OR = 5.79$, $p < .001$) or a dragon ($OR = 2.37$, $p < .001$). 



\subsubsection{Video See-through AR} \label{exp2:res:vst}



The detection thresholds for our experimental conditions are reported in Table~\ref{tab:exp2_pse} while the complete psychometric curves are shown in Figure~\ref{fig:exp2_pse_curves} (middle). The results of our statistical analyses are reported in Table~\ref{tab:exp2_results}. For VST AR we again found a main effect of height ($OR = 1.09$, $p < .001$), which is also illustrated by the positive slopes of the psychometric curves in Figure~~\ref{fig:exp2_pse_curves}. Accordingly, as the height of the vertically displaced object increased, participants were more likely to correctly indicate which object was on the ground. 

\paragraph{H4: Does an object's complexity matter?} 
The cube shape was more likely to elicit correct responses than the dragon  ($OR = .32$, $p < .001$), suggesting that object complexity is not inherently beneficial to surface contact perception. 

\paragraph{H5: Does shadow shading method matter?} 
The main effect for shadow ($OR = 2.47$, $p < .001$) indicates that a correct response was 2.47 times more likely when the object was presented with a light shadow compared to a dark shadow. In addition, there was a significant interaction between shape and shadow ($OR = .61$, $p < .05$). Analysis of the shadow by shape simple slopes indicated that the effect of shadow was significant for both shapes. For both shapes, the probability of correct response was higher when a light shadow was presented compared to a dark shadow. However, this effect was stronger for the cube ($OR = 3.17$, $p < .001$) than the dragon ($OR = 1.93$, $p < .001$). 

%Analysis of the shadow by shape simple slopes indicated that the effect of shadow was significant for both shapes. That is, the probability of correct response was higher when a light shadow was presented regardless of whether the object presented was a cube ($OR = 3.17$, $p < .001$) or a dragon ($OR = 1.93$, $p < .001$). 

\paragraph{H6: Does object orientation matter?}

There was no main effect of orientation in VST AR. The interaction between orientation and shape was also insignificant. In other words, the probability of providing a correct response was not significantly different between the two orientations in VST AR. %Further, our analysis of orientation by shape simple slopes indicated that the effect of orientation was not significant for either shape. That is, the probability of providing a correct response was not significantly different between the two orientation for either the cube or the dragon in VST AR. 

%\paragraph{Is  there  an  interaction  between  shape  and  shadow?}







\subsubsection{Virtual Reality} \label{exp2:res:vr}

The psychometric curves for our experimental conditions are shown in Figure~\ref{fig:exp2_pse_curves} (right) and the corresponding detection thresholds are reported in Table~\ref{tab:exp2_pse}. The results of our statistical analyses are reported in Table~\ref{tab:exp2_results}. For VR we found a main effect of height ($OR = 1.06$, $p < .001$) such that for every 1mm increase in height, the odds of correctly stating which object was closer to the ground increased by a factor of 1.06.The psychometric curves in Figure~\ref{fig:exp2_pse_curves} also illustrate that participants became more likely to correctly indicate which object was placed on the ground as the height of the vertically displaced objects increased. 


\paragraph{H5: Does an object's complexity matter?} 
The cube was more likely to elicit correct responses than the dragon  ($OR = .27$, $p < .001$), suggesting that object complexity is not inherently beneficial to surface contact perception. 

% these results
\paragraph{H4: Does shadow shading method matter?} 
The main effect for shadow ($OR = 1.68$, $p < .001$) indicates that a correct response was 1.68 times more likely when the object was presented with a light shadow compared to a dark shadow. The interaction between shape and shadow was significant ($OR = .64$, $p < .05$). Unlike our results for Experiment 1, the analysis of the shadow by shape simple slopes indicated that the effect of shadow was significant for both shapes in VR. The probability of correct response was higher when a light shadow was presented regardless of the object presented, although the shadow effect was stronger for the cube ($OR = 2.11$, $p < .001$) than the dragon ($OR = 1.34$, $p < .001$).

\paragraph{H6: Does object orientation matter?}
%\holly{This originally said that there was a main effect of orientation, but the main effect of orientation was NOT significant. It also said that the simple slopes showed that the effect of orientation was the same for both shapes, but that is not the case.} \haley{RIP that was definitely from an older version of the paper. smh I've become change blind to this paper after so many revisions.  Thanks for catching this, Holly!}
The main effect of orientation was not significant. However, there was a significant interaction between shape and orientation ($OR = 2.16$, $p < .001$). Analysis of the orientation by shape simple slopes indicated that a correct response was more likely when the cube was presented at 0$^\circ$ than when the cube was rotated 45$^\circ$ ($OR = .60$, $p < .01$). In contrast, the probability of a correct response was higher when the dragon was rotated 45$^\circ$ than when it was presented at 0$^\circ$ ($OR = 1.29$, $p < .05$).

%There was a significant main effect of orientation ($OR = .88$, $p < .01$) indicating that, overall, participants were more likely to make a correct judgment when the object was at its default orientation. This main effect was qualified by an interaction between object shape and orientation. Our analysis of orientation by shape simple slopes indicated that the effect of orientation was significant for both objects. That is, the probability of providing a correct response was higher when an object was rotated by 0$^\circ$ when the object presented was a cube ($OR = .60$, $p < .01$) and the probability of correct response higher when an object was rotated by 45$^\circ$ a dragon ($OR = 1.29$, $p < .05$).

%\paragraph{Is  there  an  interaction  between  shape  and  shadow?}












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsubsection{Does shadow shading method matter?} \label{exp2_results_shading}
 
For each device, we evaluated the two shadow shading conditions (dark and light) when collapsed across all other conditions and found that people's  likelihood of correct response for whether an object was off the ground or not was significantly higher when presented with the non-photorealistic, light shadow in all three XR displays. Tables \ref{tab:exp2_ost}-\ref{tab:exp2_vr} display the fixed effects for dark versus light shadows across all three devices with the \textit{Shadow (dark vs. light)} variable. No Bonferroni correction was applied to this analysis since only one comparison was made. Therefore, the significance value remained \textit{p}$<0.05$.


 These findings confirmed our first hypothesis (\textbf{H4}), in which we predicted that people's surface contact judgments would be more accurate when objects were presented with light cast shadows in both AR devices. However, it is interesting to note that people's judgments were also significantly better with non-photorealistic, light shadows in the VR condition in this experiment as well. 
 



\subsubsection{Does an object's complexity matter?} \label{exp2_results_complexity}
%We  anticipated that geometric complexity would not inherently improve depth perception. Given the results of our first study, in which the cube outperformed the sphere across all devices, we predicted that people's likelihood of correct response would be more affected by the shape of an object along the bottom edge than by geometric complexity---where complexity is defined by the number of polygons used to construct a given object's mesh.  Even though the complex object evaluated in this study (the Stanford dragon) provided more points of contact along the ground than either the icosahedron or the sphere that were previously evaluated, we believed that the straight, rectilinear edges of the cube would still prove more beneficial to ground contact judgments. 

To understand how object shape complexity influenced surface contact judgments in XR, we evaluated judgments for the cube and the dragon when collapsed across all other conditions. For each display the results of these analyses can be seen in Tables \ref{tab:exp2_ost}--\ref{tab:exp2_vr}, where \textit{Shape (cube vs. dragon)} is the relevant variable for our research question.  Because only one comparison was made, no Bonferroni correction was applied. 

When we compared surface contact judgments between the cube and the dragon we found that our hypothesis held true for both VST AR (Table \ref{tab:exp2_vst}) and VR (Table \ref{tab:exp2_vr}) with judgments for the cube being more accurate than those for the dragon. However, people had a higher likelihood of correct response for the dragon in OST AR (Table \ref{tab:exp2_vr}). As such, we were only partially able to confirm \textbf{H5}. Although our prediction that more complex objects would not inherently improve ground contact judgments is supported by our results in VST AR and VR---showing an advantage for the cube over the dragon---the opposite result found with the OST AR display is surprising. %a more complex interaction between shape and shadow is apparent in the OST AR display. 





\subsubsection{Does the orientation of an object matter?} \label{exp2_results_orientation} 

To determine whether orientation had an effect on judgments, we ran separate GLMs for the cube and the dragon. We did not collapse across objects for this analysis, given that a meaningful comparison of change between two objects in orientation could not be conducted. The initial orientations for each object (which we describe as $0^\circ$ orientation) is relative to that individual object's original orientation and, as such, is a local value rather than a global one. The relevant variables for our analyses in Tables \ref{tab:exp2_ost}--\ref{tab:exp2_vr} were: \textit{Orien  cube  ($0^\circ$ vs. $45^\circ$)} and \textit{Orien  dragon  ($0^\circ$ vs. $45^\circ$)}. The Bonferroni corrected significance value for these comparisons was $p<0.025$ since two comparisons were made. 





% \sarah{I think I understand this, but this doesn't seem consistent with what you say the models were in 6.4 which seems to imply all one model, not separate for cube and dragon. I think we need to be more clearer on this.} \haley{Fixed?} \sarah{better, but now I think the orient x shape label is misleading. I think this is just a comparison between orientation for the cube or dragon separately, so should not be presented as an interaction in the table. I would just say something like, Orien (0 vs. 45) for cube, and Orien (0 vs. 45) for shape.} \haley{Fixed!}


People's likelihood of correct response for the cubes significantly differed between the two orientations in OST AR (Table \ref{tab:exp2_ost})  and VR  (Table \ref{tab:exp2_vr}). Judgments for the cube at $0^{\circ}$ were more accurate than judgments for the cube at $45^{\circ}$ in OST AR, but the opposite was true in VR. People's accuracy also differed between the two dragon orientations in OST AR  (Table \ref{tab:exp2_ost})  and VR (Table \ref{tab:exp2_vr}) such that judgments for the dragon at $0^{\circ}$ were more accurate than judgments for the dragon at $45^{\circ}$ in both devices. However, in the VST AR condition, there were no significant differences in surface contact judgments between orientations for either the cube or the dragon  (Table \ref{tab:exp2_vst}). Because changes in orientation had a significant effect for both objects in OST AR and VR, \textbf{H6} was partially confirmed. 



\subsubsection{Is there an interaction between shape and shadow?} \label{exp2_results_interactions}
% Looking at shape $\times$ shadow $\times$ orientation interactions across devices,
% \sarah{are these corrected for multiple comparisons? We should talk more about whether all of these should be done, or only comparisons that are motivated, similar question to exp 1}. \haley{I agree with Sarah's comment that we should only discuss motivated comparisons. Otherwise, the actual questions of our research may become lost. This section was a relic from the the original draft that I sent out a month ago, anyway. If anything, I can parse this down to just look at shadow x orientation interactions for each shape (which is something we discussed previously) }


Given our findings in Experiment 1, which showed interactions for surface contact judgments between shape and shadow, we anticipated interactions in Experiment 2. Understanding these interactions was especially important for determining if the advantage of non-photorealistic, light shadows that we found in the current study was consistent across different shapes. We also believed that this analysis would help us better understand why we found a significant effect for shadow shading conditions in Experiment 2 but not in Experiment 1 for the VR display.  For these reasons, we conducted two unique, paired comparisons for shape $\times$ shadow conditions for each device, where the relevant variables for our investigation included \textit{Shadow$\times$Shape (cube: dark vs. light)} and  \textit{Shadow$\times$Shape (dragon: dark vs. light)}. The Bonferroni corrected significance value for these comparisons was \textit{p}$<0.025$ since two comparisons were made. %\sarah{okay now I understand the interactions you tested but these are not in the tables at all. See comment above that I don't think Orien should be presented as an interaction} \haley{Agreed! Fixed}


Across all devices we found significant effects of cast shadow shading for the cube and for the Stanford dragon, where people's surface contact judgments were more accurate with the light shadow (Tables \ref{tab:exp2_ost}-\ref{tab:exp2_vr}). These findings are encouraging because they provide evidence that the significant main effects we found for shadow shading condition in Experiment 2 are generalizable across objects of different complexity. 
\end{comment}



\begin{comment}
% Our experiment resulted in $28$ unique, paired comparisons across shape, orientation, and shadow conditions for each device. \sarah{are these corrected for multiple comparisons? We should talk more about whether all of these should be done, or only comparisons that are motivated, similar question to exp 1}.  Due to the high number of comparisons, for clarity the fixed effects and significance levels of each analysis are displayed in Table \ref{tab:exp2_ost} for the OST AR display, Table \ref{tab:exp2_vst} for the VST AR display, and Table \ref{tab:exp2_vr} for the VR display. 

% Patterns across devices 

%The video see-through and virtual reality conditions resulted in remarkably similar response patterns. The order of variables from highest to lowest likelihood of correct response is the same for both devices, as seen in Tables \ref{tab:exp2_vst} and \ref{tab:exp2_vr}. For both displays, all cube conditions outperformed all dragon conditions. And all light shadow conditions outperformed all dark shadow conditions for a given shape (cube or dragon). However, for each device, the degree of significance between these relationships varied. \sarah{it's not really meaningful to talk about degree of significance, if you are using a specific threshold such as .05 or .01 to claim significance.}

%% VR 
%In VR, all cube conditions performed significantly better than the dragon conditions (See Table \ref{tab:exp2_vr}). In addition, there was no significant difference in performance between three out of the four cube conditions (Cube $45^\circ$LS, Cube $0^\circ$LS, and Cube $0^\circ$DS), and there was no significant difference in performance between three out of the four dragon conditions (Dragon $45^\circ$LS, Dragon $0^\circ$LS, and Dragon $45^\circ$DS). There were, however, significant differences in performance between the two dark shadow conditions for the cube  ($\beta  = 0.817 , SE= 0.231 , p<0.001$) and the two dark shadow conditions for the dragon ($\beta  = 0.448 , SE= 0.154 , p=0.004$). 

%%% VST AR
%In contrast, for the video see-through AR, there was more overlap in performance between the worst performing cube conditions and the best performing dragon conditions such that both cube with dark shadow conditions performed similarly to the dragon with light shadow conditions. The exception to this rule was that there was a significant difference between the Cube$0^\circ$DS and Dragon$0^\circ$LS conditions ($\beta= 0.496 , SE= 0.184 , p=0.007$). 

%%% OST AR
%The optical see-through AR display evoked very different responses from participants, which we expect is due to the dramatic differences in rendering and hardware between this device and both the VST AR and VR display conditions. In OST AR, we found that the light shadow conditions significantly outperformed all dark shadow conditions---regardless of object shape (See Table \ref{tab:exp2_ost}). The exception to this statement is the worst performing light shadow condition (Cube $0^\circ$LS) and the best performing dark shadow condition (Dragon $45^\circ$DS), which were not significantly different ($\beta= 0.097 , SE= 0.197 , p=0.622$). How geometric shape informs ground contact judgments is less clear in OST AR. Unlike what we see in the other two XR conditions, the cube conditions have dramatically different performance depending on shadow shading method, where both of the cube with dark shadow conditions are the worst performing stimuli but the cube at $45^\circ$ with light shadow performs better than all other conditions. This curious pattern can be seen in Table \ref{tab:exp2_ost}.  %, and its implications are discussed further in Section \ref{exp2_discussion}.} 
\end{comment}


% shadow shading
%Did we once again see a dramatic performance difference between the cube conditions with the light shadow and the cube conditions with the dark shadows? Yes. shadow had a polarizing effect on ground contact judgments. 



%% OST AR
%  cubes all dif from each other
%  dragons same with light shadow

%% VST AR
%  cubes = same
%  dragons = same 

%% VR
%  cubes LS = same. DS = dif.
%  dragons LS = same. DS = dif. 

%  Orientation $\times$ shadow 
%% OST AR
%  cubes = different
%  dragons = different

%% VST AR
%  cubes = different
%  dragons = different

%% VR
%  cubes = 45 same. 0 different.  
%  dragons =  45 same. 0 different.

% PSE_BAR...   







\subsubsection{How difficult was each condition?}
%To inform our results, we also collected post surveys after participants complete the experiment in each device and after participants completed the entire experiment. Volunteers were asked about the difficulty of this second experiment in comparison to the first, and our results were mixed. Some participants found that the second experiment was harder, others reported that the second experiment was easier, and one participant responded that they were the same difficulty. 


After completing the second experiment, volunteers were asked to rank each device by difficulty and by quality of graphics as in Experiment 1. All participants ranked the video see-through display as the most difficult device (6/6) and the device with the lowest quality of graphics (6/6). In contrast, the optical see-through display was most consistently rated as the easiest display (4/6) and the display with the highest quality of graphics (5/6). Ratings were also corroborated by comments at the end of the survey. Both P2 and P4 stated that the HoloLens ``\textit{felt more clear}," and P1 commented that ``\textit{the resolution of the Zed was really painful for my eyes."} %Given overall performance of the dragon object across devices, it is possible that fine depth judgments like those used in this study are affected by quality of graphics---despite evidence that quality of graphics does not inherently affect depth perception in VR\cite{Thompson:2004:DQC}. 

Participants were also asked about the strategies they used to discern surface contact. P3 commented that the dragon was ``\textit{easier but more mentally exhausting... since the dragon moved.}" Their comment implied that they had to visually search for a shadow before making a judgment. Their complaint is reasonable since, as the shape of the dragon was asymmetrical, changes in orientation were more pronounced (See Figure \ref{fig:exp2_dragons}). P3 further bemoaned of the dragon that ``\textit{when too detailed it was overwhelming, [but] when not detailed enough it became equally difficult to use}." P2 commented that the dragon provided more ``\textit{pockets of shadow,"} which altered their strategy such that ``\textit{ It wasn't just watching an edge, more like watching for shape and quantity of shadow.}" This comment hints that people may have been able to use additional depth information provided by the dragon (e.g., shape from shading) to inform their judgments of surface contact. 



%Peering closer into the relationship between shape and shadow in the optical see-through display (See Table \ref{tab:exp1_ost}), we can see that the fixed effects between light and dark shadow conditions did not significantly differ for the icosahedron ($\beta = 0.309, p=0.060$), nor did they differ for the sphere ($\beta=0.134, p=0.351$). However, light and dark shadows did have a significant effect for the cube ($\beta = 1.446, p<0.001$). In fact, the cube with the light shadow performs significantly better than all other conditions while the cube with the dark shadow performs worse than all other conditions. For the Microsoft HoloLens, the dramatic difference in performance between light and dark shadows in the cube condition seems to indicate that \haley{what?}. It also demonstrates why the icosahedron out performs the cube when we collapse across shadow conditions. 


%%If we recall from Section \ref{exp2_results_orientation}, there was no significant difference across orientations for either the cube condition or the dragon condition in VST AR---which was not true for either the OST AR or VR displays. Looking at Table \ref{tab:exp2_vst}, it is apparent how there was no significance in object orientation for VST AR. For each shape (cube or dragon) and for each shadow condition (light or dark) there were no significant differences between the object when presented at $0^\circ$ and the object presented at $45^\circ$. 


\subsection{Discussion} \label{exp2_discussion}
%\bbc{This point needs to be brought up in the discussion, but isn't that I can see. The point is: what is different between this experiment and experiment 1 for VR? Orientation and shape complexity.}
% \bbc{However, the results show that in VR, the cube is easier to make a correct judgment on than the dragon (I think that's what your results show). This would lead us to believe that it must be the orientation that makes the light shadows important in VR}.

In Experiment 2, for both AR display conditions, we again found that people's judgments of surface contact benefited from the presence of non-photorealistic, light cast shadows. However, in contrast to our first study, we also found that light shadows improved surface contact judgments in VR. Looking at shape $\times$ shadow interactions for the cube in Experiment 1 and Experiment 2 in VR may provide some insight into this difference in shadow effectiveness for VR between experiments. Both experiments evaluated the same cube object, but the object was presented at a new orientation in Experiment 2. Because we found a significant difference in orientation for the cube and because we found an effect of shadow shading condition in Experiment 2, we infer that the change in orientation for the cube made the light shadows more important in VR. 

%In contrast to the results of our first experiment regarding shape $\times$ shadow interactions (where judgments were not affected by shadow shading for the cube or icosahedron in VR), we did find an effect of shadow shading condition in Experiment 2 for VR. We believe that presenting the cube at a second orientation (rotated by $45^{\circ}$) in Experiment 2 affected people's ability to discern surface contact for our analysis. This idea is further reinforced by our findings for the influence of object orientation in Experiment 2, in which surface contact judgments for the cube rotated by $45^{\circ}$ were less accurate than judgments for the cube rotated by $0^{\circ}$. \sarah{I read this paragraph several times and I am confused about the argument.}\jeanine{Tried to alter beginning a bit, but not sure it helped....}

%Overall, however---across both experiments, across all object shapes, and regardless of object orientation---we consistently found that people's surface contact judgments when presented with non-photorealistic shadows were either more accurate or as accurate as those presented with photorealistic shadow shading. 


%%\sarah{I think some discussion of shadow effect in VR in exp 2 but not exp 1 needs to be added. Why might there have been a difference between experiments?} \haley{Fixed}

%Looking at shape $\times$ shadow interactions, in both VST AR and VR performance was dictated more by object than by shadow shading condition. In contrast, in OST AR, performance was driven by shadow shading condition more so than object type. 

Our hypothesis that surface contact judgments for the dragon would be worse than the cube was partially supported. Although we found better performance with the cube compared to the dragon in both VST AR and VR, we found better performance with the dragon in OST AR. With the current experiment alone, we are unable to explain why people's judgments for the dragon in the OST AR device alone were significantly more accurate than those for the cube. However, the current study provides evidence that more complex geometries do not inherently benefit surface contact perception. Although complex 3D shapes can provide more depth information via self-shading cues, it appears that other factors such as the bottom edge of the object may be more important. However, additional future research is needed to verify this claim. 

%Replicating the trend we found in Experiment 1, the cube with light shadow conditions and the cube with dark shadow conditions yielded polarized judgments in the surface contact task, such that the best condition was the cube $45^\circ$ with light shadow, and the two worst conditions were both of the cube conditions with dark shadows. Based on the prior results of Adams et al. \cite{Adams:2021:SLC}, we believe the OST AR results are due to the contrast between the object and its shadow for the cube condition. Because self shading was not manipulated for a given target object, the dark self-shading information of the cube allowed the light shadow shading method to perform especially well. But this made it difficult for people to discern the difference between the object and its shadow in the dark shadow conditions given the HoloLens uses additive light to render dark color values. 


%\haa{orientation discussion} 


Given the effects of orientation that we found in both the OST AR and VR displays, it will be important to consider the orientation of objects in XR in future application development. This finding is in line with prior research which shows that the angle from which we view a 3D object may affect spatial perception judgments related to that object\cite{Lawson:2008:UMF,Ahn:2019:SPA}.  The lack of difference in orientation for the video see-through conditions requires further investigation. 


%Our results on orientation also have implications for the study and development of XR applications. In the realm of research, it is apparent that the angle from which we view a 3D object may affect spatial perception judgments related to that object \cite{Ooi:2001:DDA, Messing:2005:DPV, Ahn:2019:SPA, Feldstein:2020:EDP}. Accordingly, researchers must be careful about which objects they use to evaluate depth perception and how they position target objects in space when evaluating depth perception in XR. One solution would be to progressively rotate a virtual target to minimize the influence of one orientation like in Peillard et al.  \cite{Peillard:2019:SED}. However, for the development of commercial and educational XR applications,  we recognize that people may need to view virtual images that are placed at a specific angle, for example, when interacting with a virtual desktop monitor in AR. For these kinds of applications, understanding how specific shapes and orientations of objects influence where people perceive them to be positioned in space may be more pertinent. 


%\jeanine{Why was this curious??} \haley{Curious because I have no idea why VST AR would not show any effects of orientation when the other two devices did! Any thoughts on this?}\bbc{I don't think this remark belongs here. Remove it and comment on it in the discussion: It is interesting that ..... We do not understand why ... subject for future investigation ...} 

%\input{tables/Exp2_Tables_Big}
% Dragon x shadow vs cube x shadow
% 

%\haa{You should look into how accurate people were in a given device. If people were highly accurate in OST AR and highly inaccurate in VST AR, then this could be due to resolution} It is possible that the dragon provided additional depth information, which prevented it from performing as poorly as the cube in the dark shadow condition. %It is possible that the additional complexity of the dragon object provided sufficient supplementary depth information to help mitigate the negative effects of the dark shadow conditions for this game object. As in the experiment conducted by \haley{Adams et al. }, we find that surface contact perception between an object and its shadow is highly sensitive in optical see-through displays. 



% By looking at the shape $\times$ shadow interactions discussed in Section \ref{exp2_results_interactions} and visualized in Table \ref{tab:exp2_ost}, we may glean some insight into how the OST AR display performed differently than the other two XR devices. It is possible that people may be relying on additional depth cues from the dragon in the OST AR

%% For the cube primitive, the presence of a light or dark shadow had a polarizing effect on performance. For example, the best performing condition in OST AR was a cube with a light shadow and the worst performing condition was a cube with a dark shadow.




\begin{comment}
\begin{figure*}[ht] 
        \centering 
        \includegraphics[width=\linewidth,keepaspectratio]{fig/study2_exp2_bars_lapses.png}  
        \caption{ Experiment 2 --- The absolute detection thresholds, or points of subjective equality (PSE), for the dark and light shadow conditions for each shape (cube, dragon). In our experiment, thresholds equal the level of vertical displacement at which participants were able to discern that an object was placed above the ground. 
        PSE thresholds correspond to 75\% probability of correct response as specified by the psychometric functions displayed in Figure \ref{fig:exp1_pse_curves}. 
        Error bars show  95 \% confidence intervals. For visual reference, the statistical significance for our evaluations of H4 (interactions between shape and shadow) at p $<$ 0.05 are noted by (*).  }       
        \label{fig:exp2_bars}
\end{figure*}
\end{comment}

==> tables/Exp1_Tables.tex <==







\fboxsep=1mm 
\definecolor{BgColor}{HTML}{ffffff} %3c92da
\definecolor{OffWhite}{HTML}{ffffff}
\definecolor{OffBlack}{HTML}{2E2E2E}



\definecolor{Pos}{HTML}{2878CC} %darker ver 2469b3
\definecolor{PosLite}{HTML}{96bfeb} 

\definecolor{Neg}{HTML}{617285}  %576778
\definecolor{NegLite}{HTML}{a2b5ca}





%% TABLE FOR EXP OST AR RESULTS
\begin{table}[!t]
\small
\centering 
\renewcommand{\arraystretch}{1.0}\setlength{\tabcolsep}{1pt} 
\begin{tabularx}{\linewidth}{@{}XXXXXXX@{}}
      \multicolumn{1}{l}{} &\multicolumn{1}{c}{Cube LS} &\multicolumn{1}{c}{Ico LS} &\multicolumn{1}{c}{Ico DS} &\multicolumn{1}{c}{Sph DS} &\multicolumn{1}{c}{Sph LS} &\multicolumn{1}{c}{Cube DS}  \\
 
        \rowcolor{Pos}\cellcolor{white} Cube LS  
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\includegraphics[width=\linewidth]{tables/cubew_tab2.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.404$ \quad $p$ ~\textdblhyphen~ $0.029^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.714$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.010$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.144$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.446$ \quad $p$ {\tiny \textless} $0.001^*$} \\
        
        \rowcolor{Pos}\cellcolor{white} Ico LS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.404$ \quad	$p$ ~\textdblhyphen~ $0.029^*$} \cellcolor{Neg} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/icow_tab2.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.309$ \quad $p$ ~\textdblhyphen~ $0.060$} \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.606$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.740$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.042$ \quad	$p$ {\tiny \textless} $0.001^*$} \\
         
        \rowcolor{Pos} \cellcolor{white}Ico DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.714$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.309$ \quad $p$ ~\textdblhyphen~ $0.060$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/ico_tab3.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.297$ \quad $p$ ~\textdblhyphen~ $0.050$}
        \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.430$ \quad $p$ ~\textdblhyphen~ $0.004^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.732$ \quad $p$ {\tiny\textless} $0.001^*$}	\\
         
        \rowcolor{Neg} \cellcolor{white} Sph DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.010$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.606$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.297$ \quad $p$ ~\textdblhyphen~ $0.050$} \cellcolor{NegLite}	
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/sphere_tab9.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.134$ \quad $p$ ~\textdblhyphen~ $0.351$} \cellcolor{PosLite} 
        &\textcolor{white}{$\beta$ ~\textdblhyphen~ $0.436$ \quad $p$ ~\textdblhyphen~ $0.002^*$} \cellcolor{Pos}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Sph LS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.144$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.740$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.430$ \quad $p$ ~\textdblhyphen~ $0.004^*$} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.134$ \quad $p$ ~\textdblhyphen~ $0.351$} \cellcolor{NegLite} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/spherew_tab2.PNG}} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.302$ \quad $p$ ~\textdblhyphen~ $0.028^*$ } \cellcolor{Pos} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Cube DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.446$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.042$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.732$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.436$ \quad $p$ ~\textdblhyphen~ $0.002^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.302$ \quad $p$ ~\textdblhyphen~ $0.028^*$} 
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/cube_tab2.png}}  \\ \\
        
\end{tabularx}
\caption{Fixed effects of generalized linear mixed model from first experiment for the OST AR display}\label{tab:exp1_ost}

\end{table}




%% TABLE FOR EXP VST AR RESULTS
\begin{table}[!t]
\small
\centering 
\renewcommand{\arraystretch}{1.0}\setlength{\tabcolsep}{1pt} 
\begin{tabularx}{\linewidth}{@{}XXXXXXX@{}}
      \multicolumn{1}{l}{} &\multicolumn{1}{c}{Cube LS} &\multicolumn{1}{c}{Ico LS} &\multicolumn{1}{c}{Cube DS} &\multicolumn{1}{c}{Sph LS} &\multicolumn{1}{c}{Ico DS} &\multicolumn{1}{c}{Sph DS}  \\
      
        \rowcolor{Pos}\cellcolor{white} Cube LS  
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\includegraphics[width=\linewidth]{tables/cubew_tab2.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.880$ \quad $p$ ~\textdblhyphen~ $0.001^*$} \cellcolor{Pos} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.880$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.880$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.168$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.204$ \quad $p$ {\tiny \textless} $0.001^*$} \\
        
        \rowcolor{Pos}\cellcolor{white} Ico LS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.880$ \quad	{\tiny \textless} $0.001^*$} \cellcolor{Neg} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/icow_tab2.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.000$ \quad $p$ ~\textdblhyphen~ $0.99$} \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.000$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.289$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.324$ \quad	$p$ {\tiny \textless} $0.001^*$} \\
         
        \rowcolor{Pos} \cellcolor{white}Cube DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.880$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.000$ \quad $p$ ~\textdblhyphen~ $0.99$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/cube_tab2.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.000$ \quad $p$ {\tiny \textless} $0.001^*$}
        \cellcolor{Pos} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.289$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.324$ \quad $p$ {\tiny\textless} $0.001^*$}	\\
         
        \rowcolor{Neg} \cellcolor{white} Sph LS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.880$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.000$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.000$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}	
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/spherew_tab2.png}} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.289$ \quad $p$ ~\textdblhyphen~ $0.038^*$} \cellcolor{Pos} 
        &\textcolor{white}{$\beta$ ~\textdblhyphen~ $0.324$ \quad $p$ ~\textdblhyphen~ $0.019^*$ \cellcolor{Pos}}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Ico DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.168$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.289$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.289$ \quad $p$ {\tiny \textless} $0.001^*$}  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.289$ \quad $p$ ~\textdblhyphen~ $0.038^*$} \cellcolor{Neg} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/ico_tab3.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.036$ \quad $p$ ~\textdblhyphen~ $0.789$ \cellcolor{PosLite}} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Sph DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.204$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.324$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.324$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.324$ \quad $p$ ~\textdblhyphen~ $0.019^*$} \cellcolor{Neg} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.032$ \quad $p$ ~\textdblhyphen~ $0.789$} \cellcolor{NegLite} 
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/sphere_tab9.png}}  \\ \\
\end{tabularx}
\caption{Fixed effects of generalized linear mixed model from first experiment for the VST AR display}\label{tab:exp1_vst}

\end{table}


%% TABLE FOR EXP VR RESULTS
\begin{table}[!t]
\small
\centering 
\renewcommand{\arraystretch}{1.0}\setlength{\tabcolsep}{1pt} 
\begin{tabularx}{\linewidth}{@{}XXXXXXX@{}}
      \multicolumn{1}{l}{} &\multicolumn{1}{c}{Cube LS} &\multicolumn{1}{c}{Cube DS} &\multicolumn{1}{c}{Sph LS} &\multicolumn{1}{c}{Sph DS} &\multicolumn{1}{c}{Ico DS} &\multicolumn{1}{c}{Ico LS}  \\
 
        \rowcolor{Pos}\cellcolor{white} Cube LS 
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\includegraphics[width=\linewidth]{tables/cubew_tab2.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.274$ \quad $p$ ~\textdblhyphen~ $0.330$} \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.772$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.144$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.285$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.294$ \quad $p$ {\tiny \textless} $0.001^*$} \\
        
        \rowcolor{Pos}\cellcolor{white} Cube DS  
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.274$ \quad	$p$ ~\textdblhyphen~ $0.330$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/cube_tab2.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.499$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.870$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.012$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.021$ \quad	$p$ {\tiny \textless} $0.001^*$} \\
         
        \rowcolor{Pos} \cellcolor{white}Sph LS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.772$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.499$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/spherew_tab2.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.371$ \quad $p$ ~\textdblhyphen~ $0.011^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.513$ \quad $p$ {\tiny\textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.522$ \quad $p$ {\tiny\textless} $0.001^*$}	\\
         
        \rowcolor{Neg} \cellcolor{white} Sph DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.144$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.870$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.371$ \quad $p$ ~\textdblhyphen~ $0.011^*$} 	
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/sphere_tab9.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.141$ \quad $p$ ~\textdblhyphen~ $0.303$} \cellcolor{PosLite} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.151$ \quad $p$ ~\textdblhyphen~ $0.272$ \cellcolor{PosLite}}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Ico DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.285$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.012$ \quad $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.513$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.142$ \quad $p$ ~\textdblhyphen~ $0.303$} \cellcolor{NegLite} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/ico_tab3.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.009$ \quad $p$ ~\textdblhyphen~ $0.946$ \cellcolor{PosLite}} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Ico LS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.294$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.021$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.522$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.151$ \quad $p$ ~\textdblhyphen~ $0.272$ \cellcolor{NegLite}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.009$ \quad $p$ ~\textdblhyphen~ $0.946$ \cellcolor{NegLite}}
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/icow_tab2.png}}  \\ \\
\end{tabularx}
\caption{Fixed effects of generalized linear mixed model from first experiment for the VR display}\label{tab:exp1_vr}

\end{table}


==> tables/Exp1_Tables_ver2.tex <==







\begin{table*}[t]
\caption{Results of planned comparisons using binary logistic regression models for the OST AR condition are displayed. \emph{B} is the regression coefficient, SE is the standard error of the regression coefficient, $OR$ is the odds ratio, and $p$ is the significance level. Negative values for \emph{B} indicate that the first factor in the comparison was more accurate, whereas positive values indicate that the second factor was more accurate. } 
\label{tab:exp1_res}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ll Sccc Sccc Sccc}
\\
\multicolumn{14}{c}{\textbf{Results for Experiment 1}} 
\toprule
\\
&& \multicolumn{4}{c}{\textbf{OST AR}}  &\multicolumn{4}{c}{\textbf{VST AR}}  &\multicolumn{4}{c}{\textbf{VR}} \\ 
\midrule
    Predictor  &
    &\emph{B} &$SE_{B}$  &$OR$ &$[CI]_{OR}$  
    &\emph{B} &$SE_{B}$  &$OR$ &$[CI]_{OR}$ 
    &\emph{B} &$SE_{B}$  &$OR$ &$[CI]_{OR}$ \\
\midrule
    Shadow&(dark vs. light)    
        & 0.54$\ $***  &0.09    & 1.71  & $[N,M]$   
        & 0.82$\ $***   &0.11   & 2.28   & $[N,M]$ 
        & 0.21  &0.11   & 1.23   & $[N,M]$ \\ \\ 
    Shape&(cube vs. ico)                     
        & 0.16  &0.12   & 0.85   & $[N,M]$   
        &-1.08$\ $***   & 0.15   & 2.93   & $[N,M]$  
        &-2.10$\ $***  &0.16   & 8.20   & $[N,M]$  \\
       &(cube vs. sphere)                  
        &-0.35**  &0.11   & 1.42   & $[N,M]$   
        &-1.59$\ $***   & 0.14   & 4.90   & $[N,M]$  
        &-1.78$\ $***  &0.16   & 8.20   & $[N,M]$  \\
       &(ico vs. sphere)                   
        &-0.52$\ $***  &0.11    & 1.67   & $[N,M]$  
        &-0.51$\ $***   &0.11   & 1.67   & $[N,M]$  
        & 0.32$\ $**  &0.20   & 1.06   & $[N,M]$  
     \\ \\
    Shadow$\times$Shape 
     &(cube: dark vs. light)    
        & 1.44$\ $***  &0.17    & 4.21   & $[N,M]$  
        & 0.88$\ $***  &0.24   & 2.40   & $[N,M]$  
        &   &     &   &  \\
     &(ico: dark vs. light)     
        &   &     &   &
        & 1.28$\ $***  &0.17   & 3.58   & $[N,M]$ 
        &   &     &   &    \\
     &(sphere: dark vs. light)  
        &   &     &   &
        & 0.32$\ $*  &0.14   & 1.38   & $[N,M]$ 
        & 0.36$\ $*  &0.14   & 1.43   & $[N,M]$    \\ 
    Height&                                  
     &0.09$\ $*** &0.01 &1.09 &$[N,M]$ \\
    Intercept&                               & & & &  \\ %p<0.001 
\midrule 
    &\multicolumn{9}{c}{ }   &\multicolumn{4}{c}{$* p < 0.5$ \quad $** p < 0.01$ \quad $*** p < 0.001$} \\
\end{tabular}}%
\end{table*}



\begin{comment}

\begin{table}[t]
\caption{Results of planned comparisons using binary logistic regression models for the OST AR condition are displayed. \emph{B} is the regression coefficient, SE is the standard error of the regression coefficient, $OR$ is the odds ratio, and $p$ is the significance level. Negative values for \emph{B} indicate that the first factor in the comparison was more accurate, whereas positive values indicate that the second factor was more accurate. } 
\label{tab:exp1_ost}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llSccc}
\multicolumn{6}{c}{\textbf{Results for Experiment 1 in OST AR}} \\ 
\toprule
     Predictor                             &&\emph{B} &$SE_{B}$  &$OR$ &$[CI]_{OR}$  \\
\midrule
     Shadow&(dark vs. light)                  & 0.54$\ $***  &0.09    & 1.71  & $[N,M]$   \\ \\ 
     Shape&(cube vs. ico)                     &0.16  &0.12   & 0.85   & $[N,M]$   \\
      &(cube vs. sphere)                  &-0.35**  &0.11   & 1.42   & $[N,M]$   \\
      &(ico vs. sphere)                   &-0.52 ***  &0.11    & 1.67   & $[N,M]$  
     \\ \\
     Shadow$\times$Shape &(cube: dark vs. light)    & 1.44$\ $***  &0.17    & 4.21   & $[N,M]$  \\
       &(ico: dark vs. light)     &   &     &   &    \\
       &(sphere: dark vs. light)  &   &    &   &   \\ 
     Height&                                  &0.09$\ $*** &0.01 &1.09 &$[N,M]$ \\
    Intercept&                               & & & &  \\ %p<0.001 
\midrule 
    &&     \multicolumn{4}{c}{$* p < 0.5$ \quad $** p < 0.01$ \quad $*** p < 0.001$} \\
\end{tabular}}%
\end{table}

% coefficients are only slightly different :) 
% cube vs sphere (prev not signif. now yes) 


\begin{table}[t]
\caption{Results of planned comparisons using binary logistic regression models for the VST AR condition are displayed.}
\label{tab:exp1_vst}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llSccc}
\multicolumn{6}{c}{\textbf{Results for Experiment 1 in VST AR}} \\
\toprule
     Predictor                             &&\emph{B} &$SE_{B}$  &$OR$ &$[CI]_{OR}$  \\
\midrule
     Shadow 
     &(dark vs. light)                    & 0.82***  &0.11   & 2.28  & $[N,M]$  \\ \\
     Shape 
      &(cube vs. ico)                       & -1.08*** &0.15   & 2.93  & $[N,M]$  \\ 
      &(cube vs. sphere)                    & -1.59*** &0.14   & 4.90  & $[N,M]$  \\
      &(ico vs. sphere)                     & -0.51*** &0.11   & 1.67  & $[N,M]$  
     \\ \\
     Shadow$\times$Shape 
      &(cube: dark vs. light)     & 0.88*** &0.24  & 2.40  & $[N,M]$   \\
      &(ico: dark vs. light)      & 1.28*** &0.17  & 3.58  & $[N,M]$   \\
      &(sphere: dark vs. light)   & 0.32* &0.14  & 1.38  & $[N,M]$   \\ \\ 
    Height&&                     0.07$\ $*** &0.01 &1.07 &$[N,M]$ \\
    Intercept&&                  & & &  \\ %p<0.001 
     \midrule
    &&  \multicolumn{4}{c}{$* p < 0.5$ \quad $** p < 0.01$ \quad $*** p < 0.001$} \\
\end{tabular}}%
\end{table}

% coefficients are only slightly different :) 
% cube x shadows & sphere x shadows (prev not signif. now yes)

\begin{table}[t]
\caption{Results of planned comparisons using binary logistic regression models for the VR condition are displayed.}
\label{tab:exp1_vr}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llSccc}
\multicolumn{6}{c}{\textbf{Results for Experiment 1 in VR}} \\
\toprule
     Predictor                             &&\emph{B} &$SE_{B}$  &$OR$ &$[CI]_{OR}$  \\
\midrule 
     Shadow
       &(dark vs. light)                  & 0.21   &0.11  & 1.23  & $[N,M]$  \\ \\
     Shape
       &(cube vs. ico)                     & -2.10***  &0.16  & 8.20  & $[N,M]$  \\
       &(cube vs. sphere)                  & -1.78***  &0.16  & 5.95  & $[N,M]$  \\
       &(ico vs. sphere)                   & 0.32**   &0.10  & 0.73  & $[N,M]$  \\ 
     \\ 
     Shadow$\times$Shape
       &(cube: dark vs. light)     &   &  &  &  \\
       &(ico: dark vs. light)      &   &  &  &  \\
       &(sphere: dark vs. light)   & 0.36*   &0.14  &1.43  & $[N,M]$  \\ \\
    Height&&                     0.06$\ $*** &0.20 &1.06  &$[N,M]$ \\
    Intercept&&                  & & &  \\ %p<0.001 
     \midrule
    &&  \multicolumn{4}{c}{$* p < 0.5$ \quad $** p < 0.01$ \quad $*** p < 0.001$} \\
\end{tabular}}%
\end{table} 

\end{comment}

==> tables/Exp2_Tables_Big.tex <==



\fboxsep=1mm 
\definecolor{BgColor}{HTML}{ffffff} %3c92da
\definecolor{OffWhite}{HTML}{ffffff}
\definecolor{OffBlack}{HTML}{2E2E2E}



\definecolor{Pos}{HTML}{2878CC} %darker ver 2469b3
\definecolor{PosLite}{HTML}{96bfeb} 

\definecolor{Neg}{HTML}{617285}  %576778
\definecolor{NegLite}{HTML}{a2b5ca}





\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcommand{\bigcell}[2][l]{%
  \begin{tabularx}[#1]{@{}c@{}}#2\end{tabularx}}
  
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}


%% TABLE FOR EXP OST AR RESULTS 
\begin{table*}[ht]
\small
\centering 
\renewcommand{\arraystretch}{1.0}\setlength{\tabcolsep}{1pt} 
\begin{tabularx}{\linewidth}{@{}XXLLLLLLL@{}}
      \multicolumn{1}{l}{} &\multicolumn{1}{c}{Cube 45 LS} &\multicolumn{1}{c}{Dragon 45 LS} &\multicolumn{1}{c}{Dragon 0 LS} &\multicolumn{1}{c}{Cube 0 LS} &\multicolumn{1}{c}{Dragon 45 DS} &\multicolumn{1}{c}{Dragon 0 DS} &\multicolumn{1}{c}{Cube 45 DS} &\multicolumn{1}{c}{Cube 0 DS} \\
 
        \rowcolor{Pos}\cellcolor{white} Cube 45 LS  
        &\cellcolor{BgColor}\raisebox{-0.675\totalheight}{\hspace{0.5em}  \includegraphics[width=0.7\linewidth]{tables/cube45w_tab.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.912$ \newline  $p$ ~\textdblhyphen~ $0.004^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.171$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.535$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.632$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.145$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.305$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $3.061$ \newline $p$ {\tiny \textless} $0.001^*$} \\
        
        \rowcolor{Pos}\cellcolor{white} Dragon 45 LS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.912$ \newline	$p$ ~\textdblhyphen~ $0.004^*$} \cellcolor{Neg} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragonw_45_tab.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.259$ \newline $p$ ~\textdblhyphen~ $0.282$} \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.623$ \newline $p$ ~\textdblhyphen~ $0.006^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.720$ \newline $p$ ~\textdblhyphen~ $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.233$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.393$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.148$ \newline $p$ {\tiny \textless} $0.001^*$} \\
         
        \rowcolor{Pos} \cellcolor{white}Dragon 0 LS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.171$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.259$ \newline $p$ ~\textdblhyphen~ $0.282$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragonw_tab.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.364$ \newline $p$ ~\textdblhyphen~ $0.090$} \cellcolor{NegLite}
        \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.461$ \newline $p$ ~\textdblhyphen~ $0.029^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.974$ \newline $p$ {\tiny\textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.134$ \newline $p$ {\tiny\textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.890$ \newline $p$ {\tiny\textless} $0.001^*$}	\\
         
        \rowcolor{Neg} \cellcolor{white} Cube 0 LS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.535$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.623$ \newline $p$ ~\textdblhyphen~ $0.006^*$}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.364$ \newline $p$ ~\textdblhyphen~ $0.090$}  \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/cubew_tab2.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.097$ \newline $p$ ~\textdblhyphen~ $0.622$} \cellcolor{PosLite}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.610$  \newline $p$ ~\textdblhyphen~ $0.001^*$} \cellcolor{Pos}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.770$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}
        &\textcolor{white}{$\beta$ ~\textdblhyphen~ $1.526$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Dragon 45 DS 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.632$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.720$ \newline $p$ ~\textdblhyphen~ $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.461$ \newline $p$ ~\textdblhyphen~ $0.029^*$} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.097$ \newline $p$ ~\textdblhyphen~ $0.622$} \cellcolor{NegLite} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragon_45_tab.png}} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.513$ \newline $p$ ~\textdblhyphen~ $0.005^*$} \cellcolor{Pos}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.673$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.429$ \newline $p$ {\tiny \textless} $0.001^*$ } \cellcolor{Pos} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Dragon 0 DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.145$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.233$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.974$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.610$ \newline $p$ ~\textdblhyphen~ $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.513$ \newline $p$ ~\textdblhyphen~ $0.005^*$} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragon_tab.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.160$ \newline $p$ ~\textdblhyphen~ $0.327$} \cellcolor{PosLite} 
        &\textcolor{white}{$\beta$ ~\textdblhyphen~ $0.916$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Cube 45 DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.305$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.393$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.134$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.770$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.673$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.160$ \newline $p$ ~\textdblhyphen~ $0.327$} \cellcolor{NegLite} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em}  \includegraphics[width=0.7\linewidth]{tables/cube45_tab.png}} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.756$ \newline $p$ {\tiny \textless} $0.001^*$ } \cellcolor{Pos} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Cube 0 DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-3.061$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.148$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.890$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.526$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.429$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.916$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.756$ \hspace{2em} $p$ {\tiny \textless} $0.001^*$} 
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/cube_tab2.png}}  \\ \\
        
\end{tabularx}
\caption{Fixed effects of generalized linear mixed model from second experiment for the OST AR display}\label{tab:exp2_ost}

\end{table*}




%% TABLE FOR EXP VST AR RESULTS
\begin{table*}[ht!]
\small
\centering 
\renewcommand{\arraystretch}{1.0}\setlength{\tabcolsep}{1pt} 
\begin{tabularx}{\linewidth}{@{}LLLLLLLLL@{}}
      \multicolumn{1}{l}{} &\multicolumn{1}{c}{Cube 45 LS} &\multicolumn{1}{c}{Cube 0 LS} &\multicolumn{1}{c}{Cube 0 DS} &\multicolumn{1}{c}{Cube 45 DS} &\multicolumn{1}{c}{Dragon 45 LS} &\multicolumn{1}{c}{Dragon 0 LS} &\multicolumn{1}{c}{Dragon 0 DS} &\multicolumn{1}{c}{Dragon 45 DS} \\
 
        \rowcolor{Pos}\cellcolor{white} Cube 45 LS  
        &\cellcolor{BgColor}\raisebox{-0.675\totalheight}{\hspace{0.5em}  \includegraphics[width=0.7\linewidth]{tables/cube45w_tab.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.218$ \newline  $p$ ~\textdblhyphen~ $0.46$} \cellcolor{PosLite}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.113$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.429$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.445$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.608$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.177$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.219$ \newline $p$ {\tiny \textless} $0.001^*$} \\
        
        \rowcolor{Pos}\cellcolor{white} Cube 0 LS  
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.218$ \newline  $p$ ~\textdblhyphen~ $0.46$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/cubew_tab2.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.894$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.210$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.226$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.390$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.958$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.000$ \newline $p$ {\tiny \textless} $0.001^*$} \\
         
        \rowcolor{Pos} \cellcolor{white}Cube 0 DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.113$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.894$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/cube_tab2.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.316$ \newline $p$ ~\textdblhyphen~ $0.093$} \cellcolor{PosLite}
        \cellcolor{PosLite} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.332$ \newline $p$ ~\textdblhyphen~ $0.077$} \cellcolor{PosLite}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.496$ \newline $p$ ~\textdblhyphen~ $0.007^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.064$ \newline $p$ {\tiny\textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.106$ \newline $p$ {\tiny\textless} $0.001^*$}	\\
         
        \rowcolor{Neg} \cellcolor{white} Cube 45 DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.429$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.210$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.316$ \newline $p$ ~\textdblhyphen~ $0.093$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/cube45_tab.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.016$ \newline $p$ ~\textdblhyphen~ $0.930$} \cellcolor{PosLite}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.176$  \newline $p$ ~\textdblhyphen~ $0.300$} \cellcolor{PosLite}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.748$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}
        &\textcolor{white}{$\beta$ ~\textdblhyphen~ $0.790$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Dragon 45 LS 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.445$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.226$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.332$ \newline $p$ ~\textdblhyphen~ $0.077$} \cellcolor{NegLite}  
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.016$ \newline $p$ ~\textdblhyphen~ $0.622$} \cellcolor{NegLite} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragonw_45_tab.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.164$ \newline $p$ ~\textdblhyphen~ $0.343$} \cellcolor{PosLite}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.732$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.774$ \newline $p$ {\tiny \textless} $0.001^*$ } \cellcolor{Pos} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Dragon 0 LS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.608$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.390$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.496$ \newline $p$ ~\textdblhyphen~ $0.007^*$}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.180$ \newline $p$ ~\textdblhyphen~ $0.300$} \cellcolor{NegLite}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.164$ \newline $p$ ~\textdblhyphen~ $0.343$} \cellcolor{NegLite} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragonw_tab.png}} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.568$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos} 
        &\textcolor{white}{$\beta$ ~\textdblhyphen~ $0.610$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Dragon 0 DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.177$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.958$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.064$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.748$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.732$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.568$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em}  \includegraphics[width=0.7\linewidth]{tables/dragon_tab.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.042$ \newline $p$ ~\textdblhyphen~ $0.772$} \cellcolor{PosLite} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Dragon 45 DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.219$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.000$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.106$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.790$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.774$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.610$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.042$ \newline $p$ ~\textdblhyphen~ $0.772$} \cellcolor{NegLite}
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragon_45_tab.png}}  \\ \\
\end{tabularx}
\caption{Fixed effects of generalized linear mixed model from second experiment for the VST AR display}\label{tab:exp2_vst}
\end{table*}




%% TABLE FOR EXP VR RESULTS
\begin{table*}[ht!]
\small
\centering 
\renewcommand{\arraystretch}{1.0}\setlength{\tabcolsep}{1pt} 
\begin{tabularx}{\linewidth}{@{}XXLLLLLLL@{}}
      \multicolumn{1}{l}{} &\multicolumn{1}{c}{Cube 45 LS} &\multicolumn{1}{c}{Cube 0 LS} &\multicolumn{1}{c}{Cube 0 DS} &\multicolumn{1}{c}{Cube 45 DS} &\multicolumn{1}{c}{Dragon 45 LS} &\multicolumn{1}{c}{Dragon 0 LS} &\multicolumn{1}{c}{Dragon 45 DS} &\multicolumn{1}{c}{Dragon 0 DS} \\
 
        \rowcolor{Pos}\cellcolor{white} Cube 45 LS  
        &\cellcolor{BgColor}\raisebox{-0.675\totalheight}{\hspace{0.5em}  \includegraphics[width=0.7\linewidth]{tables/cube45w_tab.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.000$ \newline  $p$ ~\textdblhyphen~ $1.000$} \cellcolor{PosLite}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.275$ \newline $p$ ~\textdblhyphen~ $0.328$} \cellcolor{PosLite}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.092$ \newline $p$ {\tiny \textless} $0.001^*$}  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.507$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.549$ \newline $p$ {\tiny \textless} $0.001^*$}  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.590$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.037$ \newline $p$ {\tiny \textless} $0.001^*$} \\
        
        \rowcolor{Pos}\cellcolor{white} Cube 0 LS  
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.000$ \newline	$p$ ~\textdblhyphen~ $1.000$} \cellcolor{NegLite} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/cube45w_tab.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.275$ \newline $p$ ~\textdblhyphen~ $0.328$}  \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.092$ \newline $p$ ~\textdblhyphen~ $0.006^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.507$ \newline $p$ ~\textdblhyphen~ $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.549$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.590$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $2.037$ \newline $p$ {\tiny \textless} $0.001^*$} \\
         
        \rowcolor{Pos} \cellcolor{white}Cube 0 DS  
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.275$ \newline $p$ ~\textdblhyphen~ $0.328$} \cellcolor{NegLite}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.275$ \newline $p$ ~\textdblhyphen~ $0.328$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/cubew_tab2.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.817$ \newline $p$ {\tiny\textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.232$ \newline $p$ {\tiny\textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.274$ \newline $p$ {\tiny\textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.315$ \newline $p$ {\tiny\textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.762$ \newline $p$ {\tiny\textless} $0.001^*$}	\\
         
        \rowcolor{Neg} \cellcolor{white} Cube 45 DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.092$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.092$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.817$ \newline $p$ {\tiny \textless} $0.001^*$}  
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/cube_tab2.png}} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.817$ \newline $p$ ~\textdblhyphen~ $0.021^*$} \cellcolor{Pos}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.457$  \newline $p$ ~\textdblhyphen~ $0.011^*$} \cellcolor{Pos}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.498$ \newline $p$ {\tiny \textless} $0.005^*$} \cellcolor{Pos}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.946$ \newline $p$ {\tiny \textless} $0.001^*$} \cellcolor{Pos}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Dragon 45 LS 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.507$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.507$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.232$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.817$ \newline $p$ ~\textdblhyphen~ $0.021^*$} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragonw_45_tab.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.042$ \newline $p$ ~\textdblhyphen~ $0.803$} \cellcolor{PosLite}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.082$ \newline $p$ ~\textdblhyphen~ $0.619$} \cellcolor{PosLite}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.530$ \newline $p$ {\tiny \textless} $0.001^*$ } \cellcolor{Pos} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Dragon 0 LS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.549$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.549$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.274$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.457$ \newline $p$ ~\textdblhyphen~ $0.011^*$}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.042$ \newline $p$ ~\textdblhyphen~ $0.803$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragonw_tab.png}} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.041$ \newline $p$ ~\textdblhyphen~ $0.805$} \cellcolor{PosLite} 
        &\textcolor{white}{$\beta$ ~\textdblhyphen~ $0.488$ \newline $p$ ~\textdblhyphen~ $0.002^*$} \cellcolor{Pos}  \\ 
                        
        \rowcolor{Neg} \cellcolor{white} Dragon 45 DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.590$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.590$ \newline $p$ {\tiny \textless} $0.001^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.314$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.498$ \newline $p$ ~\textdblhyphen~ $0.005^*$} 
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.082$ \newline $p$ {\tiny \textless} $0.619$}\cellcolor{NegLite}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.041$ \newline $p$ ~\textdblhyphen~ $0.805$}\cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\hspace{0.5em}  \includegraphics[width=0.7\linewidth]{tables/dragon_45_tab.png}} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.448$ \newline $p$ ~\textdblhyphen~ $0.004^*$} \cellcolor{Pos} \\ 
        
        \rowcolor{Neg} \cellcolor{white} Dragon 0 DS   
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.037$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-2.037$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.762$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.946$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.530$ \newline $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.489$ \newline $p$ ~\textdblhyphen~ $0.002^*$} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.448$ \newline $p$ ~\textdblhyphen~ $0.004^*$} 
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\hspace{0.5em} \includegraphics[width=0.7\linewidth]{tables/dragon_tab.png}}  \\ \\
        
\end{tabularx}
\caption{Fixed effects of generalized linear mixed model from second experiment for the VR display}\label{tab:exp2_vr}

\end{table*}



==> tables/Exp2_Tables_Small.tex <==



\fboxsep=1mm 
\definecolor{BgColor}{HTML}{ffffff} %3c92da
\definecolor{OffWhite}{HTML}{ffffff}
\definecolor{OffBlack}{HTML}{141414}


\definecolor{Pos}{HTML}{3382b5} %%053061 - 3e8cbf
\definecolor{PosMed}{HTML}{3382b5} 
\definecolor{PosLite}{HTML}{cae1ee} 

\definecolor{Neg}{HTML}{C84C50}  %%900d26 - d6604d
\definecolor{NegMed}{HTML}{C84C50} %bf3338 = redsh, d6604d = orangsh
\definecolor{NegLite}{HTML}{fdd9c4}%{c6cfdb} %ff7a84 



%% TABLE FOR EXP OST AR RESULTS
\begin{table}[ht]
\small
\centering 
\renewcommand{\arraystretch}{1.0}\setlength{\tabcolsep}{1pt} 
\begin{tabularx}{\linewidth}{@{}XXXXX@{}}
      \multicolumn{1}{l}{} &\multicolumn{1}{c}{Cube 45 LS} &\multicolumn{1}{c}{Cube 0 LS} &\multicolumn{1}{c}{Cube 45 DS} &\multicolumn{1}{c}{Cube 0 DS}  \\
 
        \rowcolor{Pos}\cellcolor{white} Cube 45 LS
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\includegraphics[width=\linewidth]{tables/cube45w_tab.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.404$ \quad $p$ ~\textdblhyphen~ $0.029^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.144$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.446$ \quad $p$ {\tiny \textless} $0.001^*$} \\
        
        \rowcolor{Pos}\cellcolor{white} Cube 0 LS 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.404$ \quad	$p$ ~\textdblhyphen~ $0.029^*$} \cellcolor{Neg} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/cubew_tab2.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.309$ \quad $p$ ~\textdblhyphen~ $0.060$} \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.606$ \quad $p$ {\tiny \textless} $0.001^*$}  \\
         
        \rowcolor{Pos} \cellcolor{white}Cube 45 DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.714$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.309$ \quad $p$ ~\textdblhyphen~ $0.060$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/cube45_tab.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.297$ \quad $p$ ~\textdblhyphen~ $0.050$} 	\\
         
        \rowcolor{Neg} \cellcolor{white} Cube 0 DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.010$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.606$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.297$ \quad $p$ ~\textdblhyphen~ $0.050$} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/cube_tab2.png}}   \\ \\
        
        
        \multicolumn{1}{l}{} &\multicolumn{1}{c}{Cube 45 LS} &\multicolumn{1}{c}{Cube 0 LS} &\multicolumn{1}{c}{Dragon 45 DS} &\multicolumn{1}{c}{Cube 0 DS}  \\
 
        \rowcolor{Pos}\cellcolor{white} Dragon 45 LS
        &\cellcolor{BgColor}  \raisebox{-0.675\totalheight}{\includegraphics[width=\linewidth]{tables/dragonw_45_tab.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.404$ \quad $p$ ~\textdblhyphen~ $0.029^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.144$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $1.446$ \quad $p$ {\tiny \textless} $0.001^*$} \\
        
        \rowcolor{Pos}\cellcolor{white} Dragon 0 LS 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.404$ \quad	$p$ ~\textdblhyphen~ $0.029^*$} \cellcolor{Neg} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/dragonw_tab.png}}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $0.309$ \quad $p$ ~\textdblhyphen~ $0.060$} \cellcolor{PosLite} 
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.606$ \quad $p$ {\tiny \textless} $0.001^*$}  \\
         
        \rowcolor{Pos} \cellcolor{white}Dragon 45 DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.714$ \quad $p$ {\tiny \textless} $0.001^*$} \cellcolor{Neg}
        &\textcolor{OffBlack}{$\beta$ ~\textdblhyphen~ $-0.309$ \quad $p$ ~\textdblhyphen~ $0.060$} \cellcolor{NegLite}
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/dragon_45_tab.png}}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $0.297$ \quad $p$ ~\textdblhyphen~ $0.050$} 	\\
         
        \rowcolor{Neg} \cellcolor{white} Dragon 0 DS  
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-1.010$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.606$ \quad $p$ {\tiny \textless} $0.001^*$}
        &\textcolor{OffWhite}{$\beta$ ~\textdblhyphen~ $-0.297$ \quad $p$ ~\textdblhyphen~ $0.050$} 
        &\cellcolor{BgColor} \raisebox{-0.675\totalheight}{\includegraphics[width=0.98\linewidth]{tables/dragon_tab.png}}   \\ \\ 
        
\end{tabularx}
\caption{Fixed effects of generalized linear mixed model from first experiment for the OST AR display}\label{tab:exp2_ost}

\end{table}



==> tables/Exp2_Tables_ver2.tex <==




\begin{table}
\caption{Results for Experiment 2 in OST AR } %\haley{Currently uses Odds Ratios. But I'd rather not include a power analysis (See prior comment)}}  
\label{tab:exp2_ost}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\toprule
     Fixed effect                             &  &\emph{B}  &$OR$ &$p$ \\
\midrule
     Shadow&(dark vs. light)                     & 1.297     & 0  & $<0.0001^*$ \\ 
     Shape&(cube vs. dragon)                     & 0.507     & 0  & $<0.0001^*$ \\ 
     Orien cube&($0^\circ$ vs. $45^\circ$)       & 0.836     & 0  & $<0.0001^*$ \\ 
     Orien dragon&($0^\circ$ vs. $45^\circ$)     & 0.424     & 0  & $=0.0034^*$  
     \\ \\ 
    Shadow$\times$Shape&(cube: dark vs. light)       & 1.715 & 0  & $<0.0001^*$ \\ 
    Shadow$\times$Shape&(dragon: dark vs. light)     & 0.878 & 0  & $<0.0001^*$ \\ 
\end{tabular}}%
\end{table}


\begin{table}
\caption{Results for Experiment 2 in VST AR}
\label{tab:exp2_vst}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\toprule
     Fixed effect                             &  &\emph{B}  &$OR$ &$p$ \\
\midrule
     Shadow&(dark vs. light)                      & 0.789   & 0  & $<0.0001^*$ \\
     Shape&(cube vs. dragon)                      &-1.065   & 0  & $<0.0001^*$ \\
     Orien cube&($0^\circ$ vs. $45^\circ$)        &-0.158   & 0  & $=0.31$ \\
     Orien dragon&($0^\circ$ vs. $45^\circ$)     & 0.043    & 0   & $=0.699$  
     \\ \\
    Shadow$\times$Shape&(cube: dark vs. light)       & 1.165  & 0   & $<0.0001^*$ \\
    Shadow$\times$Shape&(dragon: dark vs. light)     & 0.669  & 0   & $<0.0001^*$ \\
\end{tabular}}%
\end{table}


\begin{table}[t]
\caption{Results for Experiment 2 in VR}
\label{tab:exp2_vr}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccc}
\toprule
     Fixed effect                             &  &\emph{B}  &$OR$ &$p$ \\
\midrule
     Shadow&(dark vs. light)                    & 0.436     & 0  & $<0.0001^*$ \\ 
     Shape&(cube vs. dragon)                    & -1.252    & 0  & $<0.0001^*$ \\ 
     Orien cube&($0^\circ$ vs. $45^\circ$)      & -0.517    & 0  & $=0.0039^*$ \\ 
     Orien dragon&($0^\circ$ vs. $45^\circ$)    & 0.261     & 0  & $=0.021^*$  
     \\ \\
    Shadow$\times$Shape&(cube: dark vs. light)    &  0.744  & 0  & $<0.0001^*$ \\
    Shadow$\times$Shape&(dragon: dark vs. light)  &  0.298  & 0  & $=0.0083^*$ \\ 
\end{tabular}}%
\end{table}

